StartLux-Decision: AutoThink Decision Models with Reinforcement Learning for Calibrated Deliberative Decisions

We introduce StartLux-Decision, decision models from 0.8B to 27B parameters that combine efficient single-pass prediction with adaptive, confidence-guided reasoning. The Instant models use bidirectional attention in full-attention layers to improve decision accuracy while keeping single-pass inference. The AutoThink models invoke explicit reasoning for uncertain decisions and answer confident cases directly. A three-stage training pipeline establishes shared decision capabilities, specializes the two variants, and equips AutoThink with reasoning through reasoning supervision and reinforcement learning. We introduce Reinforcement Learning for Calibrated Deliberative Decisions (RLCD$^2$), which uses a frozen model and proper scoring rules to reward improvements in decision probability quality and applies a soft penalty to overlong reasoning traces. RLCD$^2$ raises the share of reasoning traces that terminate within the generation limit by up to 48 percentage points and cuts average reasoning length by up to 65%, while largely preserving decision accuracy. On the public subset of Decision Index 0.3, the Instant models outperform the strongest evaluated comparable-scale open-weight decision models by 7.4-16.9 points, and the 27B AutoThink model reaches 73.4. We also introduce DecisionPivot, a programmatically verifiable benchmark of computational decisions built from contrast pairs that differ in a single answer-changing detail. On DecisionPivot, AutoThink outperforms its Instant counterparts by 11.5-18.4 points in pair accuracy and leads among evaluated systems. The models can be run using frameworks such as vLLM and MLX, with quantized versions available to reduce memory usage.Inference code and links to model weights are available at https://github.com/StartLuxLabs/Startlux-Decision .

==> sections/00_front_matter.tex <==
\begin{abstract}
We release StartLux-Decision, open decision models in six sizes (0.8B to 35B) that read a state of
text and images with typed questions. StartLux-Decision returns probabilities that a system can act
on, from one forward pass, and reasons in the same weights when the one-pass answer is unsure. A
request with three questions takes 12 to 102 ms on one H200, and one threshold on the one-pass
probability decides which questions get a thought (auto-think). On Decision Index 0.2.1 (own runs,
mostly in-domain for the later checkpoints) the 27B rises from 63.9 at release to 70.4 after a data
round and 72.3 with reasoning. Four findings mark the places where that promise can fail. Training
on the answer alone removes the end of a thought, and three stages restore it. Training data help
only the task families they contain, so reused test sets measure exposure. Reinforcement learning
calibrates the answer after a thought, mostly by shortening it. A confidence that selected an answer
overstates it (92\% right for one response, 78\% for the best of 32), and a map told what the policy
looked at closes the gap. The one-pass checkpoints and the inference package are public under CC
BY-NC 4.0 and Apache-2.0.
\end{abstract}

\begin{figure}[!htbp]
\renewcommand{\thefigure}{1}
\centering
\adjincludegraphics[max width=\linewidth,max height=0.5\textheight]{figures/fig1_headline.pdf}
\caption{At every size the StartLux-Decision checkpoints lie above the other open decision models of that size on Decision Index 0.2.1, and the one model above the released 27B is larger (31B). StartLux-Decision: own runs of the public runner between 27 September and 7 October 2026, not submitted to the board. ``With reasoning'' is the -Think checkpoint at the default threshold (one run each, and two reasoning runs of one system differ by 0.05). Orange squares: other open decision models at the size their authors name, from the maintainer-run board (read 28 September 2026), from their authors' reports, or from our own runs of the public weights. Table~\ref{tab:13} gives the provenance and date of the main points. Dashed line: the hosted reference model, whose size is not public. \dag{} with adaptive reasoning. Most systems, ours included, have training data aimed at benchmarks of the index.}\label{fig:1}
\end{figure}

\begin{figure}[!htbp]
\renewcommand{\thefigure}{2}
\centering
\adjincludegraphics[max width=\linewidth,max height=0.5\textheight]{figures/fig_flow.pdf}
\caption{One sequence of stages makes every StartLux-Decision model, and the end of a thought is lost inside it, at the data round (marker 4: the closing probability falls from 0.54 to 0.06 at 9B). A public multimodal model of each size goes through the release stage (full fine-tuning on the broad part of Lux-Release, a rank-64 adapter on its hard part, an equal blend of the two and one temperature per question type), which gives the released StartLux-Decision checkpoints. A decision data round, an adapter on the released weights trained on Lux-Rounds, gives the -Rounds checkpoints. Thinking replay, the reader round and, at 4B and 9B, the stop step, trained on Lux-Think, give the -Think checkpoints. Reinforcement learning on Lux-RL (dashed) is a variant that was not adopted. Lux-Breadth and Lux-Proc enter only the ablation rounds of Section~\ref{sec:4.4}. Lower strip: one request at inference, with the threshold $\tau$ on the top one-pass probability as the single control. Index values in the boxes are for the 4B, and the legend gives the size of every mix.}\label{fig:2}
\end{figure}


==> sections/02_models_interface.tex <==
\clearpage
\section{Models and interface}\label{sec:2}

A StartLux-Decision model answers typed questions about a state and returns a probability for every
option of every question. This chapter describes how the probabilities are read, how the same
weights reason when the one-pass answer is unsure, what the family consists of, and one change of
the attention that is under test.

\subsection{Typed decisions read in one pass}\label{sec:2.1}

A request holds a \emph{state} (a string or any JSON value, with or without images) and a set of
named questions. A question has one of three types: a choice among named options, yes or no, or a
level on an ordered scale of 2 to 10 levels, and every option may carry a criterion in words. The
response gives one answer per question with a probability for every option. Requests and responses
use the wire format of the hosted reference model of this class, so a client written for that
service works against our server unchanged.

Each question is rendered as its own prompt with the full state. The assistant turn is opened with
reasoning switched off, and the answer is read at the last position of the prompt, where the model
would write its first answer token. Nothing is generated. The logits of the option letters at that
position are divided by a temperature and normalised over the listed options. There is one
temperature per question type, fitted after training on held-out items and stored with the
checkpoint. Every fitted value is above 1: without it the read-out is too sure of itself, the more
so the smaller the model and most of all on yes/no questions.

One pass reads 26 options, one letter each. A longer list is answered by a knock-out: groups of at
most 25 options are read side by side, the three most probable options of each group go to a final
round, and the options that miss the final keep a small share of the probability. On intent lists of
228 options the released 4B, 9B and 27B answer 83.9, 88.4 and 86.8\% correctly, and the correct
option is lost before the final round in at most 2.1\% of the items. All questions of a request run
in the same forward pass, one batch row per question: a request with 1,024 questions gives
probabilities within 0.008 of those of 1,024 single requests.

A prompt can run to 262,144 tokens, the native context of the starting models. When the questions of
a request share a beginning longer than 4,096 tokens, the runtime reads it once, in chunks of 32,768
tokens, and the questions branch off it as one batch. Images are resized to at most 1,048,576 pixels
and become one token per 32 $\times$ 32 pixels. The vision tower is that of the starting model and
was never trained.

\subsection{Reasoning behind a gate}\label{sec:2.2}

The same weights can write a reasoning text, a \emph{thought}, before they answer. One number
controls this: a threshold $\tau$ on the top probability of the one-pass answer. The model writes a
thought for a question if and only if that probability is below $\tau$. With $\tau$ = 0 it never
thinks and a request costs one forward pass, with $\tau$ = 1 it always thinks, and the default is
$\tau$ = 0.9. The rule acts per question, so in a request with several questions none waits for the
thought of another.

When the gate fires, the same prompt is opened with reasoning switched on and a fixed first
sentence, and the model writes until it closes the thought or a budget of 4,096 tokens is spent. A
thought that reaches the budget is not discarded: the runtime appends a closing sentence and the
answer is read. The question is then read again with the last 4,000 characters of the thought in
context, which gives the distribution after the thought. The reported distribution, the
\emph{default answer}, is the equal mixture of the one-pass distribution and the distribution after
the thought. Averaged over all answers of an index run, a request costs 193 reasoning tokens per
answer at 27B and 497 to 1,144 at 4B, depending on the training stage. Figure~\ref{fig:2} shows how
a model is made and how it answers.

\begin{figure}[!htbp]
\renewcommand{\thefigure}{2}
\centering
\adjincludegraphics[max width=\linewidth,max height=0.5\textheight]{figures/fig2_pipeline.pdf}
\caption{How a StartLux-Decision model is made and how it answers. Upper part: the training stages in order (two rows, each read from left to right), with what each is trained on, its loss, the Decision Index 0.2.1 after it and its cost in GPU-hours on H200 (numbers for the 4B, and the index after the reader round and after the stop step is with reasoning at the default threshold). The orange mark shows where the ability to end a thought is lost. Dashed boxes: two alternatives to the three reasoning stages, both trained from the model after the data round. Lower strip: one request at inference, with the threshold $\tau$ on the top one-pass probability as the single control.}\label{fig:2}
\end{figure}

\subsection{The family}\label{sec:2.3}

Six checkpoints are public: five dense models with 0.87, 2.27, 4.66, 9.65 and 27.78 billion
parameters and a mixture of experts with about 3 of 35 billion parameters active per token
(Table~\ref{tab:1}). All are built on public multimodal models of a hybrid design, with three
linear-attention layers for every attention layer at each of the five dense sizes. Decision training
adds no parameters: adapters are merged, so a released checkpoint has the parameter count of its
starting model. The weights are in bf16 and are also distributed as GGUF files for the dense sizes.
The decision procedure (prompt, letter read-out, temperatures, knock-out) is code of the inference
package and is the same in front of every backend.

The released weights are under CC BY-NC 4.0, because several training sources carry share-alike,
non-commercial or research-only terms (Appendix~\ref{sec:D}). The inference package and the server
are under Apache-2.0. The checkpoints after the data rounds and after the reasoning stages, the
reasoning server and the training mixes are not released at the date of this version. The released
inference package answers in one pass only.

\subsection{Bidirectional attention over the prompt (under test)}\label{sec:2.4}

In every released model the attention is causal: a token sees the tokens before it and none after
it. For a one-pass decision this is inherited from the starting model and not required by the task.
The whole prompt is known before the forward pass and nothing is generated, so no position has to be
hidden from an earlier one. Under causal attention the evidence is encoded before the model has read
the question and the options, which come after it.

The entry in first place on edition 0.3 of the index lifts the causal mask in its full-attention
layers, and its model card names this change and the breadth of its training data as the two sources
of its gain. We built the same variant to test it on our recipe. A flag in the model's configuration
makes the attention layers bidirectional over the prompt of the one-pass read-out, so that every
prompt token attends to every other one. The linear-attention layers keep their causal recurrence,
as in that entry's published code, and prompt, read-out position, letters and temperatures stay as
above. Tests on CPU came before any training: with the flag off the changed code gives bit-identical
outputs on five code paths, rows of one batch do not see each other, and training and inference code
agree to within 2.2e-6 in probability. The flag switched on in a model trained with causal attention
changes the chosen option on 2 of 20 test prompts, so the attention has to be trained with it. One
cost follows from the design and has not been measured: once the evidence attends to the question, a
long shared state can no longer be read once for all questions of a request.

The first two 4B runs change nothing but the attention. With the data, the adapter and the start of
the final recipe, the flag raises the public index from 64.78 to 66.31, with every area higher, and
it is the first change in our ablations that raises the reused tasks without adding data
(Section~\ref{sec:4.3}). From the untrained model with the settings of the leading entries it raises
the index from 40.87 to 44.76. These are single runs. A repeat of the final recipe that sizes the
spread between runs, and the flag on the full-coverage round and on the first stage of the release
recipe, each against its causal counterpart, were still running when this was written
\todo[TODO(r6\_4b\_kr23ebi, s1\_4b\_bi against s1\_4b\_ca, r6\_4b\_kr23es1bi against
r6\_4b\_kr23es1ca)]{the larger runs with bidirectional prompt attention}.


==> sections/02_overview.tex <==
\clearpage
\section{Overview}\label{sec:2}

This chapter gives the whole picture on three pages: how a model is made (2.1), what it reaches
after every stage (2.2), what the stages cost (2.3), what is released (2.4), and how to read the
numbers of this report (2.5).

\subsection{Model flow}\label{sec:2.1}

\begin{figure}[!htbp]
\renewcommand{\thefigure}{2}
\centering
\adjincludegraphics[max width=\linewidth,max height=0.5\textheight]{figures/fig2_pipeline.pdf}
\caption{How a StartLux-Decision model is made and how it answers. Upper part: the training stages in order (two rows, each read from left to right), with what each is trained on, its loss, the Decision Index 0.2.1 after it and its cost in GPU-hours on H200 (numbers for the 4B, and the index after the reader round and after the stop step is with reasoning at the default threshold). The orange mark shows where the ability to end a thought is lost. Dashed boxes: two alternatives to the three reasoning stages, both trained from the model after the data round. Lower strip: one request at inference, with the threshold $\tau$ on the top one-pass probability as the single control.}\label{fig:2}
\end{figure}

The stages follow the upper lane of Figure~\ref{fig:2}. Chapter~\ref{sec:5} describes them in the
same order, and Chapter~\ref{sec:4} the data.

\textbf{Starting model.} Each size starts from a public multimodal language model of that size, with
a context of 262,144 tokens and a vision tower. Nothing is added to the architecture: an answer is
read from the model's own output layer at the 26 letter tokens.

\textbf{Release recipe.} Two models are trained from the starting weights: one with all text
parameters for one epoch on a broad mix of typed decisions (2.73 million rows, 0.79 million for the
27B), one with a rank-64 adapter for two epochs on a curated mix of hard decisions (190,418 rows,
92,228 for the 4B). Their equal-weight average is the released model. The 0.8B is the first model
alone. One temperature per question type is fitted afterwards.

\textbf{Decision data rounds.} A round is one rank-64 adapter on the released weights, one epoch,
merged. The final round has 1.08 million rows: a sample of the release mix, anchor rows whose target
is the released model's own distribution, decisions written and labelled by larger models under a
two-verifier agreement filter, general multiple choice, and sources aimed at the benchmark families
the model answers worst. Every round starts from the released weights and replaces the previous one.

\textbf{Diagnosis.} The rounds train one position, the answer letter. We measure what this does to
the ability to reason before answering and find that the end of a thought is lost: at 9B the
probability of closing a finished thought falls from 0.54 to 0.06.

\textbf{Thinking replay.} The starting model of the same size writes reasoning for training items.
The best complete sample per item becomes a target, and the decision model is trained on these
targets with a language-model loss. At inference there is one model.

\textbf{Reader round.} The model is trained to give its answer after a thought of its own, and to
keep its one-pass answer where it was.

\textbf{Stop step.} At 4B and 9B the reader round removes the end of the thought again. The model
writes thoughts, we read its answer after every eighth of each, and it is trained on its own
thoughts cut where the answer stops changing. The 27B does not need this step.

\textbf{Alternatives we measured.} One joint stage in place of the three, and policy-gradient
training of the thinker with a price per token.

\textbf{At inference} (Section~\ref{sec:3.4}). Every question is answered in one pass. If the top
probability is below the threshold $\tau$, the model writes a thought, reads it, and reports the
mixture of the two answers. The default is $\tau$ = 0.9, and $\tau$ = 0 is the one-pass model.

\subsection{Results snapshot}\label{sec:2.2}

\begin{table}[!htbp]
\renewcommand{\thetable}{2.1}
\centering
\caption{Decision Index 0.2.1 by size and stage (own runs of the public runner with one configuration, 27 September to 7 October 2026, not submitted, with reasoning at the default threshold). The full table by stage is Table~\ref{tab:5.1}, by area Table~\ref{tab:6.1} and by benchmark Appendix~\ref{sec:H}.}\label{tab:2.1}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrlll}
\toprule
\textbf{size} & {\begin{tabular}[b]{@{}r@{}}\textbf{released,}\\\textbf{one pass}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{data}\\\textbf{rounds,}\\\textbf{one pass}\end{tabular}} & \textbf{with reasoning} & {\begin{tabular}[b]{@{}l@{}}\textbf{reasoning}\\\textbf{tokens per}\\\textbf{answer}\end{tabular}} & {\begin{tabular}[b]{@{}l@{}}\textbf{thoughts at the}\\\textbf{4,096-token limit}\end{tabular}} \\
\midrule
0.8B & 38.88 & 51.60 & -- & -- & -- \\
2B & 44.19 & 57.66 & -- & -- & -- \\
4B & 52.76 & 64.78 & 67.72 and 67.37 after the stop step & 1,144 and 497 & 57.5\% and 10.4\% \\
9B & 58.64 & 67.75 & 69.77 and 70.16 after the stop step & 1,049 and 552 & 62.9\% and 15.8\% \\
27B & 63.88 & 70.43 & 72.34 & 193 & 6.0\% \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

Where to find what: interface and limits, Tables~\ref{tab:3.1} to \ref{tab:3.3}
\textperiodcentered{} other open decision models and the hosted reference, Table~\ref{tab:6.2}
\textperiodcentered{} long context, reranking, images and Chinese, Tables~\ref{tab:6.4} to
\ref{tab:6.7} \textperiodcentered{} calibration of the one-pass outputs, Section~\ref{sec:6.11}
\textperiodcentered{} selection and certificates, Tables~\ref{tab:7.1} to \ref{tab:7.3}
\textperiodcentered{} latency and throughput, Table~\ref{tab:8.1}.

\subsection{Costs}\label{sec:2.3}

All training and evaluation ran on one cluster of eight nodes with eight H200 GPUs each.
Table~\ref{tab:2.2} gives GPU-hours per stage and size. The nine training runs behind the five dense
released models took 363 GPU-hours, and the whole release campaign, with rejected and aborted runs,
about 827. A data round of the final recipe costs 20 GPU-hours at 4B and 98 at 27B with the
evaluation of its checkpoint. The three reasoning stages cost about 25 GPU-hours in total at 4B,
without the starting model's writing of the replay samples. The expensive item is evaluation with
reasoning: one index run of the 27B takes 71 GPU-hours.

\begin{table}[!htbp]
\renewcommand{\thetable}{2.2}
\centering
\caption{GPU-hours per stage and size (H200). Release rows: time reported by the trainer $\times$ GPUs of the run. Other rows: duration of the scheduled step on one node $\times$ 8, which includes loading, merging and the checks that are part of the step. \todo{the detailed compute table (02\_compute\_table.md) is to become Appendix F.10}}\label{tab:2.2}
{\footnotesize\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrrr}
\toprule
\textbf{stage} & \textbf{0.8B} & \textbf{2B} & \textbf{4B} & \textbf{9B} & \textbf{27B} \\
\midrule
release: full fine-tuning & 8.2 & 14.0 & 33.6 & 70.6 & 178.6 \\
release: adapter fine-tuning & -- & 4.5 & 4.0 & 11.1 & 38.7 \\
data round, final recipe \textsuperscript{a} & 6.0 & 8.4 & 19.6 & 28.9 & 98.4 \\
thinking replay, training \textsuperscript{b} & -- & -- & 4.0 & 4.8 & 4.9 \\
reader round & -- & -- & 6.5 & 8.2 & 16.7 \\
stop step: thoughts, read-outs, training & -- & -- & 14.1 & 15.4 & -- \\
reinforcement-learning variant (120 iterations) & -- & -- & 9.6 & -- & -- \\
Decision Index run, one pass & \todo{} & \todo{} & about 2 & about 3 & \todo{} \\
Decision Index run with reasoning \textsuperscript{c} & -- & -- & 22.8 and 13.4 after the stop step & 28.2 & 70.7 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{a} 0.8B and 2B: training time only. 4B to 27B: the whole step with merge and the
evaluation of the checkpoint. \textsuperscript{b} without the starting model's writing of the
reasoning samples \todo{add}. \textsuperscript{c} replay and reader round. The 4B trained with
reinforcement learning needs 7.0.\par}
\end{table}

\subsection{Released artefacts and licences}\label{sec:2.4}

\begin{table}[!htbp]
\renewcommand{\thetable}{2.3}
\centering
\caption{What is released at the date of this version. \todo{links; release decisions marked ``open''}}\label{tab:2.3}
{\scriptsize\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lll}
\toprule
\textbf{artefact} & \textbf{status} & \textbf{licence} \\
\midrule
six checkpoints, 0.8B to 35B-A3B (the ``released'' columns of this report) & public & CC BY-NC 4.0 \\
GGUF files of the five dense sizes (BF16, Q8\_0, Q4\_K\_M) & public & CC BY-NC 4.0 \\
inference package and server in the wire format of the hosted reference & public & Apache-2.0 \\
model cards with input and output specification and evaluation summary & public & -- \\
evaluation runner configuration and table files of this report & \todo{open} &  \\
checkpoints after the data rounds & not released (decision open) &  \\
checkpoints after the reasoning stages, and the reasoning server & not released (decision open) &  \\
calibration maps and the certificate procedure (Chapter~\ref{sec:7}) & \todo{open} &  \\
training mixes & not released (sources and licences in Table~\ref{tab:4.1}) & per source \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

The starting models are released by their authors under Apache-2.0 (Table~\ref{tab:3.3},
\todo{confirm for the 27B and the 35B-A3B}). Several training sources carry share-alike,
non-commercial or research-only terms. Appendix~\ref{sec:G} lists them, and the weights are released
for non-commercial use.

\subsection{How to read our numbers}\label{sec:2.5}

\textbf{Own runs, one configuration.} Every index value of ours is an own run of the public runner
(133,876 requests, coverage 1.0) and has not been submitted to the board. Values of other systems
are self-reported board values or values of their model cards with the date given, unless a table
says ``own run''.

\textbf{In-domain.} For the checkpoints after the data rounds, 33 of the 38 index benchmarks have
training data aimed at them in some form: an official training split, a generator in the benchmark's
layout, or related public data (Table~\ref{tab:4.3}). The index of those checkpoints measures how
well the recipe fits the suite, not zero-shot transfer. Sections~\ref{sec:6.5} to \ref{sec:6.10} and
\ref{sec:6.14} report sets that never entered training. On the 42 decision tasks among them the
released weights are as good as the checkpoints after the data rounds or better.

\textbf{Reasoning is a different operating point.} One-pass and reasoning results are reported in
separate columns. A reasoning run costs 193 additional tokens per answer at 27B and 497 to 1,144 at
4B and 9B (Tables~\ref{tab:2.1} and \ref{tab:5.6}), and its latency is that of generation.

\textbf{Spread.} Two runs of one reasoning system with thoughts sampled anew differ by 0.05 index
points. The same recipe trained twice differs by 0.18, and three rounds of nearly the same recipe
span 0.9 (Section~\ref{sec:6.1}). A difference between two training rounds below one point is not a
result unless a repeat confirms it.

\textbf{Design choices and the index.} Thresholds, mixture weights and stage designs were chosen on
held-out items of the training distribution and on a set of diagnostic items, not on the index.
Where a held-out comparison and the index disagree we say so.


==> sections/03_data.tex <==
\section{Data}\label{sec:3}

Every training row asks one question about one state, and the costliest failures we met in our data
were mismatches between the rows and the decisions they were meant to teach: a label prior, a skew
in what was asked, a shortcut in the options. A row has a question type (a choice among 2 to 26
options, a yes/no question, or a score on 2 to 10 levels), the state, the instructions, the options
with their criteria, a target probability for every option, a label kind and a parent group. All
rows derived from one state share a parent group, and decontamination and development splits act on
whole groups. At packing the option order of every row is permuted by a hash of the row, so the
position of the answer carries no information, while score levels keep their order.
Table~\ref{tab:6} lists the six mixes of this report, and Appendix~\ref{sec:D} lists every source
with its licence.

\begin{table}[!htbp]
\renewcommand{\thetable}{6}
\centering
\caption{Two mixes make the one-pass checkpoints and one makes the reasoning stages, and every label comes from a source, a program or filtered model writing. Label: H = human or source gold label, T = written or labelled by a model, P = computed by a program.}\label{tab:6}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.1092}}>{\raggedright\arraybackslash}p{\mdw{0.1512}}>{\raggedright\arraybackslash}p{\mdw{0.1966}}>{\raggedright\arraybackslash}p{\mdw{0.4559}}>{\raggedright\arraybackslash}p{\mdw{0.0737}}}
\toprule
\textbf{mix} & \textbf{used in} & \textbf{rows} & \textbf{what it holds} & \textbf{labels} \\
\midrule
Lux-Release, broad part & release stage, full fine-tuning & 2,726,203 (27B 791,992) & community corpora of typed decisions, train splits of public classification, inference, question-answering, safety, preference and tool sets, train splits of 15 index benchmarks, knowledge multiple choice, program-generated questions & H, T, P \\
Lux-Release, hard part & release stage, adapter & 190,418 (4B 92,228) & small hard decision sets, teacher-written hard decisions (2B, 9B, 27B), and smaller shares of the source families of the broad part & H, T, P \\
Lux-Rounds & decision data round & 1,078,788 & a sample of the release mix, anchor rows, teacher-labelled workplace decisions, general multiple choice, train splits and generators aimed at single index benchmarks & H, T, P \\
Lux-Breadth & ablation rounds at 4B & 642,628 core rows, and further files & 343 task families of a public collection recast as typed decisions, at most 3,000 rows per family, with single-skill, twin-reserved and benchmark-source files & H \\
Lux-Proc & ablation rounds at 4B & 135,006 & fifteen procedural families written by us: policies with exceptions, claims about logs, state tracking, table lookup, validation of a call against a schema, multi-hop answerability and others & P \\
Lux-Think & reasoning stages & replay targets 15,870 (4B), 16,369 (9B), 4,395 (27B), stop targets 5,311 (4B) & thoughts written by the starting model for training items, and the model's own thoughts with their read-outs & T \\
Lux-RL & reinforcement learning & 26,931 items & items whose one-pass top probability is below 0.9: causal questions, code execution, chess, narrative reasoning, generated arithmetic and rule tasks & H, P \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\subsection{Four kinds of source}\label{sec:3.1}

The mixes draw on four kinds of source, and each has its own failure mode.

\textbf{Converted public training splits.} Most rows are training splits of public data sets recast
as typed decisions. In the release pool the target is a single gold label of the source in 74.4\% of
the rows, a label computed by a program in 16.9\%, a distribution written by a model in 7.3\% and a
distribution that the source provides in 1.4\%. Lux-Breadth extends this kind with several hundred
task families. The failure mode is the label prior: a training split can ask a different question in
the same layout, with a different share of answers.

\textbf{Program-generated families.} Where a model has never been shown a task, we write a generator
from general knowledge of the domain and compute the label: exact-probability questions (39,995
rows, the target a counted fraction), chords on generated arrangements, phishing decisions whose
label follows from where the link points and who sends it, state tracking, select-all questions on
synthetic paragraphs, and chess positions labelled by an engine. Lux-Proc adds fifteen procedural
families whose templates are independent of our benchmark's generators. A probe that sees only the
options stays within 3 points of the majority rate in every family, and an independent second
implementation re-solves all 135,006 rows. The failure mode of generators is a shortcut in the
options.

\textbf{Written by models and filtered.} Hard decisions with one defensible answer are scarce in
public data, so open models wrote them from seeds that fix the family, the question type, a domain
and, for yes/no questions, the answer. Two verifier models answer each item blind with shuffled
labels, and an item is kept only when both choose the writer's label: 69.1\% of the valid items
passed for the release (38,150 rows) and 98.4\% for the data rounds (41,687 rows after
de-duplication). The filter cannot see a skew in what is asked. Every item of the second batch is an
exception case, and a 4B trained on it flags too much on a third-party set of invoice decisions
(exact-action agreement 39.8 $\rightarrow$ 26.0).

\textbf{Anchor rows.} A data round must not undo the release. Anchor rows have the released model's
own distribution as their target and three times the weight of an ordinary row, which holds the
model to what it already does (25,191 rows in Lux-Rounds). Lux-Think follows the same idea for the
reasoning stages: its rows are thoughts written by the starting model or by the model itself, never
by another family of models.

\begin{table}[!htbp]
\renewcommand{\thetable}{7}
\centering
\caption{More than half of Lux-Rounds is training splits aimed at single benchmarks of the index, against 10.0\% benchmark train splits in the broad part of Lux-Release. Upper block: the mixes behind the released weights, rows after packing and share of rows by source family. Lower block: Lux-Rounds by ingredient (4B build). Earlier rounds of the 4B line held 311,560 to 1,111,709 rows, and the other sizes use the sources of the lower block with an anchor of their own.}\label{tab:7}
{\footnotesize\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrr}
\toprule
\textbf{Lux-Release} & {\begin{tabular}[b]{@{}r@{}}\textbf{broad part,}\\\textbf{0.8B--9B}\end{tabular}} & \textbf{broad part, 27B} & {\begin{tabular}[b]{@{}r@{}}\textbf{hard part, 2B}\\\textbf{/ 9B / 27B}\end{tabular}} & \textbf{hard part, 4B} \\
\midrule
rows (tokens) & 2,726,203 (879 M) & 791,992 (318 M) & 190,418 (106 M) & 92,228 (41 M) \\
general public mixture & 43.6\% & 18.6\% & 12.2\% & 17.1\% \\
community corpora & 24.4\% & 17.2\% & 16.8\% & 27.5\% \\
benchmark train splits & 10.0\% & 26.4\% & 5.5\% & -- \\
knowledge and commonsense multiple choice & 7.1\% & 22.3\% & 7.7\% & 6.5\% \\
program-generated & 5.8\% & 2.5\% & 11.5\% & 6.5\% \\
small hard sets & 0.9\% & 1.4\% & 19.5\% & 40.4\% \\
teacher-written (own) & -- & -- & 19.2\% & -- \\
tools, earlier pool, safety, palettes & 8.2\% & 11.5\% & 7.5\% & 2.0\% \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\medskip
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrr}
\toprule
\textbf{Lux-Rounds, by ingredient} & \textbf{rows} & {\begin{tabular}[b]{@{}r@{}}\textbf{share}\\\textbf{of}\\\textbf{rows}\end{tabular}} \\
\midrule
sample of the release mix & 29,993 & 2.8\% \\
anchor rows (weight 3) & 25,191 & 2.3\% \\
teacher-labelled decisions & 41,687 & 3.9\% \\
general multiple choice & 29,296 & 2.7\% \\
targeted: train splits and training sides of upstream sources & 588,673 & 54.6\% \\
targeted: generators & 296,060 & 27.4\% \\
targeted: written by API models & 53,422 & 5.0\% \\
related public data & 14,466 & 1.3\% \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

Table~\ref{tab:7} shows where the weight of each mix lies. For the -Rounds and -Think checkpoints 33
of the 38 benchmarks of the index have training data aimed at them in some form, and the training
split of a public typed-decisions set is in every mix, so our score on its test split is a
specialist's.

\subsection{Decontamination and label priors}\label{sec:3.2}

\textbf{Leak scan.} Protected texts are the complete test files of the index and the 231 public
JevBench items (46 files, 1,158,879 rows at the release), later extended by third-party sets, our
twin test sets and the items of our own benchmark. Texts are cut into lower-cased word 13-grams,
hashed and sampled one in four on both sides. A training row is flagged when it shares two sampled
13-grams with the protected set, or when a protected text of 5 to 12 words (a whole query, question
or claim) equals one of its fields, and every row of a flagged parent group is dropped. A 13-gram
that recurs in more than 20 protected rows or 20 parent groups is treated as template text. The scan
removed 41,710 rows from the first 4B mix and 35,238 from the 27B mix. It has one trap of its own:
under a newer Python version it reports no hit at all, without an error, so every scan runs in a
fixed environment and is checked against a planted protected text.

\textbf{What was not filtered.} The rebuilt training splits of Lux-Release were scanned but not
filtered: 23,209 of their rows in the broad part for the 0.8B to 9B models share text with a test
row. A row-by-row comparison finds 68 rows that repeat a test item: one contract with its 17
questions that its source has in both the training and the test split, one sarcasm item, and 50
intent utterances. They correspond to 0.5 to 0.8\% of the test questions of three benchmarks. The
comparison finds equal text, not paraphrases. Every file of Lux-Rounds is filtered. The training
split of GSM8K could not be used at all: 6,017 of its 7,473 problems carry text of protected items,
because a routing benchmark of the index takes GSM8K training problems as its prompts.

\textbf{Label priors.} Before a source enters a round we compare the share of each answer with the
benchmark's, check that option and key order follow the benchmark's layout, read the rows removed as
duplicates, ask what a reader of the options alone could exploit, and test the source alone in a 4B
round. Each check comes from a failure. The official training set of a tool-retrieval benchmark has
29\% relevant candidates where the benchmark has 3\%, and with it that benchmark fell from 63.3 to
36.5 at 4B. Our first rebuild of an aspect-sentiment set had 18\% ``yes'' against 0.3\% to 3.4\% in
the benchmark's enumeration, and generated code-execution rows whose wrong options came from nearby
programs took the real benchmark from 24.9--27.1 to 13.4--15.1. A duplicate filter keyed on the
wrong fields had reduced 12,240 headline pairs to one row in the released models' mixes.

\subsection{Key findings}\label{sec:3.3}

\begin{mdfindings}
\begin{itemize}
\item The label prior of a source matters more than its size. One official training set with 29\% relevant
candidates, where the benchmark has 3\%, cost that benchmark 26 points at 4B.
\item A filter of written data checks the answer, not the question. Two verifiers agreed with 98.4\% of
the written items, and the batch still taught the 4B to flag too much, because every item was an
exception case.
\item \textbf{Decontamination needs a positive control.} The scan reports nothing, without an error, under
a newer Python version, and a scan that finds nothing looks the same as a clean file. Anyone who
builds a decision mix can run these three checks before training.
\end{itemize}
\end{mdfindings}


==> sections/03_interface_models.tex <==
\clearpage
\section{Interface and models}\label{sec:3}

StartLux-Decision answers typed questions about a state and returns a probability for every option
of every question. This chapter specifies the request and the response (Section~\ref{sec:3.1}), how
the probabilities are read in one forward pass (3.2), long inputs and images (3.3), the reasoning
mode with its single control (3.4), and the configuration of each model (3.5). A variant of the
attention over the prompt that is under test closes the chapter (3.6). Results are in
Chapter~\ref{sec:6}, and speed and memory are in Chapter~\ref{sec:8}.

\subsection{Requests, question types, outputs}\label{sec:3.1}

A request holds a \texttt{state} and a set of named \texttt{questions}. The state is a string or any
JSON value and may come with images. A question has a \texttt{type}, \texttt{instructions} and
\texttt{criteria}. The response holds one answer per question, the token usage and the model name.
Requests and responses use the wire format of the hosted reference model (the
\texttt{/\allowbreak{}v1/\allowbreak{}systemone} format of Jev), so a client written for that
service works against our server unchanged. Table~\ref{tab:3.1} lists the three question types, and
Section~\ref{sec:1.1} shows one request with its response.

\begin{table}[!htbp]
\renewcommand{\thetable}{3.1}
\centering
\caption{Question types of StartLux-Decision (all sizes, released inference package of 2026-10-03).}\label{tab:3.1}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.1054}}>{\raggedright\arraybackslash}p{\mdw{0.2204}}>{\raggedright\arraybackslash}p{\mdw{0.3250}}>{\raggedright\arraybackslash}p{\mdw{0.3354}}}
\toprule
\textbf{question type} & \textbf{what is asked} & \textbf{limits} & \textbf{what is returned} \\
\midrule
\texttt{choice} & which one of the named options holds, and every option may carry a description & at least two options \textsuperscript{a} and no upper limit: up to 26 are read in one pass, longer lists in several passes. An option name is one line of at most 200 characters & \texttt{choice}, the most probable option. \texttt{probabilities} for every option. \texttt{confidence} = (p\_max $-$ 1/n) / (1 $-$ 1/n) for n options \\
\texttt{noul} (yes/no) & whether something holds, and the two answers may carry descriptions & -- & \texttt{noul}, the probability of yes. No \texttt{confidence} field (\textbar{}2p $-$ 1\textbar{} is the equivalent) \\
\texttt{score} & a level on an ordered scale, the levels listed lowest first & 2 to 10 levels & \texttt{score}, the probability-weighted mean level counted from 0. \texttt{probabilities} per level. \texttt{legend}. \texttt{confidence} = 1 $-$ d / d\_even, floored at 0 \textsuperscript{b} \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{a} A question with a single option is answered with probability 1 without a forward
pass. \textsuperscript{b} d is the probability-weighted distance, in levels, from the most likely
level, and d\_even is that distance for an even spread measured from the middle level.\par}
\end{table}

The two \texttt{confidence} formulas are those of the hosted reference, so code that applies a
threshold to this field behaves the same against either service. The policies of this report (the
threshold of Section~\ref{sec:3.4}, the certificates of Chapter~\ref{sec:7}) act on the top
probability, not on this field.

A prompt, which is the state plus one question, can be as long as 262,144 tokens. A malformed body
is answered with status 400, and a request the model cannot answer, such as a score with more than
ten levels or a prompt over the length limit, with status 422. For comparison, the documentation of
the hosted reference (read 2026-10-03) states 255 options per choice, 64K tokens per request, text
input only and no reasoning setting.

\subsection{Reading probabilities in one pass}\label{sec:3.2}

\textbf{Position of the read-out.} Each question is rendered as its own prompt with the full state
(Listing~\ref{lst:3.1}). The assistant turn is opened with reasoning switched off, and the answer is
read at the last position of the prompt, where the model would write its first answer token. Nothing
is generated. The logits z of the option letters at that position are divided by a temperature T and
normalised over the listed options:

\begin{lstlisting}
p(option i) = exp(z_i / T_type) / Sum_j exp(z_j / T_type),   j over the options of the question.
\end{lstlisting}

\begin{figure}[!htbp]
\renewcommand{\figurename}{Listing}\renewcommand{\thefigure}{3.1}
\begin{lstlisting}
system     Apply the criterion to the evidence. Choose exactly one listed option. Answer with its letter only.
user       Evidence:
           <state: the string, or the JSON value written out>

           Question: <instructions>
           Options:
           A) <option name>: <description>
           B) ...
assistant  <empty reasoning block>          <- the option letters are read at this position
\end{lstlisting}
\caption{The prompt of one question (rendering version 3 of the released package). With images, each image takes its place inside the evidence.}\label{lst:3.1}
\end{figure}

\textbf{Option letters.} Options are lettered A, B, C, \ldots{} in the order of the request. The
levels of a score are listed lowest first, and a yes/no question shows ``yes'' and ``no''. The 26
upper-case letters are single tokens, which the package checks when a model is loaded. An option
without a description is shown by its name alone, and names that are themselves bare letters or
numbers are hidden when every option has a description, because a line such as ``A) C: Paris'' would
make the answer letter ambiguous. In a JSON state, arrays of eight or more elements carry the index
of each element, so that a question can refer to an item by its position.

\textbf{Temperature per question type.} There is one temperature for each of the three question
types. It is fitted after training on held-out items (Section~\ref{sec:5.10}) and stored with the
checkpoint. A temperature changes the probabilities and never the option that has the highest one.
The released checkpoints carry, for yes/no, choice and score questions: 3.29 / 1.76 / 1.89 (0.8B),
2.29 / 1.53 / 1.62 (2B), 1.59 / 1.39 / 1.42 (4B), 1.72 / 1.23 / 1.29 (9B) and 1.42 / 1.21 / 1.23
(27B). Every value is above 1: without the temperature the read-out is too sure of itself, the more
so the smaller the model and most of all on yes/no questions.

\textbf{Lists beyond 26 options.} One pass reads 26 options, one letter each. A longer list is
answered by a knock-out: the options are split into groups of near-equal size with at most 25
options, the groups are read side by side, the three most probable options of each group go to a
final round (which is itself split if more than 26 options reach it), and the options that miss the
final keep a share of 0.001 of the probability in proportion to their group score, so every option
gets a probability above zero. On intent lists cut or extended to a given length the released 4B /
9B / 27B answer 95.7 / 96.8 / 96.8\% at 26 options and 83.9 / 88.4 / 86.8\% at 228, and the correct
option is lost before the final round in at most 2.1\% of the items. The cost of the knock-out is
tokens and rounds (Appendix~\ref{sec:H.6}). The limit of 26 belongs to the label alphabet, not to
the model. A longer alphabet read at one position works after one short training round, as that
appendix shows. It is not part of the released models.

\textbf{Many questions per request.} All questions of a request are answered in the same forward
pass over the shared state, one row of the batch per question. Every layer is causal and the rows
are padded on the right, so a row never sees another row and padding never reaches the position that
is read: an answer does not depend on which other questions are in the request. A request with 1,024
questions runs, and its probabilities differ from those of 1,024 single requests by at most 0.008,
which is rounding inside mixed-precision batches (Section~\ref{sec:8.2}).

\subsection{Long context and images}\label{sec:3.3}

\textbf{Context length.} A prompt can run to 262,144 tokens (256K) at every size. This is the native
context of the starting models. The questions of a request repeat the state, so their prompts begin
with the same tokens. When that shared beginning is longer than 4,096 tokens the runtime reads it
once, in chunks of 32,768 tokens, and all questions branch off it as one batch
(Section~\ref{sec:8.3}). Prompts of this length take seconds, not milliseconds, and at 256K tokens
the 27B and the 35B-A3B need most of an 80 GB GPU. Accuracy on long inputs has been measured on
documents up to 128K tokens and on retrieval items up to 248K (Section~\ref{sec:6.5}).

\textbf{Images.} A request can carry images as part of its evidence. In a string state the mark
\texttt{\textless{}image\textgreater{}} shows where each image goes, one mark per image in order.
Without marks the images come first, followed by the state. Each image is resized to at most
1,048,576 pixels with its aspect ratio kept and becomes one token per 32 $\times$ 32 pixels, so a
1024 $\times$ 1024 photograph is 1,024 tokens. The vision tower runs once per request and every
question reads the same image tokens through the letter read-out described above. The tower is that
of the starting model: decision training used text only, and the data rounds changed neither the
tower nor the tokenizer. It adds 0.2 to 0.9 GB of GPU memory and can be left out when a server is
started. The GGUF and Apple-Silicon backends read text only. Results are in Section~\ref{sec:6.7}.
\todo{largest number of images per request that was tested}

\subsection{Reasoning and the single control}\label{sec:3.4}

The same weights can write a reasoning text, which we call a thought, before they answer. One number
controls this.

\textbf{The control.} A threshold $\tau$ on the top probability of the one-pass answer: the model
writes a thought for a question if and only if that probability is below $\tau$. With $\tau$ = 0 the
model never writes a thought and a request costs one forward pass. With $\tau$ = 1 it writes one for
every question. The default is $\tau$ = 0.9. The rule is applied per question, so in a request with
several questions each follows its own path and none waits for the thought of another.

\textbf{The two paths of a request} (lower strip of Figure~\ref{fig:2}).

\begin{enumerate}
\item The question is read in one pass as described above. This gives the one-pass distribution p0.
\item If max p0 $\geq$ $\tau$, p0 is returned.
\item Otherwise the same prompt is opened with reasoning switched on, and the thought starts with a fixed
sentence (``Let me work through this carefully, step by step.''). The model writes until it closes
the thought or the budget is spent.
\item The question is read again with the thought in the context, from the same option letters. This gives
the distribution after the thought, p1. The read-out sees the last 4,000 characters of the thought.
\item The reported distribution is the mixture (1 $-$ w) \textperiodcentered{} p0 + w
\textperiodcentered{} p1 with w = 0.5.
\end{enumerate}

For a list of more than 26 options the model reasons only in the final round of the knock-out. The
thought is used for the second read-out only: the response carries the answers and, in
\texttt{usage}, the number of tokens the model wrote. Requests are stateless, so no thought enters a
later request.

\textbf{Budget, and what happens at the limit.} A thought has a budget of 4,096 tokens in the index
runs of this report, or what is left of the context if that is less. A thought that has not ended at
the budget is not discarded: the runtime appends the sentence ``I have to decide now with what I
have worked out so far.'' and the closing mark, and step 4 reads the answer. No request fails
because a thought did not end. A second guard can be switched on: the thought is then written 1,024
tokens at a time and ended when its tail has become a loop, cut back to the first repeats (rules in
Appendix~\ref{sec:J.2}). A variant that looks for repetition every 256 tokens was measured on 3,021
held-out items of the training distribution that a 4B routes to reasoning: after the stop step 3.5\%
of the 4B's thoughts stay open at the budget instead of 14.1\%, and before the stop step 24.1\%
instead of 88.6\%, with the reported answer unchanged within its interval (75.60 against 75.31,
+0.30, interval $-$0.40 to +0.99, and 75.54 in both cases before the stop step). The check has not
been measured on the index. How often a thought reaches the budget depends on the size and on the
training stage (Chapter~\ref{sec:5}). In index runs at the default threshold without the guard,
6.0\% of the 27B's thoughts reach it, with 710 tokens per thought on average. At 4B and 9B the share
is 57.5\% and 62.9\% after the reader round (3,439 and 3,517 tokens per thought), and 10.4\% at 4B
after the stop step (1,585 tokens). Averaged over all answers, including those that are not thought
about, a request costs 193 reasoning tokens per answer at 27B and 497 to 1,144 at 4B (after and
before the stop step, Table~\ref{tab:5.6}).

\begin{table}[!htbp]
\renewcommand{\thetable}{3.2}
\centering
\caption{Controls of the reasoning mode and the values used in this report. Only $\tau$ is meant as a user setting. The other values belong to a checkpoint.}\label{tab:3.2}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.1469}}>{\raggedright\arraybackslash}p{\mdw{0.2543}}>{\raggedright\arraybackslash}p{\mdw{0.5848}}}
\toprule
\textbf{control} & \textbf{value} & \textbf{meaning} \\
\midrule
threshold $\tau$ & 0.9 (default), 0 = never think, 1 = always think & a thought is written when the top one-pass probability is below $\tau$ \\
mixture weight w & 0.5 & weight of the distribution after the thought in the reported distribution \\
thought budget & 4,096 tokens & at the limit: closing sentence, then the answer is read \\
opening of the thought & fixed sentence & the same for every question and size \\
sampling of the thought & temperature 0.6, top-p 0.95, top-k 20 & the two read-outs are not sampled \\
read-back & last 4,000 characters of the thought & a longer thought is marked as cut at its beginning \\
temperature after the thought & 1 & the one-pass path keeps the per-type temperatures \\
loop guard & off (default), steps of 1,024 tokens, a check every 256 tokens in the held-out test of Table~\ref{tab:5.10} & on in the runs marked ``with the detector''. With the check every 256 tokens, 3.5\% of the thoughts of the 4B after the stop step stay open at the budget instead of 14.1\% (24.1\% instead of 88.6\% before the stop step) at an unchanged answer, measured on held-out items, not on the index \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

The runs of this report use $\tau$ = 0.9 and w = 0.5 at every size. Both are values to be re-fitted
for a checkpoint on held-out items of the training distribution, never on a benchmark. One such fit,
on 9,604 held-out items of a 4B checkpoint, chose $\tau$ = 0.9 and found the accuracy flat for w
between 0.5 and 1.0. The effect of $\tau$ on accuracy and cost is in Section~\ref{sec:6.12}. A
second way to decide when to reason, a typed question about the value of reasoning that is read in
the same pass as the answer, is described in Section~\ref{sec:7.6}. It is not the default.

\textbf{Status.} The reasoning mode ran in all our evaluation runs through a server process in front
of generation servers (Appendix~\ref{sec:J.2}). The released inference package of 2026-10-03 answers
in one pass only. \todo{release status of the reasoning server, and of the checkpoints after the
reasoning stages}

\subsection{Configurations}\label{sec:3.5}

All six models are built on public multimodal language models of a hybrid design that mixes
linear-attention layers with attention layers, three linear-attention layers for every attention
layer at each of the five dense sizes. The released weights are in bf16. Decision training adds no
parameters: adapters are merged, so a released checkpoint has the parameter count of its starting
model.

\begin{table}[!htbp]
\renewcommand{\thetable}{3.3}
\centering
\caption{Model configurations, read from the released checkpoints (configuration file and tensor shapes). Vocabulary 248,320 tokens, 262,144 positions and image patches of 16 pixels at every size listed. Text layers are given as total (linear-attention, attention). The parameter count includes the vision tower with its projection, given in brackets. Download sizes are those of the released weight repositories, and GGUF files hold the text decoder only.}\label{tab:3.3}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.1151}}>{\raggedright\arraybackslash}p{\mdw{0.1795}}>{\raggedleft\arraybackslash}p{\mdw{0.1359}}>{\raggedleft\arraybackslash}p{\mdw{0.0901}}>{\raggedleft\arraybackslash}p{\mdw{0.1094}}>{\raggedright\arraybackslash}p{\mdw{0.1371}}>{\raggedleft\arraybackslash}p{\mdw{0.1014}}>{\raggedleft\arraybackslash}p{\mdw{0.1190}}}
\toprule
\textbf{model} & \textbf{starting model (licence)} & \textbf{text layers} & \textbf{hidden size} & \textbf{vision tower (layers, width)} & \textbf{parameters (vision tower)} & \textbf{released weights} & \textbf{GGUF BF16 / Q8\_0 / Q4\_K\_M} \\
\midrule
StartLux-Decision-0.8B & Qwen3.5-0.8B (Apache-2.0) & 24 (18, 6) & 1,024 & 12, 768 & 0.87B (0.10B) & 1.8 GB & 1.52 / 0.81 / 0.53 GB \\
StartLux-Decision-2B & Qwen3.5-2B (Apache-2.0) & 24 (18, 6) & 2,048 & 24, 1,024 & 2.27B (0.33B) & 4.6 GB & 3.78 / 2.01 / 1.27 GB \\
StartLux-Decision-4B & Qwen3.5-4B (Apache-2.0) & 32 (24, 8) & 2,560 & 24, 1,024 & 4.66B (0.33B) & 9.3 GB & 8.42 / 4.48 / 2.71 GB \\
StartLux-Decision-9B & Qwen3.5-9B (Apache-2.0) \textsuperscript{a} & 32 (24, 8) & 4,096 & 27, 1,152 & 9.65B (0.46B) & 19.4 GB & 17.92 / 9.53 / 5.63 GB \\
StartLux-Decision-27B & Qwen3.8-27B (Apache-2.0) \textsuperscript{b} & 64 (48, 16) & 5,120 & 27, 1,152 & 27.78B (0.46B) & 55.6 GB & 53.81 / 28.60 / 16.55 GB \\
StartLux-Decision-35B-A3B & Qwen3.6-35B-A3B \textsuperscript{b}, mixture of experts, about 3B of 35B parameters active per token & \todo{from the released checkpoint} & \todo{} & \todo{} & \todo{} & 71.9 GB & not available \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{a} Snapshot of the public repository at revision c2022362, recorded in the manifest
stored with the starting weights. \textsuperscript{b} Named by the directory of the starting weights
on the training nodes. No manifest was stored with them. \todo{licence file of the 27B and 35B-A3B
starting models; configuration and parameter count of the released 35B-A3B} The 0.8B starts from the
base (not instruction-tuned) model of its size, the 2B and 4B from the instruction-tuned models.\par}
\end{table}

\textbf{What is trained.} The release recipe trains two models from the same starting weights: one
with all text parameters fine-tuned on a broad mix of typed decisions, and one with a merged rank-64
adapter trained on a curated mix. The released 2B, 4B, 9B and 27B weights are their equal-weight
average, and the released 0.8B is the fully fine-tuned model alone (Section~\ref{sec:5.2}). A data
round is a rank-64 adapter ($\alpha$ = 128) on every projection matrix of the text layers, trained
on the released weights and merged after the round (Section~\ref{sec:5.3}). The vision tower is
never trained.

\todo{number of trainable parameters per size and stage; recipe of the 35B-A3B confirmed against its
build records}

\textbf{Precision and formats.} bf16 is the reference for every number in this report unless a table
says otherwise. The dense sizes are also distributed as GGUF files for llama.cpp, and the models run
with FP8 weights and, on Apple Silicon, through MLX (Appendix~\ref{sec:J.3}). The decision procedure
(prompt, letter read-out, temperatures, knock-out) is code of the inference package and is the same
in front of every backend.

\subsection{Bidirectional attention over the prompt (under test)}\label{sec:3.6}

In every released model the attention is causal: a token sees the tokens before it and none after
it. For a one-pass decision this is inherited from the starting model and not required by the task.
The whole prompt is known before the forward pass, the answer is read at its last position and
nothing is generated, so no position has to be hidden from an earlier one. Under causal attention
the evidence is encoded before the model has read the question and the options, which come after it,
and only the positions from the question onwards can relate the two.

The entry in first place on edition 0.3 of the index lifts the causal mask in its full-attention
layers, and its model card names this change and the breadth of its training data as the two sources
of its gain. We built the same variant to test it on our recipe. A flag in the model's configuration
makes the attention layers bidirectional over the prompt of the one-pass read-out: every prompt
token attends to every other prompt token, also to those after it. The linear-attention layers,
three of every four, keep their causal recurrence, as they do in that entry's published code. The
prompt, the read-out position, the letters and the temperatures stay those of Section~\ref{sec:3.2}.

The change lives in copies of our trainer, of the long-context runtime and of the evaluation code,
so the released path is untouched. Four tests on CPU came before any training. With the flag off,
the copies give bit-identical outputs to the originals on five code paths. Rows of one batch do not
see each other. The training code and the inference code give the same probabilities to within
2.2e-6. And the flag switched on in a model trained with causal attention changes the chosen option
on 2 of 20 test prompts, so the attention has to be trained with the flag and cannot be switched on
afterwards. One cost follows from the design: once the evidence attends to the question, a long
shared state can no longer be read once for all the questions of a request (Section~\ref{sec:8.2}).
That cost has not been measured.

Five 4B runs with the flag test the variant, each against a causal counterpart: the final-recipe
round and the full-coverage round of Section~\ref{sec:5.3.1}, the run from the untrained model with
the settings of the leading entries, the first stage of the release recipe (full fine-tuning on 2.72
million rows from the untrained model) against the causal first stage of the release, and a
full-coverage round on the first stage with the flag against the same round on the causal one.
\todo[TODO(r6\_4b\_kr20bi, r6\_4b\_kr23ebi, ft4\_abi, s1\_4b\_bi, s1\_4b\_ca, r6\_4b\_kr23es1bi,
r6\_4b\_kr23es1ca)]{results of the rounds with bidirectional prompt attention and their causal
counterparts} No released checkpoint uses this attention, and no reasoning stage has been run on a
model that does.


==> sections/04_one_pass.tex <==
\section{StartLux-Decision: one-pass training}\label{sec:4}

One-pass checkpoints have to answer decisions they were never trained for, and the public index
cannot show whether they do. The data round adds 6.5 to 13.5 index points at every size and nothing
on reused test sets, twin test sets or the rebuilt GSM8K rows (Table~\ref{tab:8}). Taken apart at
4B, every group of its data helps only the task families it contains.

\subsection{Main results}\label{sec:4.1}

\begin{table}[!htbp]
\renewcommand{\thetable}{8}
\centering
\caption{The data round raises the index at every size and leaves reused test sets, twin test sets and the rebuilt GSM8K rows where they were or lower. StartLux-Decision (released) against StartLux-Decision-Rounds in one pass. Index: Decision Index 0.2.1. Reused tasks: the 35 reused public test sets of our benchmark on items that our training data do not contain, -Rounds minus released with its 95\% bootstrap interval. Twins: the 20 twin test sets, chance-corrected, areas weighted as on the board without arts. GSM8K: the rows rebuilt for edition 0.3, chance-corrected skill. Generated tasks: second versions of three generated tasks, mean accuracy in percent. Own runs, 5 to 7 October 2026.}\label{tab:8}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrrr}
\toprule
\textbf{size} & {\begin{tabular}[b]{@{}r@{}}\textbf{index:}\\\textbf{released $\rightarrow$}\\\textbf{-Rounds}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{reused tasks:}\\\textbf{difference}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{twins:}\\\textbf{released $\rightarrow$}\\\textbf{-Rounds}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{rebuilt GSM8K:}\\\textbf{released $\rightarrow$}\\\textbf{-Rounds}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{generated}\\\textbf{tasks: released}\\\textbf{$\rightarrow$ -Rounds}\end{tabular}} \\
\midrule
0.8B & 38.88 $\rightarrow$ 51.60 & -- & -- & -- & -- \\
2B & 44.19 $\rightarrow$ 57.66 & -- & -- & -- & -- \\
4B & 52.76 $\rightarrow$ 64.78 & +0.1 {[}$-$0.6, +0.7{]} & 63.3 $\rightarrow$ 62.9 & 37.2 $\rightarrow$ 23.0 & 59.7 $\rightarrow$ 60.6 \\
9B & 58.64 $\rightarrow$ 67.75 & 0.0 {[}$-$0.6, +0.7{]} & 66.4 $\rightarrow$ 66.9 & 30.8 $\rightarrow$ 26.1 & 61.4 $\rightarrow$ 65.1 \\
27B & 63.88 $\rightarrow$ 70.43 & $-$1.0 {[}$-$1.6, $-$0.4{]} & 71.1 $\rightarrow$ 71.3 & 60.5 $\rightarrow$ 53.7 & 79.2 $\rightarrow$ 81.2 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

Table~\ref{tab:8} compares the two one-pass checkpoints of each size on Decision Index 0.2.1 and on
four sets the round was not aimed at (own runs, 5 to 7 October 2026). On the index the round gains
at every size, and there it is in-domain for 33 of 38 benchmarks. Outside the index we trail our own
released weights. On the unseen items of the reused test sets the round changes the score by $-$1.0
at 27B (interval $-$1.6 to $-$0.4), about the spread between two training runs at 4B
(Section~\ref{sec:4.4}), and by nothing at 9B and 4B, on the twin test sets it moves the 27B from
71.1 to 71.3, and on the rebuilt GSM8K rows, whose options no longer give the answer away, it is
below the released weights at every size. Only the generated tasks rise, by less than four points at
every size. We think the reason is that the round was built with the index as its development set,
so what it adds is a fit to the index's benchmarks: at 27B the largest steps are select-all
questions (+49.1 skill points), phishing decisions (+44.1), causal reasoning (+34.6) and chords
(+32.7), while at 0.8B a multiple-choice knowledge benchmark does not move (22.9 $\rightarrow$
22.5).

\subsection{Release stage}\label{sec:4.2}

A model fully fine-tuned on a broad mix and an adapter trained on hard decisions are each good at
one thing. The first carries the index, the second the hard public items: at 4B the adapter model
answers 205 of the 231 public JevBench items and the fully fine-tuned model 198. The release stage
keeps most of both by blending them. Both models are trained from the same starting weights. The
first trains all text parameters for one epoch on the broad part of Lux-Release. The loss is the
soft cross-entropy between the target distribution of a row and the softmax over its listed options,
computed on the letter rows of the model's own output layer at the last prompt position. No
parameter is added, so the quantity trained is the quantity served. The second trains a rank-64
adapter for two epochs on the hard part. The released model is their tensor-by-tensor average with
equal weights, with one temperature per question type fitted afterwards. The blend answers 204 of
the public items at 4B, and it costs the fully fine-tuned model 2.0 index points at 4B and 0.1 to
0.5 at the other sizes.

Full fine-tuning does most of the work. Read with our read-out before any training, the 27B starting
model scores 49.27, and 64.02 after that step. The 0.8B is the fully fine-tuned model alone, trained
from the base checkpoint of its size, which was the better start (38.86 against 36.76). The peak
learning rate of full fine-tuning falls with size, from 2e-5 at 0.8B to 2e-6 at 27B: at 2e-5 the 9B
scored 51.68, below the 4B at the same rate (54.82). A second-stage adapter on the fine-tuned
weights, trained on rows the first model gets wrong, scored below its parent in all eleven runs, by
0.50 to 2.86 points, and is in no released model.

\subsection{Decision data round}\label{sec:4.3}

A data round is one rank-64 adapter on every projection matrix of the text layers, trained on the
released weights for one epoch at a learning rate of 5e-5 on Lux-Rounds and merged. Rounds are not
stacked: every round starts from the released weights and replaces the previous one, so that each
round is measured against the same start. The anchor rows hold the model to its released answers. A
round costs 19.6 GPU-hours at 4B and 98.4 at 27B with the evaluation of its checkpoint. A blend
needs no training: half of the released 27B and half of StartLux-Decision-27B-Rounds score 69.23 on
the index, 82\% of the public gain, and give back about 70\% of the loss on unseen tasks ($-$0.3
against the released weights, interval $-$0.8 to +0.1).

\subsection{Ablations at 4B}\label{sec:4.4}

The round changes many things at once. On 7 and 8 October 2026 we took its data apart at 4B
(Table~\ref{tab:9}). Each adapter round starts from the released weights with the settings of
StartLux-Decision-4B-Rounds and adds one group of data to Lux-Rounds or removes one. Two rounds
combine groups. The \emph{full-coverage} round adds every group we expected to help: 200,000 rows of
Lux-Breadth, its select-all file, the training splits of the families from which our twin test sets
are built (\emph{twin-reserved families}), the families that had been held back to protect the
reused tasks of our benchmark (\emph{benchmark-source families}: rating, preference, safety and
logic sets), 97,001 rows of Lux-Proc, and two of six \emph{weak-area training sets}, arithmetic and
answerability (the other four hold sarcasm, financial-sentiment, phishing and paraphrase data). It
holds no sarcasm and no stance file. The other combined round adds the twin-reserved families at all
usable rows with breadth rows and the single-skill files of stance, sarcasm and select-all. Two
further runs follow the recipe of the leading entries of edition 0.3: all weights of the untrained
4B, one epoch at 2e-6 or 5e-6, on about 825,000 rows of Lux-Breadth and Lux-Proc.

\begin{table}[!htbp]
\renewcommand{\thetable}{9}
\centering
\caption{A group of data helps only the task families it contains, and bidirectional attention is the one change that raised every measure without new data. Ablations at 4B (one pass, own runs of 7 and 8 October 2026, one training run per row). A row is an adapter round on the released weights with the settings of StartLux-Decision-4B-Rounds, unless it says otherwise. Index: Decision Index 0.2.1. Twins: plain mean of the 20 twin tasks, chance-corrected (Table~\ref{tab:8} weights the areas as the board does). Reused tasks: the 35 reused public test sets on unseen items, paired difference to StartLux-Decision-4B-Rounds with its 95\% bootstrap interval. Generated tasks: second versions, accuracy in percent, chance 50. GSM8K: the rows rebuilt for edition 0.3, chance-corrected skill.}\label{tab:9}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.3016}}>{\raggedleft\arraybackslash}p{\mdw{0.0701}}>{\raggedleft\arraybackslash}p{\mdw{0.0696}}>{\raggedleft\arraybackslash}p{\mdw{0.1588}}>{\raggedleft\arraybackslash}p{\mdw{0.2706}}>{\raggedleft\arraybackslash}p{\mdw{0.1162}}}
\toprule
\textbf{4B checkpoint} & \textbf{index} & \textbf{twins} & \textbf{reused tasks against -Rounds} & \textbf{generated: answerable facts / filter match / tool-call validity} & \textbf{rebuilt GSM8K} \\
\midrule
\mdourrow StartLux-Decision-4B (released) & 52.76 & 61.9 & -- & 65.5 / 57.5 / 56.0 & 37.2 \\
\mdourrow StartLux-Decision-4B-Rounds & 64.78 & 61.6 & 0 & 61.5 / 63.2 / 57.2 & 23.0 \\
second run of the -Rounds recipe, mix sampled again & 64.91 & 61.8 & $-$0.7 {[}$-$1.3, 0.0{]} & 59.7 / 64.0 / 57.0 & 25.2 \\
full coverage & 64.82 & 67.6 \textsuperscript{f} & +0.8 {[}+0.1, +1.7{]} \textsuperscript{f} & 77.3 / 66.8 / 68.2 & 33.3 \\
+ Lux-Proc only (97,001 rows) & 65.03 & 61.7 & $-$0.5 {[}$-$1.2, +0.2{]} & 75.8 / 66.3 / 67.0 & 28.3 \\
+ benchmark-source families only (143,157 rows) & 65.04 & 61.8 & +1.9 {[}+1.1, +2.6{]} \textsuperscript{f} & 61.2 / 62.7 / 57.2 & 26.4 \\
+ six weak-area training sets only (117,167 rows) & 65.14 & 64.4 \textsuperscript{f} & $-$1.5 {[}$-$2.3, $-$0.9{]} \textsuperscript{f} & 59.0 / 62.5 / 58.0 & 34.1 \\
$-$ the 13,776 rows of VAST & 64.77 & 61.6 & $-$0.3 {[}$-$0.8, +0.3{]} & 58.7 / 65.2 / 56.5 & 28.9 \\
+ twin-reserved families at all usable rows (121,204), breadth and single-skill files & 65.16 & 65.6 \textsuperscript{f} & $-$1.0 {[}$-$1.7, $-$0.3{]} & 61.7 / 65.2 / 60.2 & 28.1 \\
same data, bidirectional prompt attention & 66.31 & 64.1 & +1.0 {[}+0.2, +1.8{]} & 62.7 / 66.8 / 58.8 & 25.0 \\
full coverage, bidirectional prompt attention & 66.97 & 70.8 \textsuperscript{f} & +3.9 {[}+2.9, +4.8{]} \textsuperscript{f} & 92.2 / 71.7 / 66.7 & 35.8 \\
the recipe of Section~\ref{sec:4.7}, first run & 65.81 & 72.1 \textsuperscript{f} & +3.8 {[}+2.9, +4.8{]} \textsuperscript{f} & 90.7 / 71.0 / 66.3 & 61.5 \\
the recipe of Section~\ref{sec:4.7}, second run & 66.23 & 72.2 \textsuperscript{f} & +3.6 {[}+2.6, +4.6{]} \textsuperscript{f} & 88.8 / 69.7 / 67.2 & 60.4 \\
all weights from the untrained 4B, 2e-6, Lux-Breadth and Lux-Proc only & 40.87 & 55.6 & $-$3.3 {[}$-$4.3, $-$2.2{]} & -- & 27.2 \\
the same at 5e-6 & 44.71 & 59.2 & $-$2.9 {[}$-$3.9, $-$1.8{]} & -- & 46.4 \\
the 2e-6 run with bidirectional prompt attention & 44.76 & 56.3 & $-$0.9 \textsuperscript{b} & -- & -- \\
half blend of the 2e-6 run with the released weights & 49.60 & 61.1 & $-$0.7 {[}$-$1.4, +0.1{]} & -- & 35.8 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{f} in-family: the round trains on the family or the training split of some of these
test sets. \textsuperscript{b} no interval in our record of the run.\par}
\end{table}

\textbf{What was held fixed.} Every adapter round of Table~\ref{tab:9} starts from the released
weights with the settings of the -Rounds recipe (rank-64 adapter on every projection matrix, one
epoch, learning rate 5e-5, the same packing) and differs from it only in the data named in its row.
All rounds were read by the same evaluation chain. Each row is one training run. Two runs of one
recipe have differed by 0.18 index points, three rounds of nearly the same recipe have spanned 0.9,
and a second run of the -Rounds recipe with the mix sampled again moved the index by 0.13, the twin
mean by 0.2 and single twins by up to 4.9 points, the generated tasks by $-$1.8 to +0.8 and the
reused tasks by $-$0.7 (interval $-$1.3 to 0.0): $-$1.2 on the 16 tasks outside the families of
every round and +0.2 on the 18 inside them. Differences on the reused tasks carry paired 95\%
intervals over items, and those on the other measures carry none. The interval over items does not
contain the spread between runs, so we read a change on the reused tasks as real only beyond about
one point (1.5 on one of the two parts) and a change on a single twin only beyond about five.

The public index cannot tell the data rounds apart. Every adapter round that changes only the data
lies within 0.4 points of StartLux-Decision-4B-Rounds on the index (64.77 to 65.16 against 64.78),
and three rounds of nearly the same recipe have spanned 0.9. The other measures separate the rounds,
each with a floor of its own: rounds without Lux-Proc move a generated task by $-$2.8 to +3.0
points, and rounds without the arithmetic file lie 3.4 to 5.9 skill points above the -Rounds
checkpoint on the rebuilt GSM8K rows.

Each gain sits in the families a group contains. The full-coverage round is level on the index and
gains 6.0 points on the twins, 15.8, 3.6 and 11.0 on the three generated tasks and 10.3 on the
rebuilt GSM8K rows. Lux-Proc alone gives 14.3, 3.1 and 9.8 points on the generated tasks and nothing
on the twins. Two of its fifteen families, multi-hop answerability and the validation of a call
against a schema, are of the kind that answerable facts and tool-call validity test, and those two
tasks gain most: the gain is on the kind of task the families teach, and transfer has to be read on
generated tasks of new kinds. The benchmark-source families give nothing on either. The round with
the twin-reserved families gains 4.0 on the twins, and every adapter round without twin data stays
within 0.2 of the -Rounds checkpoint there. The weak-area files give 11.1 skill points on the
rebuilt GSM8K rows through their arithmetic part.

On reused test sets the gain is exposure. The benchmark-source families hold the families of 18 of
the 35 reused tasks (preference and judging sets, safety and injection sets, FOLIO, PAWS, AmbigQA,
two legal sets and a vulnerable-code set), and 16 tasks belong to families that no file of these
rounds holds. The round on those families gives +8.6 on its 18 tasks (interval +7.1 to +10.1) and
+0.3 on the 16 others ($-$0.7 to +1.3). The full-coverage round gives +9.0 (+7.3 to +10.5) and
$-$1.3 ($-$2.5 to 0.0). The weak-area round, which holds none of the 18 families, gives $-$5.7 on
them ($-$7.1 to $-$4.5) and $-$0.8 on the 16 ($-$1.8 to +0.3). The second run of the -Rounds recipe
moves the 18 by +0.2 and the 16 by $-$1.2, so the nine points on covered families lie far outside
the spread between runs, and changes of about one point on the others do not. No group of data
raised a reused task whose family it does not contain, and the pattern holds in all three rounds in
which it can be tested. The items are unseen in every case, so for these checkpoints the 18 tasks
measure exposure to a family, and it is worth about nine points. A round can be expected to raise
the private tests of the next index edition only where its data hold their families.

\subsection{Bidirectional prompt attention}\label{sec:4.5}

With the data, adapter and start of StartLux-Decision-4B-Rounds, switching the attention layers to
bidirectional attention over the prompt (Section~\ref{sec:2.5}) raises the index from 64.78 to
66.31, with every area higher (knowledge 45.4 $\rightarrow$ 47.2, language 69.4 $\rightarrow$ 70.7,
retrieval 69.9 $\rightarrow$ 71.9, tools 86.0 $\rightarrow$ 87.3, arts 53.9 $\rightarrow$ 54.8). The
twins rise from 61.6 to 64.1, the reused tasks by 1.0 points (interval +0.2 to +1.8) and the three
generated tasks by 1.2 to 3.6 points. It is the first change in these ablations that raises the
reused tasks without adding data. From the untrained model it raises the index from 40.87 to 44.76,
with tools at 68.4 instead of 56.9, and the reused tasks from $-$3.3 to $-$0.9 against the -Rounds
checkpoint. Each is one run. The index move of the first is larger than the 0.9 that three rounds of
nearly the same recipe have spanned, and the second run of the -Rounds recipe moved the index by
only 0.13. On the reused tasks the gain lies in the 16 tasks outside the families of every round,
+3.0 (interval +1.5 to +4.5) against $-$1.2 for the second run, while the 18 inside them move by
+1.1: the change of attention raised tasks for which no data were added. On the full-coverage data
the flag gains more. Against the same round without it, the index rises from 64.82 to 66.97, the
twins from 67.6 to 70.8 and the reused tasks by 3.1 points (interval +2.2 to +3.9), 1.8 on the 18
tasks of covered families and 2.3 on the 16 others, and answerable facts goes from 77.3 to 92.2. Two
runs on two mixes, both beyond the spread between runs, make the flag part of the recipe.

\subsection{What did not work}\label{sec:4.6}

Each item below is a prediction that the ablations tested, with what we saw.

Training from the untrained model with the settings of the leading entries. If their recipe carried
over to 4B, the run would match the -Rounds checkpoint. At 2e-6 it scores 40.87 on the index and at
5e-6 44.71, below even the released weights (52.76), and it is 3.3 and 2.9 points below the -Rounds
checkpoint on the reused tasks. A half blend with the released weights does not recover it (49.60).
This is one size and one data set, and the leading entries train at 27B. One number points
elsewhere: at 5e-6 the run has the highest skill on the rebuilt GSM8K rows of any 4B checkpoint,
46.4. Its data hold no GSM8K row in the old layout, while Lux-Proc added to Lux-Rounds, which keeps
those rows, reaches 28.3. We read this as a sign that the old rows teach the model to answer from
the layout of the options.

\textbf{More rows of the same families.} If quantity mattered beyond 3,000 rows per task, 1.7 times
as many twin-reserved rows would raise the twins. They give 65.6 against 65.7 with the cap.

Data of the ``same'' skill with other labels. If any sarcasm data taught sarcasm, the weak-area
sarcasm file would raise the sarcasm twin. Three of its four sources take their label from a mark
the writer set (a hashtag, ``/s'' on Reddit) or from the site that published a headline, and in that
round the twin is at 34.6 against 39.2 for the released weights. An earlier round with other stance
and irony data sets from the task collection had lowered the stance twin from 44.9 to 36.9 and the
sarcasm twin to 32.6.

Removing a suspected source of a bias. Our checkpoints lean towards the answer ``none'' on the
stance twin. If VAST, a stance set in Lux-Rounds, caused this, the stance twin would rise without
it. Without its 13,776 rows the index, the twins and the reused tasks do not move, and the stance
twin falls from 38.7 to 29.5. When the target is not named in the text, the untrained 4B already
answers ``none'' 65\% of the time: the bias is older than our training.

\textbf{Breadth rows alone.} If breadth transferred by itself, a round on 642,628 rows of
Lux-Breadth with the core of the release mix and no file aimed at the index would raise the reused
tasks. It moves them by $-$0.6 (interval $-$1.4 to +0.1), with +0.7 on the index and 0.0 on the
generated tasks.

\subsection{The recipe as it stands}\label{sec:4.7}

The recipe for the next one-pass checkpoints has three steps. Start from the released weights. Train
one data round on Lux-Rounds with the full-coverage data, which holds neither sarcasm file, with the
GSM8K rows of the old layout replaced by 1,452 clean GSM8K training problems in the rebuilt layout
and with 45 groups of rows dropped that the current leak scan flags. Then run the reasoning stages
of Chapter~\ref{sec:5}.

The GSM8K replacement was first tested in a package of four repairs on Lux-Rounds, with ANLI cut to
8,000 rows with balanced labels, select-all rows capped at 15,000 per family with the EuroVoc cases
of fewer than two correct options removed, and the 45 flagged groups dropped. The package raises the
skill on the rebuilt GSM8K rows from 23.0 to 51.1 and lowers it on the old rows from 91.8 to 52.4.
That costs 0.67 index points (64.78 to 64.11), all of them on GSM8K: with the rebuilt rows in place
the package is 0.7 points above the -Rounds checkpoint. On the 35 reused tasks it is 1.0 point lower
(interval $-$1.7 to $-$0.2), with losses of 3 to 9 points on six tasks (two prompt-injection tasks,
FOLIO, AgentReward, NeVIR and FaithBench) and gains of 3 to 5 points on four others, which is within
the $-$0.7 that the second run of the -Rounds recipe moved. The ANLI and select-all cuts showed no
benefit on any measure, so the recipe keeps the GSM8K replacement and the leak-scan drop and leaves
the two cuts out Two runs of the recipe with bidirectional prompt attention agree
(Table~\ref{tab:9}). They reach 65.81 and 66.23 on the index, 60.4 and 61.5 skill on the rebuilt
GSM8K rows (35.8 without the replacement), 72.1 and 72.2 on the twins and +3.8 and +3.6 on the
reused tasks against StartLux-Decision-4B-Rounds. The index is 1.2 points below the full-coverage
round without the replacement because the old GSM8K rows no longer give the answer away (old-row
skill 58.3 against 92.3). With the rebuilt rows the two score the same (65.9 against 65.8), and
every other measure is level. Every adapter round of the recipe trains with bidirectional attention
over the prompt (Section~\ref{sec:4.5}). A checkpoint of this recipe is in-family on the twins and
on 18 reused tasks, so its transfer has to be read on generated tasks. No 27B round is trained
before the recipe is settled at 4B.

Six further questions were opened on 7 October, at 4B unless stated. Five are answered at 4B, and
the recipe is running at 9B:

\begin{itemize}
\item bidirectional attention over the prompt on the full-coverage round gains more than on the -Rounds
data (Section~\ref{sec:4.5}). Set from the first stage of the release stage it adds nothing beyond
setting it in the data round (index 67.04 against 66.97, reused tasks +0.2, interval $-$0.5 to
+0.9). Both rounds that start from the first stage alone, without the adapter half and the blend of
the release stage, score 10 to 13 points higher on tool-call validity than the same rounds from the
released weights (78.0 against 68.2 causal, 79.5 against 66.7 bidirectional) and stay level
elsewhere, one run each. On the recipe of this section the gain does not repeat: started from the
first stage alone the round scores 66.00 on the index (65.81 and 66.23 from the released weights),
54.5 on the reused tasks (55.7, 53.3), 71.7 on the twins (72.1, 72.2) and 65.2 on tool-call validity
(66.3, 67.2). The second half of the release stage neither helps nor hurts the final round at 4B
\item contrast pairs for stance and sarcasm written by other language models, in two versions (16,036
rows, and 8,859 rows filtered against surface cues): the filtered file raises the stance twin from
38.7 to 45.5 (a second run of the recipe moves it by $-$0.4) and leaves the other measures within
the spread between runs, while the unfiltered file raises nothing (stance 37.5, sarcasm 36.1).
Filtering the pairs against surface cues decides whether they teach stance, and neither version
helps sarcasm
\item large files from the original training splits of the twin sources and their relatives (368,053 rows
from Corr2Cause, ProofWriter, VitaminC, WANLI and others) raise the twins from 61.6 to 69.7, all of
it on their own families (ProofWriter 43.3 to 95.6, Corr2Cause 35.4 to 88.0), leave the index
(65.00) and the generated tasks where they were, and lower the reused tasks by 2.0 points (interval
$-$2.7 to $-$1.2), beyond the spread between runs. They stay out of the recipe
\item ten families of the public procedural corpus from which the leading entry's procedural rows come,
9,000 rows each, raise the index by 0.9 points (64.78 to 65.69) and leave the generated tasks where
they were (59.3, 64.0 and 57.3 against 61.5, 63.2 and 57.2), with $-$0.6 {[}$-$1.2, 0.0{]} on the
reused tasks, while our own procedural families lift the same three generated tasks by 14.3, 3.1 and
9.8 points. The corpus is fitted to the index, not to the decisions behind it. On top of the recipe
of this section it adds nothing to the index (65.96 against 65.81 and 66.23 for two runs without it)
and lowers tool-call validity by 3 to 4 points and the twins by 1.1, so it stays out
\item a second run of the -Rounds recipe gives the spread between runs used in Section~\ref{sec:4.4}
(Table~\ref{tab:9})
\item the recipe at 9B, with bidirectional attention over the prompt, raises the index from 67.75 to
68.29, the reused tasks from 51.9 to 59.1, the generated tasks of version 0 from 72.6 to 77.1 and
the twins from 66.2 to 73.0 over the -Rounds checkpoint (one run). Answerable facts, filter match
and tool-call validity go from 63.8, 62.5 and 68.8 to 88.8, 72.2 and 74.3. At 9B the recipe moves
the reused and generated tasks far more than the index
\end{itemize}

\subsection{Key findings}\label{sec:4.8}

\begin{mdfindings}
\begin{itemize}
\item A group of training data helps only the task families it contains. Rating, preference and safety
families raise the 18 reused tasks of their families by 8.6 points and the 16 others by 0.3, and
Lux-Proc raises generated tasks of its kind by 3.1 to 14.3 points.
\item The public index cannot tell data rounds apart. Every round that changes only the data lies within
0.4 index points of the -Rounds checkpoint, while the other four measures move by several points.
\item \textbf{Bidirectional attention over the prompt is the one change that raised every measure without
new data}, from 64.78 to 66.31 on the index and by 1.0 points on the reused tasks in its first 4B
run.
\item \textbf{Training all weights from the untrained model with the settings of the leading entries, more
rows of the same families, and data of the ``same'' skill with other labels did not help at 4B.}
\end{itemize}
\end{mdfindings}


==> sections/04_training_data.tex <==
\clearpage
\section{Training data}\label{sec:4}

This chapter documents the data of both training lines: the release recipe (Section~\ref{sec:5.2}),
which produced the public weights, and the decision data rounds (Section~\ref{sec:5.3}), which
produced the evaluated checkpoints that are not yet released. Every source is converted into one
record format, the typed decision. Table~\ref{tab:4.1} lists the sources, Table~\ref{tab:4.2} the
composition of every mix, and Table~\ref{tab:4.3} what each mix contains that is aimed at a
benchmark of the Decision Index. The release drew on a pool of 6,397,500 candidate decisions in 25
source files. The final data round trains on 1,078,788 rows from 30 files. Appendix~\ref{sec:G} has
the per-data-set licence tables, the generators, the teacher prompts and the filter statistics.
Section~\ref{sec:4.1.1} lists data that was built on 7 October 2026 for the decision data rounds
that were running when this was written. None of it is in a released model or in the final data
round.

\subsection{Sources and conversion to typed decisions}\label{sec:4.1}

\textbf{Record format.} A training row asks one question about one state. It has a type, which is a
choice among 2 to 26 options (C), a yes/no question (Y) or a score on 2 to 10 ordered levels (S),
and it has the state, the instructions, the options with their criteria, a target probability for
every option, a label kind, a parent group and an optional weight. The target is a single gold label
of the source in 74.4\% of the release pool, a label computed by a program in 16.9\%, a distribution
written by a model in 7.3\%, and a distribution that the source provides (several annotators, an
exact probability) in 1.4\%. All rows derived from one state share a parent group, and
decontamination and development splits act on whole groups.

\textbf{Conversion.} One converter per source maps its fields to this record. A label becomes a
one-hot target. A distribution is kept, normalised and rounded to six decimals. A choice with more
than 26 options keeps every option with positive probability and is filled to 26 at random. Rows
with a uniform target are dropped as placeholders (137,203 rows of one community corpus), except
program labels and questions that are undecidable by design. Train splits of benchmarks are rebuilt
in the request layout of the index's public kit, from train and development files only. At packing
the option order of every row is permuted by a hash of the row, so the position of the answer
carries no information. Score levels keep their order. Rows longer than 12,288 tokens are dropped,
not truncated.

\begingroup
\renewcommand{\thetable}{4.1}
\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\begin{longtable}{>{\raggedright\arraybackslash}p{\mdw{0.2474}}>{\raggedright\arraybackslash}p{\mdw{0.0859}}>{\raggedleft\arraybackslash}p{\mdw{0.1178}}>{\raggedright\arraybackslash}p{\mdw{0.1007}}>{\raggedright\arraybackslash}p{\mdw{0.1761}}>{\raggedright\arraybackslash}p{\mdw{0.0831}}>{\raggedright\arraybackslash}p{\mdw{0.1761}}}
\caption{Sources. Block A: the candidate pool of the release by source family (rows in the pool $\rightarrow$ rows in the full-fine-tuning mix of the 0.8B to 9B models). Block B: the final decision data round (4B build, rows after de-duplication). Label: H = human or source gold label, T = written or labelled by a model, P = computed by a program. Licences are as stated on the official card or repository on 7 October 2026, and ``mixed'' is resolved per data set in Tables~\ref{tab:G.4} to \ref{tab:G.6}. The last column names the index benchmark at which the rows are aimed.}\label{tab:4.1}\\
\toprule
\textbf{source} & \textbf{type} & \textbf{rows} & \textbf{label} & \textbf{licence} & \textbf{split} & \textbf{in-domain for} \\
\midrule
\endfirsthead
\multicolumn{7}{l}{\textit{Table~\thetable{} (continued)}}\\
\toprule
\textbf{source} & \textbf{type} & \textbf{rows} & \textbf{label} & \textbf{licence} & \textbf{split} & \textbf{in-domain for} \\
\midrule
\endhead
\bottomrule
\endfoot
\textbf{A. Release: candidate pool} &  & \textbf{6,397,500} &  &  &  &  \\
Community corpora of typed decisions (four) & C Y S & 2,224,874 $\rightarrow$ 664,849 & T, P, H & Apache-2.0, CC0-1.0 / CC BY 4.0 by source, mixed per row, one ``unknown'' & train & -- \\
General public mixture: train splits of public classification, inference, question-answering, safety, preference and tool sets, with format variants (Table~\ref{tab:G.4}) & C Y S & 1,976,644 $\rightarrow$ 1,189,277 & H, P, T & mixed, with non-commercial and share-alike sets & train & BANKING77, CLINC150, WinoGrande, HellaSwag \\
Program-generated: a public procedural corpus (729,910) and our exact-probability questions (39,995) & C Y S & 769,905 $\rightarrow$ 157,045 & P & Apache-2.0, own & -- & -- \\
Train and development splits of 15 index benchmarks, rebuilt in the suite's layout & C Y & 441,457 $\rightarrow$ 273,022 & H & mixed: one CC BY-NC 4.0, two CC BY-SA 4.0, four without a stated licence & train, dev & those benchmarks \\
Tool-use decisions from three function-calling corpora, agent traces and API-Bank training dialogues & C & 340,899 & source labels & Apache-2.0, CC BY 4.0, MIT & train & BFCL (layout), API-Bank \\
Knowledge and commonsense multiple choice (twelve public sets) and When2Call preference pairs & C & 292,428 $\rightarrow$ 194,029 & H & mixed: one CC BY-NC 3.0, one non-commercial research only, one CC BY-SA 4.0, two ``unknown'' & train & WinoGrande, HellaSwag, When2Call, layout of MMLU-Pro, GPQA \\
Pool of public train splits from an earlier project of ours & C Y S & 238,469 & H & mixed, with CC BY-NC and CC BY-NC-SA sets & train & -- \\
Small hard decision sets (four public sets) & C Y S & 39,281 $\rightarrow$ 25,444 & T, P & Apache-2.0, CC BY 4.0 & train & -- \\
Teacher-written hard decisions (own, Section~\ref{sec:4.2}) & C Y S & 38,150 (adapter mixes only) & T & own & -- & -- \\
Safety judgments (WildJailbreak, 8,000 prompts per data type) & C Y & 31,997 & source labels & ODC-BY, gated & train & -- \\
Colour-palette preference pairs & C & 3,396 & H & not confirmed & train ratings & cfcolor \\
\textbf{B. Final decision data round} &  & \textbf{1,078,788} &  &  &  &  \\
Teacher-labelled workplace decisions (Section~\ref{sec:4.2}) & C Y S & 41,687 & T & own & -- & -- \\
Sample of the adapter mix of the release & C Y S & 29,993 & as in A & mixed & train & -- \\
Anchor rows: target is the released model's own distribution, weight 3 & C Y S & 25,191 & the model & own & -- & -- \\
General multiple choice (seven public sets) & C & 29,296 & H & mixed (as above) & train & layout of MMLU-Pro, GPQA \\
Replay of the train splits of 13 index benchmarks & C Y & 100,679 & H & mixed (Table~\ref{tab:G.5}) & train, dev & 13 benchmarks (Table~\ref{tab:4.3}) \\
Aspect-category sentiment in the benchmark's enumeration, weight 0.2 & Y & 234,504 & H & none stated & train & ACOS \\
Shopping-query relevance, square-root label shares & C & 89,904 & H & Apache-2.0 & train & Amazon ESCI \\
Sarcasm categories for every training text, weight 0.5 & Y & 20,736 & H & MIT & train & iSarcasmEval \\
When-to-call decisions, official training set & C & 8,798 & source labels & CC BY 4.0 & train & When2Call \\
WinoGrande train (20,000 of 40,398) & C & 20,000 & H & none on the card, repository Apache-2.0 & train & WinoGrande \\
Colour-palette preference pairs & C & 3,396 & H & not confirmed & train ratings & cfcolor \\
Group-statement preference, training questions & C & 2,236 & H & CC BY 4.0 & train & Habermas Machine \\
Forecasting questions resolved before the test window & Y & 7,825 & outcomes & CC BY-SA 4.0 & before 2026-07-01 & ForecastBench \\
Select-all questions, training side of six upstream sources & Y & 100,595 & H, classifier scores & mixed (Table~\ref{tab:G.5}) & train & SATA-Bench \\
Entity-level financial sentiment, another corpus & C & 13,975 & H & MIT & whole set & FinEntity (related) \\
Long-document questions, 20,000--46,000 characters & C Y & 491 & H & \todo{sources} & train & -- \\
Causal reasoning, generated & \todo{} & 31,363 & P & own & -- & CLadder \\
Select-all on synthetic paragraphs, generated & Y & 48,019 & P & own & -- & SATA-Bench \\
Narrative reasoning: planned by program, written by a model, verified & C & 9,547 & P, T & own & -- & MuSR \\
Appliance simulator, generated & C & 52,401 & P & own & -- & home appliance simulator \\
Phishing decisions on e-mails with a link, generated, weight 0.5 & C Y & 63,000 & P & own & -- & PhishNChips \\
Chess positions with engine labels (40,000 of 65,555) & C & 40,000 & P & own, engine GPL-3.0 & -- & ChessBench \\
Chord recognition on generated arrangements & C & 12,000 & P & own & -- & POP909-CL \\
State tracking and deduction, generated & C & 39,730 & P & own & -- & BBH \\
Retrieval items written by API models & Y & 35,567 & T & own \todo{provider terms} & -- & BRIGHT \\
Limerick minimal pairs: written by an API model, corrupted by program & C & 17,855 & T, P & own & -- & BPoMP \\
\end{longtable}
\endgroup

\subsubsection{Data groups added on 7 October 2026 (in no released model)}\label{sec:4.1.1}

Five groups of data were built on 7 October 2026 for the rounds of Section~\ref{sec:5.3} that test
breadth in place of index-targeted sources. \textbf{None of them is in a released model, and none is
in the final data round of Table~\ref{tab:4.1}.} Only the breadth and single-skill files have been
in measured rounds, three experimental rounds at 4B (Table~\ref{tab:5.13}). The other groups enter
rounds that were running or queued when this was written, and the multilingual file is in no round
yet. In this section a \emph{task}, or task family, is one source of the public task collection. The
\emph{release line} is the training line that also trains on families from which test sets of ours
are built. The rounds measured so far belong to the other line, which keeps those families out.

\begingroup
\renewcommand{\thetable}{4.4}
\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\begin{longtable}{>{\raggedright\arraybackslash}p{\mdw{0.2548}}>{\raggedright\arraybackslash}p{\mdw{0.1325}}>{\raggedright\arraybackslash}p{\mdw{0.0896}}>{\raggedleft\arraybackslash}p{\mdw{0.0870}}>{\raggedright\arraybackslash}p{\mdw{0.0638}}>{\raggedright\arraybackslash}p{\mdw{0.1342}}>{\raggedleft\arraybackslash}p{\mdw{0.0944}}>{\raggedright\arraybackslash}p{\mdw{0.1312}}}
\caption{Data groups of 7 October 2026 (rows after cleaning). ``Removed'': rows left out while a file was built because a part of the row equals an item text of a protected evaluation set (b), and rows of parent groups flagged by the scan of Section~\ref{sec:4.5} on the finished file (s). Licence by rows: commercial use allowed / no licence stated / non-commercial, in the most restrictive reading of the licence that the collection's release records for each source. H = source label, P = computed by a program. Last column: where the file is used.}\label{tab:4.4}\\
\toprule
\textbf{group} & \textbf{file} & \textbf{tasks or data sets} & \textbf{rows} & \textbf{label} & \textbf{removed} & \textbf{licence by rows} & \textbf{used in} \\
\midrule
\endfirsthead
\multicolumn{8}{l}{\textit{Table~\thetable{} (continued)}}\\
\toprule
\textbf{group} & \textbf{file} & \textbf{tasks or data sets} & \textbf{rows} & \textbf{label} & \textbf{removed} & \textbf{licence by rows} & \textbf{used in} \\
\midrule
\endhead
\bottomrule
\endfoot
Breadth: task families of a public collection recast as typed decisions (tasksource), at most 3,000 rows per task, label shares of the source & \texttt{ts\_v1\_core} & 343 tasks & 642,628 & H & s 648 & 340,383 / 251,494 / 50,751 & three measured 4B rounds (all rows, or 200,000) \\
\ldots{} multilingual, at most 600 rows per task & \texttt{ts\_v1\_multi} & 102 tasks & 47,784 & H & s 6 & 30,390 / 14,394 / 3,000 & no round yet \\
Single skills: stance (rows of the two files above, repeated) & \texttt{ts\_\allowbreak{}v1\_\allowbreak{}stance} & 18 tasks & 17,378 & H & s 9 & 10,721 / 5,344 / 1,313 & two measured 4B rounds, left out of the full-coverage round \\
\ldots{} sarcasm and irony (likewise repeated) & \texttt{ts\_\allowbreak{}v1\_\allowbreak{}sarcasm} & 10 tasks & 18,158 & H & s 1 & 8,152 / 10,006 / 0 & two measured 4B rounds, left out of the full-coverage round \\
\ldots{} select-all: one yes/no question per candidate label, from source rows with at least two true labels & \texttt{ts\_\allowbreak{}v1\_\allowbreak{}multilabel} & 3 tasks & 8,995 & H & s 0 & 8,995 / 0 / 0 & two measured 4B rounds, rounds in progress \\
Twin-reserved families: training rows of the families from which twin test sets are built & \texttt{ts\_\allowbreak{}v1\_\allowbreak{}twinfam} & 33 tasks & 72,426 & H & rows equal to twin items at build, s 340 & 32,672 / 30,813 / 8,941 & release line only, rounds in progress \\
\ldots{} three tasks whose training rows share text with twin items (Corr2Cause 2,812, CODAH 1,965, ReClor 2,981) & \texttt{ts\_\allowbreak{}v1\_\allowbreak{}twinfam2} & 3 tasks & 7,758 & H & b 807 (CODAH 529, ReClor 278), s 208 & 4,777 / 2,981 / 0 & release line only, rounds in progress \\
Benchmark-source families: tasks held back to protect reused tasks of the benchmark of Section~\ref{sec:6.14} and other protected sets (rating and preference data, safety sets, FOLIO, PAWS and others) & \texttt{ts\_v1\_v0fam} & 58 tasks & 143,157 & H & b 6,089, s 1,164 & 73,502 / 54,562 / 15,093 & release line only, rounds in progress \\
Procedural families: twelve generated families, and three more & \texttt{kr\_proc4}, \texttt{kr\_proc4b} & 15 families & 108,005 + 27,001 & P & s 0, audit (below) & own & rounds in progress \\
Weak-area training sets: arithmetic 19,954, answerability 32,000, sarcasm 29,750, financial sentiment 10,777, phishing e-mail 11,621, paraphrase 13,065 & \texttt{kr\_weak1\_{*}} (six files) & 20 data sets & 117,167 & H & b: a flagged row is replaced by the next candidate, s 53 & per data set (below) & rounds in progress \\
GSM8K training problems without protected text, held aside & \texttt{kr\_\allowbreak{}weak1\_\allowbreak{}gsm8k\_\allowbreak{}clean} & 1 data set & 2,912 & H & 6,017 of 7,473 problems excluded & MIT & \textbf{no mix} \\
\end{longtable}
\endgroup

\textbf{How the files are cleaned.} Three levels are used, from coarse to fine. \emph{Families.}
Before a row of the task collection is read, whole tasks are excluded: 91 that are, or feed, an
evaluation set of ours, 38 that are reserved for the twin test sets of Section~\ref{sec:6.15}, and 8
in Chinese. Of these 137, 41 are out because a link to a protected set could not be ruled out. A
first scan against the evaluation index (which since 7 October also holds the items of the twin test
sets and of the benchmark of Section~\ref{sec:6.14}) exposed 21 more families, which were dropped
whole: among them an entailment set against ANLI, a set of mathematics questions against the
documents of the index's retrieval benchmark, a logic set against the LogiQA twin, and two sets that
occur inside long-context evaluation documents. Among rating and preference data the breadth files
keep the HelpSteer families. UltraFeedback, hh-rlhf, oasst and prm800k share texts with evaluation
tasks of ours, stay out of the breadth files and are in the benchmark-source file after its
item-level cleaning. Inside a kept task nothing is rebalanced: in 15 tasks of the core file and 2 of
the benchmark-source file one label has more than 90\% of the rows. For 72 tasks of the breadth
files, and 84 over all eight files, the collection has a single split, and the rows come from the
training part of its own release. \emph{Items.} Every finished file passes the scan of
Section~\ref{sec:4.5} and loses each flagged parent group: 664 rows over the five breadth and
single-skill files, 340 and 208 in the two twin-reserved files, 1,164 in the benchmark-source file,
46 and 7 in the arithmetic and the phishing file. \emph{Equality.} The files that come close to an
evaluation set by design get a stricter filter while they are built. A row is left out when its
state, one half of a paired state, a line or an option equals an item text of any of the 120
protected sets, and in the benchmark-source file also when it is the same sentence up to a few
words. This left out 6,089 rows of that file, 529 of 2,495 usable CODAH rows and 278 of 4,481 usable
ReClor rows. In the weak-area files the test runs on word sequences of at least five words for every
candidate row, a flagged row is replaced by the next candidate, and a data set with more than 30\%
of flagged rows is not written. That rule excluded the training split of GSM8K: 6,017 of its 7,473
problems (80.5\%) carry text of protected evaluation items, because the routing benchmark of the
index takes GSM8K training problems as its prompts, and a few more are documents of its retrieval
benchmark. The older pool file that holds these problems in the benchmark's two layouts had met the
same texts: its scan flags 78\% of them, and 806 and 820 rows remain in mixes. The 1,456 problems
without protected text are held aside in a file of 2,912 rows. The procedural families have an audit
of their own (Section~\ref{sec:5.3}): probes that see only the options, or the question and the
options, stay within 3 points of the majority rate in every family, probes on length are at 0.50, an
independent second implementation re-solves all 135,006 rows, the scan flags none, and no row shares
a 13-gram with the 6,000 generated benchmark items.

\textbf{Licences, and what a file makes in-family.} By rows, 340,383 rows of the core file come from
sources that allow commercial use, 251,494 from sources that state no licence and 50,751 from
sources under non-commercial terms. The other files built from the collection are in
Table~\ref{tab:4.4}. The weak-area files are recorded per data set. AQuA-RAT and MathQA are
Apache-2.0. DuoRC is MIT. QuAC and SQuAD 2.0 are CC BY-SA 4.0 (the Hub card of QuAC says MIT). Of
the four sarcasm sources one is MIT and three state no licence on the copy used (for one of the
three, a set of news headlines, the author's own page states CC0). The financial-sentiment sources
are MIT except Financial PhraseBank (CC BY-NC-SA 3.0, 3,447 rows). The e-mail sources are CC BY 4.0
for three curated corpora, CC BY-NC 4.0 for a collection of phishing mail (2,969 rows) and not
stated for the copy of the Enron mail. The paraphrase sources allow research use only (MRPC, 3,065
rows) and non-commercial research use (Quora Question Pairs, 10,000 rows). The procedural families
are our own. Three groups change what an evaluation set measures for a model trained on them. The
twin-reserved files make the twin test sets of their families in-family. The benchmark-source file
makes the reused benchmark tasks named for each of its tasks in-family. And the weak-area files use,
by decision, the training split of SQuAD 2.0, whose evaluation side is a reused benchmark task, and
the training split of the FiQA card, whose test split is a twin. The test items themselves were
removed or never read, and scores of such a model on these sets are reported as in-family scores
(Sections~\ref{sec:6.14} and \ref{sec:6.15}). Two limits remain: no person has audited the new rows,
and in the phishing file the label is the corpus a message comes from: positives and negatives come
from different corpora and years, so part of that decision can be made from style.

\subsection{Teacher-labelled decisions and the agreement filter}\label{sec:4.2}

Hard decisions with one defensible answer are scarce in public data, so we let open models write
them. Both batches use one pipeline, and the prompts are in Appendix~\ref{sec:G.7}.

\begin{enumerate}
\item \textbf{Seeds.} A seed fixes the family, the question type, a domain or occupation and the length of
the state. For a yes/no question it also fixes the answer, so the batch is balanced by construction.
\item \textbf{Writing.} Qwen3.8-27B writes one item per seed as a JSON object with the rationale before
the gold label (temperature 0.9, top-p 0.95, at most 16,000 new tokens). No benchmark item is shown
to the writer.
\item \textbf{Structural checks.} Type and labels as seeded, no answer field inside the state, and for
probability items a stated distribution whose top label lies between 0.5 and 0.9.
\item \textbf{Agreement filter.} Two verifiers, Qwen3.8-27B and Qwen3.6-35B-A3B, answer each item blind,
with reasoning and with shuffled labels. An item is kept when both choose the writer's gold label.
\item \textbf{Scan.} Kept items pass the contamination scan of Section~\ref{sec:4.5}.
\end{enumerate}

\emph{Release batch.} Thirteen families of hard decisions over 45 domains. A quarter of the seeds
were written by Qwen3.6-35B-A3B, and the writers' reasoning was switched off after a pilot in which
36.5\% of the items hit the token limit. Of 80,000 seeds, 55,272 items passed the structural checks,
69.1\% of those passed both verifiers (57.1\% for subtle-error judging, 85.6\% for hard routing, and
239 of 245 in the pilot with reasoning), and 38,150 rows entered the pool. They are in the adapter
mix of the 2B, 9B and 27B only (36,579 rows), and the released 0.8B and 4B contain none. We have no
comparison that isolates their effect.

\emph{Data-round batch.} Eleven families, led by five workplace families: rubric assessment of
documents from 80 occupations, invoice processing under an approval policy, customer support under a
service policy, review of agent traces, triage of security alerts. The writer reasons before it
writes. Of the 48,000 seeds of the first batch 28,381 items were structurally valid (16,000 were cut
off at the token limit) and 27,939 passed both verifiers (98.4\%). Two smaller batches gave 6,908
and 6,953 items \todo{their seed counts and pass rates}. After de-duplication 41,687 rows are in
every data round. Two API models that answered 5,000 of these items agreed with the gold label on
98.9\% and 99.4\%.

The batch has a fault the filter cannot see: every item is an exception case. The invoice family has
1,142 ``escalate'', 716 ``hold'' and 35 ``approve'' labels, and a 4B trained on the batch flags too
much: on a third-party set of invoice decisions (evaluation only) its exact-action agreement fell
from 39.8 to 26.0, while a control round with anchor rows alone stayed at 39.3. A further batch of
routine cases did not repair this (30.2 and 32.4) and is not in the final mix.

\subsection{Programmatic generators}\label{sec:4.3}

Where a model has never been shown a task, we write a generator from general knowledge of the
domain. No evaluation item is read into a generator. Only category-level error tables are.
Appendix~\ref{sec:G.6} describes each generator.

\begin{itemize}
\item \textbf{Exact labels by program.} Exact-probability questions (release): 39,995 rows in eight
families, the target computed as a fraction and re-counted from the rendered text. Chords on
generated arrangements: 12,000 rows, and no song of the benchmark's corpus is read, because every
song of it is in the evaluation pool. Phishing decisions: 9,000 e-mails with seven questions each.
The label follows from where the link points and who sends it, and the same scenarios occur in both
classes. State tracking and deduction: 52,000 rows built. Select-all questions on synthetic
paragraphs with the benchmark's 38\% share of correct options: 48,019 rows.
\item \textbf{Labels by an engine.} Chess positions with every legal move analysed by an open engine
(65,555 rows built). The chess benchmark's official training values could not be used: they are
shuffled over 2,148 shards with about one move per position in a shard.
\item \textbf{Planned by program, written by a model.} Narrative reasoning: a planning step fixes 12,000
stories and 4,000 more of the object-placement kind, Qwen3.8-27B writes them, and only verified
stories are kept (9,547 rows) \todo{verification rule and pass rate}.
\item \textbf{Written by API models.} For reasoning-intensive retrieval, GLM-5.3 and DeepSeek-V4-Pro wrote
6,000 items (a query, one or two useful documents and tempting useless ones), and 5,162 were kept
after a blind verifier of the other model family had confirmed every positive. For a limerick
benchmark built from the one large limerick corpus, 13,510 limericks were written anew, and 6,167
pass a rhyme check against a pronouncing dictionary and yield 17,920 pairs with a programmatic
corruption.
\item \textbf{Two further generators.} Causal reasoning (31,363 rows) and the appliance simulator (52,401
rows) \todo{what is sampled and how the label is computed}.
\end{itemize}

Every generator and every rebuilt split passes five checks before it enters a round. (1)
\textbf{Label prior:} the share of each answer is compared with the benchmark's, per query where the
benchmark groups candidates. (2) \textbf{Layout parity:} option order and key order are compared
with the layout in which the suite stores the benchmark, and two families differed and were rebuilt
(68,661 tool-retrieval rows, 52,941 simulator rows). (3) \textbf{Duplicates:} after every build we
read the rows removed as duplicates per source. (4) \textbf{Options only:} we ask what a reader of
the options alone could exploit. One of our reasoning testbeds was answerable from its options in
81\% of the items and was replaced. (5) \textbf{One source, one round:} a new source is first tested
in a 4B round that differs from a finished round by that source only.

\subsection{Mixing a round}\label{sec:4.4}

A mix is built from per-source quotas and caps. Parent groups flagged by the scan are dropped, exact
duplicates are removed across files, and the shuffle is seeded by the name of the mix. A row weight
scales the loss of a row: 0.2 for the enumerated aspect--sentiment rows, 0.5 for the phishing and
sarcasm-category rows, 3 for the anchor rows.

\begin{table}[!htbp]
\renewcommand{\thetable}{4.2}
\centering
\caption{Composition of every mix. Block A: the four mixes behind the released weights, rows after packing and share of rows per source family. Block B: the final data round by ingredient (4B build). Earlier rounds of the 4B line: round 7 has 311,560 rows, round 11 665,896, round 14 838,446, round 18 1,081,189 and round 19 1,111,709 (Tables~\ref{tab:F.5} and \ref{tab:G.3b}). The other sizes use the sources of block B with an anchor of their own. The 27B takes its sample from its own full-fine-tuning mix.}\label{tab:4.2}
{\footnotesize\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrr}
\toprule
\textbf{A. Release mixes} & {\begin{tabular}[b]{@{}r@{}}\textbf{full fine-tuning,}\\\textbf{0.8B--9B}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{full fine-tuning,}\\\textbf{27B}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{adapter, 2B}\\\textbf{/ 9B / 27B}\end{tabular}} & \textbf{adapter, 4B} \\
\midrule
rows (tokens) & 2,726,203 (879 M) & 791,992 (318 M) & 190,418 (106 M) & 92,228 (41 M) \\
general public mixture & 43.6\% & 18.6\% & 12.2\% & 17.1\% \\
community corpora & 24.4\% & 17.2\% & 16.8\% & 27.5\% \\
benchmark train splits & 10.0\% & 26.4\% & 5.5\% & -- \\
knowledge and commonsense multiple choice & 7.1\% & 22.3\% & 7.7\% & 6.5\% \\
program-generated & 5.8\% & 2.5\% & 11.5\% & 6.5\% \\
small hard sets & 0.9\% & 1.4\% & 19.5\% & 40.4\% \\
teacher-written (own) & -- & -- & 19.2\% & -- \\
tools, earlier pool, safety, palettes & 8.2\% & 11.5\% & 7.5\% & 2.0\% \\
C / Y / S & 64.9 / 23.6 / 11.5\% & 76.9 / 16.4 / 6.7\% & 58.9 / 31.3 / 9.8\% & 46.2 / 41.3 / 12.4\% \\
prompt tokens, median / 99th percentile & 164 / 2,405 & 191 / 3,962 & 305 / 3,443 & 260 / 2,974 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\medskip
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrr}
\toprule
\textbf{B. Final data round, by ingredient} & \textbf{rows} & {\begin{tabular}[b]{@{}r@{}}\textbf{share}\\\textbf{of}\\\textbf{rows}\end{tabular}} \\
\midrule
sample of the release mix & 29,993 & 2.8\% \\
anchor rows (weight 3) & 25,191 & 2.3\% \\
teacher-labelled decisions & 41,687 & 3.9\% \\
general multiple choice & 29,296 & 2.7\% \\
targeted: train splits and training sides of upstream sources & 588,673 & 54.6\% \\
targeted: generators & 296,060 & 27.4\% \\
targeted: written by API models & 53,422 & 5.0\% \\
related public data & 14,466 & 1.3\% \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

More than half of the final rows are train splits, and one source, the enumerated aspect--sentiment
pairs, is 21.7\% of the rows at a fifth of the weight per row. In round 14, the last round for which
we have a weight table, about 85\% of the weight was aimed at single benchmarks \todo{the same table
for the final round}.

\subsection{What is in-domain, and decontamination}\label{sec:4.5}

Table~\ref{tab:4.3} is the context for every index number in this report.

\begin{table}[!htbp]
\renewcommand{\thetable}{4.3}
\centering
\caption{Training data aimed at each of the 38 benchmarks of the Decision Index 0.2.1. T = official training split or training set of the benchmark's source. G = our generator or written data in the benchmark's request layout, containing nothing of the benchmark. R = related public data in the benchmark's layout. -- = nothing aimed at it.}\label{tab:4.3}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.1026}}>{\raggedright\arraybackslash}p{\mdw{0.3742}}>{\raggedright\arraybackslash}p{\mdw{0.2156}}>{\raggedright\arraybackslash}p{\mdw{0.2939}}}
\toprule
\textbf{area} & \textbf{benchmark} & \textbf{released models} & \textbf{final data rounds} \\
\midrule
tools & function calling (BFCL) & R & R \\
tools & tool retrieval (ToolRet) & -- & -- (T in rounds 14, 18 and 19, removed) \\
tools & API-Bank & T \textsuperscript{a}, R & R \\
tools & When2Call & T (preference pairs, 2,700 rows) & T \\
tools & home appliance simulator & -- & G \\
retrieval & BANKING77, CLINC150 & T & T \\
retrieval & reasoning-intensive retrieval (BRIGHT) & -- & G (written items, none of its documents) \\
retrieval & Amazon ESCI & T & T (resampled) \\
retrieval & phishing decisions (PhishNChips) & -- & G \\
retrieval & claim verification (HoVer) & T & T \\
language & ContractNLI, ANLI, VAST, NLI4CT, RAGTruth, iSarcasm & T & T \\
language & WinoGrande, HellaSwag & T \textsuperscript{a} & T \\
language & aspect-category sentiment (ACOS) & T & T (resampled) \\
language & FinEntity & -- & R \\
knowledge & GSM8K & T & T \\
knowledge & causal reasoning (CLadder), MuSR & -- & G \\
knowledge & select all that apply (SATA-Bench) & -- & G, and T of its upstream sources \\
knowledge & chess (ChessBench) & -- & G \\
knowledge & BBH fixed-option tasks & -- & G (from round 18, no held-out claim on BBH) \\
knowledge & GPQA Diamond, MMLU-Pro & R \textsuperscript{b} & R \textsuperscript{b} \\
knowledge & HLE, CRUXEval & -- & -- \\
arts & chord recognition (POP909-CL) & -- & G \\
arts & Humicroedit & -- (1 row, Section~\ref{sec:4.6}) & T \\
arts & cfcolor & T \textsuperscript{a} & T \\
arts & New Yorker caption matching & T & T \\
arts & Habermas Machine, ForecastBench & -- & T \\
arts & limerick minimal pairs (BPoMP) & -- & G \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{a} \todo{confirm per size.} The manuscript lists these rows for the 27B only. The
internal record of the release says the full-fine-tuning mix of the smaller models contains the same
files. \textsuperscript{b} Layout only: general multiple-choice questions from other sources are
written in the two layouts in which the suite stores these benchmarks. The manuscript marks both
``--''.\par}
\end{table}

The released models have official training splits for 16 (4B line) to 18 (27B) of the 38 benchmarks
by the manuscript's count and for 19 by the internal record of the release, and the public
repository marks 14 \todo{settle the count and correct the public table}. The final rounds have data
aimed at 33 benchmarks, 35 with the two layout-only cases. Tool retrieval, an adversarially filtered
expert set and code execution are read zero-shot. Outside the index, the training split of a public
typed-decisions set (1,200 cases, 5,978 questions) is in every mix: our score on its test split is a
specialist's.

\textbf{Method.} Protected texts are the complete test files of the index and the 231 public
JevBench items (46 files, 1,158,879 rows at the release), extended on 1 October by five third-party
workflow sets and a long-context set. Texts are cut into lower-cased word 13-grams, hashed and
sampled one in four on both sides. A training row is flagged when it shares two sampled 13-grams
with the protected set, or when a protected text of 5 to 12 words (a whole query, question or claim)
equals one of its fields. Every row of a flagged parent group is dropped. A 13-gram that occurs in
more than 20 protected rows, or in more than 20 parent groups of the training file, is treated as a
template and ignored. Corpora that a benchmark shares between its training and test side (candidate
documents, tool schemas, product pages) are not protected. The query, question or claim always is.

\textbf{What it found, release.} The scan removed 41,710 rows from the first 4B mix and 35,238 from
the 27B mix. The rule on recurring training text was added after the first scan had flagged 64,990
rows of one multiple-choice file. With it the count is 9,723, and one of 1,319 GSM8K test questions
passes inside a community-corpus row. The rebuilt train splits were scanned but not filtered: 38,077
of their rows share text with a test row (ANLI 20,941), and 23,209 such rows are in the
full-fine-tuning mix of the 0.8B to 9B models, 20,253 in that of the 27B. A row-by-row comparison
made for this report shows what these flags are. Of the 425,112 rows of the rebuilt train splits, 18
have the state, the question and the options of a test question: 17 are one non-disclosure agreement
that its source has in both the training and the test split, with its 17 hypotheses, and one is a
sarcasm item. Fifty more (25 utterances in each of two intent benchmarks) repeat an utterance of the
test split with another option list. None of the 162,865 ANLI rows equals a test item. The flagged
ones share sentences of a premise passage, and the other flags are shared documents and fixed task
wording. The 68 rows correspond to 0.5 to 0.8\% of the test questions of three benchmarks. The
comparison finds equal text after normalisation, not paraphrases. The public statement that test
items were filtered out of these splits describes a step that was not taken, although its substance
holds up to these rows \todo{correct the public page}.  Test sets that third parties later cut from
public training data overlap as well: 62 of 310 items of a tool-calling suite and 41 of 400 cases of
the typed-decisions test split are flagged.

\textbf{What it found, data rounds.} Every new file is filtered, the replayed train splits included
\todo{the 27B rounds sample 30,000 rows of the 27B release mix, whose train-split rows were not
filtered; count them}. The scan removed 10,151 of 18,496 forecasting rows, 10,064 of 52,000
state-tracking rows and 741 of 1,500 EU-law documents of the select-all source. It over-flags
official training sets that share tool descriptions with the test side (5,856 of 8,918 When2Call
questions). There a question-level check replaces it (120 dropped, 8,798 kept). For the select-all
benchmark we looked its evaluation rows up in the upstream training files: 910 of 1,048 rows of four
subsets are there and are excluded by text.

\subsection{Key findings}\label{sec:4.6}

\begin{mdfindings}
\textbf{Targeted sources move single benchmarks and little else.} Twelve thousand generated chord
rows take chord recognition from 9.4 to 78.3 (4B, chance-corrected skill, one pass), the phishing
generator takes phishing decisions from 14.5 to 72.1, and four select-all sources add 0.5 to 0.6
index points at 4B, 9B and 27B through their benchmark alone. On a third-party set of agent
decisions (evaluation only) the 4B stands at 64.80 strict accuracy after six index points of data
rounds and at 64.95 before them.

\textbf{Official training rows with a different label prior lower the score.} The official training
set of the tool-retrieval benchmark has seven candidates per query of which 29\% are relevant. The
benchmark has 32 near neighbours of which 3\% are. With 68,661 such rows the benchmark fell from
63.3 to 36.5 at 4B, again from 62.7 to 36.5 after we had rewritten the rows in the suite's layout,
and from 61.8 to 34.9 at 9B. Without them it is back at 63.1 and the index at 64.29 instead of
63.32.

\textbf{Our own sampling of official splits had the same fault three times.} Aspect-category
sentiment had 18\% ``yes'' in our first rebuild against 0.3\% to 3.4\% in the benchmark's
enumeration. The natural enumeration gives 43.9 $\rightarrow$ 61.2. Shopping relevance was sampled
with uniform labels against a natural mix under macro-F1. Square-root shares give 45.0 $\rightarrow$
51.3. Sarcasm categories were built for sarcastic texts only and are asked for every text.

\textbf{Generated code-execution data lowers the score.} Rows whose wrong options were outputs of
nearby programs made the correct option the one most similar to the others: 24.9--27.1 $\rightarrow$
13.4--15.1 at 4B and 33.8 $\rightarrow$ 26.0 at 9B. The rows are out, and code execution stays
zero-shot.

\textbf{Rows that look like the benchmark and teach another task are worse than no rows.} Four
thousand single-turn rows rebuilt from the training dialogues of a tool-use benchmark took it from
85.4 to 32.4 ($-$1.94 index points).

\textbf{A duplicate filter keyed on the wrong fields removed whole families.} The mixer compared
state, instructions and option identifiers, not option texts: 12,240 headline pairs became 1 row and
17,920 limerick pairs 1. The released models were trained with this fault. In the first round after
the fix the headline benchmark rose from 19.2 to 29.1.

\textbf{Real data added nothing over the generator, and written data did not help its benchmark.}
21,479 chord rows from human lead sheets (CC BY-NC-SA 3.0) gave 80.5 against 78.3 and were dropped.
With the written retrieval items the retrieval benchmark stands 2.0 to 3.2 points below the round
before them (39.1 $\rightarrow$ 35.9--37.1). Their 19.6\% positives are again far from the
benchmark's prior, and we have no round that isolates them.

\textbf{A round is one draw.} The same recipe mixed under another seed scores 60.69 and 60.87 on the
index, with phishing decisions at 72.1 and 64.9. We read a difference only after pairing items and
after a repeat (Section~\ref{sec:6.1}).
\end{mdfindings}


==> sections/04_training_recipe.tex <==
\clearpage
\section{Training recipe}\label{sec:4}

A model is trained in two parts. The release recipe turns a public language model into a model that
answers a typed question in one forward pass. Data rounds then add tasks that the released model was
never shown. This chapter describes both, takes the data of the rounds apart at 4B, and states the
recipe as it stands after those ablations. The ablations give the main result of the chapter: a
group of data helps only the task families it contains, and the public index cannot tell the rounds
apart. The settings of every stage are in Appendix~\ref{sec:C}.

\subsection{Release recipe}\label{sec:4.1}

Two models are trained from the same starting weights. The first trains all text parameters for one
epoch on a broad mix (2,726,203 rows, 791,992 for the 27B). The loss is the soft cross-entropy
between the target distribution of a row and the softmax over its listed options, computed on the
letter rows of the model's own output layer at the last prompt position. No parameter is added, and
the quantity trained is the quantity served. The second trains a rank-64 adapter for two epochs on a
curated mix of hard decisions (190,418 rows, 92,228 for the 4B). The released model is their
tensor-by-tensor average with equal weights, with one temperature per question type fitted
afterwards. The 0.8B is the first model alone, trained from the base checkpoint of its size, which
was the better start (38.86 against 36.76). The peak learning rate of full fine-tuning falls with
size, from 2e-5 at 0.8B to 2e-6 at 27B: at 2e-5 the 9B scored 51.68, below the 4B at the same rate
(54.82).

The released models score 38.88, 44.19, 52.76, 58.64 and 63.88 on the index from 0.8B to 27B. Full
fine-tuning does most of it: read with our read-out before any training the 27B starting model
scores 49.27, and 64.02 after that step. Averaging costs the fully fine-tuned model 0.1 to 0.5 index
points (2.0 at 4B) and keeps most of what the adapter model gains on the hard public items. A
second-stage adapter on the fine-tuned weights, trained on rows the first model gets wrong, scored
below its parent in all eleven runs, by 0.50 to 2.86 points, and is in no released model.

\subsection{Decision data rounds}\label{sec:4.2}

A data round is one rank-64 adapter on every projection matrix of the text layers, trained on the
released weights for one epoch at a learning rate of 5e-5 and merged. Rounds are not stacked: every
round starts from the released weights and replaces the previous one. The final round has 1,078,788
rows.

In one pass the final round scores 51.60, 57.66, 64.78, 67.75 and 70.43 from 0.8B to 27B. At 27B the
largest steps are select-all questions (+49.1 skill points), phishing decisions (+44.1), causal
reasoning (+34.6) and chords (+32.7). The rounds add tasks, not knowledge: at 0.8B a multiple-choice
knowledge benchmark does not move (22.9 $\rightarrow$ 22.5) and graduate-level science questions
fall from 10.2 to 0.0.

Outside the index the rounds do not help. On the unseen items of 35 reused public test sets the
final round changes the score of the released weights by $-$1.0 at 27B (95\% interval $-$1.6 to
$-$0.4), by 0.0 at 9B and by +0.1 at 4B. On 20 twin test sets, which measure skills of index
benchmarks on other data, the 27B scores 71.1 before the round and 71.3 after it. And on the GSM8K
rows rebuilt for edition 0.3 of the index, whose options no longer give the answer away, the rounds
are below the released weights at every size, by 6.8 skill points at 27B, 4.7 at 9B and 14.2 at 4B.
A blend needs no training: half of the released 27B and half of the final round score 69.23 on the
index, 82\% of the public gain, and give back about 70\% of the loss on unseen tasks ($-$0.3 against
the released weights, interval $-$0.8 to +0.1).

\subsection{Ablations at 4B}\label{sec:4.3}

The final round changes many things at once. On 7 and 8 October 2026 we took its data apart at 4B.
Each adapter round of Table~\ref{tab:3} starts from the released weights with the settings of the
final recipe and adds one group of data to its mix or removes one. Two rounds combine groups. The
\emph{full-coverage} round adds every group we expected to help: 200,000 rows from several hundred
public task families (\emph{breadth rows}), a select-all file, the training splits of the families
from which our twin test sets are built (\emph{twin-reserved families}), families that had been held
back to protect the reused tasks of our benchmark (\emph{benchmark-source families}: rating,
preference, safety and logic sets), 97,001 procedural rows, and two of six \emph{weak-area training
sets}, arithmetic and answerability (the other four hold sarcasm, financial-sentiment, phishing and
paraphrase data). It holds no sarcasm and no stance file. The other combined round adds the
twin-reserved families at all usable rows with breadth rows and the single-skill files of stance,
sarcasm and select-all. Two further runs follow the recipe of the leading entries of edition 0.3:
all weights of the untrained 4B, one epoch at 2e-6 or 5e-6, on about 825,000 rows of breadth and
procedural data. Every round was trained once and read on five measures.

\begin{table}[!htbp]
\renewcommand{\thetable}{3}
\centering
\caption{Recipe ablations at 4B (one pass, own runs of 7 and 8 October 2026, one training run per row). A row is an adapter round on the released weights with the settings of the final recipe, unless it says otherwise. Index: Decision Index 0.2.1. Twins: plain mean of the 20 twin tasks, chance-corrected. Reused tasks: the 35 reused public test sets of our benchmark on items that our training data do not contain, paired difference to the final recipe with its 95\% bootstrap interval. Generated tasks: second versions, accuracy in percent, chance 50. GSM8K: the rows rebuilt for edition 0.3, chance-corrected skill.}\label{tab:3}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.2962}}>{\raggedleft\arraybackslash}p{\mdw{0.0701}}>{\raggedleft\arraybackslash}p{\mdw{0.0696}}>{\raggedleft\arraybackslash}p{\mdw{0.1693}}>{\raggedleft\arraybackslash}p{\mdw{0.2661}}>{\raggedleft\arraybackslash}p{\mdw{0.1155}}}
\toprule
\textbf{4B checkpoint} & \textbf{index} & \textbf{twins} & \textbf{reused tasks against the final recipe} & \textbf{generated: answerable facts / filter match / tool-call validity} & \textbf{rebuilt GSM8K} \\
\midrule
released weights & 52.76 & 61.9 & -- & 65.5 / 57.5 / 56.0 & 37.2 \\
final recipe & 64.78 & 61.6 & 0 & 61.5 / 63.2 / 57.2 & 23.0 \\
full coverage & 64.82 & 67.6 \textsuperscript{f} & +0.8 {[}+0.1, +1.7{]} \textsuperscript{f} & 77.3 / 66.8 / 68.2 & 33.3 \\
+ procedural families only (97,001 rows) & 65.03 & 61.7 & $-$0.5 {[}$-$1.2, +0.2{]} & 75.8 / 66.3 / 67.0 & 28.3 \\
+ benchmark-source families only (143,157 rows) & 65.04 & 61.8 & +1.9 {[}+1.1, +2.6{]} \textsuperscript{f} & 61.2 / 62.7 / 57.2 & 26.4 \\
+ six weak-area training sets only (117,167 rows) & 65.14 & 64.4 \textsuperscript{f} & $-$1.5 {[}$-$2.3, $-$0.9{]} \textsuperscript{f} & 59.0 / 62.5 / 58.0 & 34.1 \\
final recipe without its 13,776 rows of VAST & 64.77 & 61.6 & $-$0.3 {[}$-$0.8, +0.3{]} & 58.7 / 65.2 / 56.5 & 28.9 \\
+ twin-reserved families at all usable rows (121,204), breadth and single-skill files & 65.16 & 65.6 \textsuperscript{f} & $-$1.0 {[}$-$1.7, $-$0.3{]} & 61.7 / 65.2 / 60.2 & 28.1 \\
final recipe with bidirectional prompt attention (Section~\ref{sec:2.4}) & 66.31 & 64.1 & +1.0 {[}+0.2, +1.8{]} & 62.7 / 66.8 / 58.8 & 25.0 \\
all weights from the untrained 4B, 2e-6, breadth and procedural rows only & 40.87 & 55.6 & $-$3.3 {[}$-$4.3, $-$2.2{]} & -- & 27.2 \\
the same with bidirectional prompt attention & 44.76 & 56.3 & $-$0.9 \textsuperscript{b} & -- & -- \\
the same at 5e-6 & 44.71 & 59.2 & $-$2.9 {[}$-$3.9, $-$1.8{]} & -- & 46.4 \\
half blend of the 2e-6 run with the released weights & 49.60 & 61.1 & $-$0.7 {[}$-$1.4, +0.1{]} & -- & 35.8 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{f} in-family: the round trains on the family or the training split of some of these
test sets. \textsuperscript{b} no interval in our record of the run.\par}
\end{table}

\textbf{The public index cannot tell the data rounds apart.} Every adapter round that changes only
the data lies within 0.4 points of the final recipe on the index (64.77 to 65.16 against 64.78), and
three rounds of nearly the same recipe have spanned 0.9. The other measures separate the rounds,
each with a floor of its own: rounds without procedural data move a generated task by $-$2.8 to +3.0
points, and rounds without the arithmetic file lie 3.4 to 5.9 skill points above the final recipe on
the rebuilt GSM8K rows.

\textbf{Each gain sits in the families a group contains.} The full-coverage round is level on the
index and gains 6.0 points on the twins, 15.8, 3.6 and 11.0 on the three generated tasks and 10.3 on
the rebuilt GSM8K rows. The procedural families alone give 14.3, 3.1 and 9.8 points on the generated
tasks and nothing on the twins. Two of the three added procedural families, multi-hop answerability
and the validation of a call against a schema, are of the kind that answerable facts and tool-call
validity test, and those two tasks gain most: the gain is on the kind of task the families teach,
and transfer has to be read on generated tasks of new kinds. The benchmark-source families give
nothing on either. The round with the twin-reserved families gains 4.0 on the twins, and every
adapter round without twin data stays within 0.2 of the final recipe there. The weak-area files give
11.1 skill points on the rebuilt GSM8K rows through their arithmetic part.

\textbf{On reused test sets the gain is exposure.} The benchmark-source families hold the families
of 18 of the 35 reused tasks (preference and judging sets, safety and injection sets, FOLIO, PAWS,
AmbigQA, two legal sets and a vulnerable-code set), and 16 tasks belong to families that no file of
these rounds holds. The round on those families gives +8.6 on its 18 tasks (interval +7.1 to +10.1)
and +0.3 on the 16 others ($-$0.7 to +1.3). The full-coverage round gives +9.0 (+7.3 to +10.5) and
$-$1.3 ($-$2.5 to 0.0). The weak-area round, which holds none of the 18 families, gives $-$5.7 on
them ($-$7.1 to $-$4.5) and $-$0.8 on the 16 ($-$1.8 to +0.3). No group of data raised a reused task
whose family it does not contain. The items are unseen in every case, so for these checkpoints the
18 tasks measure exposure to a family, and it is worth about nine points. A round can be expected to
raise the private tests of the next index edition only where its data hold their families.

\textbf{Bidirectional attention over the prompt raises every measure without new data.} With the
data, the adapter and the start of the final recipe, switching the attention layers to bidirectional
attention over the prompt raises the index from 64.78 to 66.31 (knowledge 45.4 $\rightarrow$ 47.2,
language 69.4 $\rightarrow$ 70.7, retrieval 69.9 $\rightarrow$ 71.9, tools 86.0 $\rightarrow$ 87.3,
arts 53.9 $\rightarrow$ 54.8), the twins from 61.6 to 64.1, the reused tasks by 1.0 points (interval
+0.2 to +1.8) and the three generated tasks by 1.2 to 3.6 points. It is the first change in these
ablations that raises the reused tasks without adding data. From the untrained model it raises the
index from 40.87 to 44.76, with tools at 68.4 instead of 56.9, and the reused tasks from $-$3.3 to
$-$0.9 against the final recipe. Each is one run, and the index move of the first is larger than the
0.9 that three rounds of nearly the same recipe have spanned, but it has to be read against a repeat
of the final recipe \todo[TODO(r6\_4b\_kr20r2)]{spread between two runs of the final recipe on the
measures of Table 3}.

\subsection{What did not work}\label{sec:4.4}

\emph{Training from the untrained model with the settings of the leading entries.} At 2e-6 the run
scores 40.87 on the index and at 5e-6 44.71, below the released weights (52.76), and it is 3.3 and
2.9 points below the final recipe on the reused tasks. A half blend with the released weights does
not recover it (49.60). This is one size and one data set, and the leading entries train at 27B. One
number points elsewhere: at 5e-6 the run has the highest skill on the rebuilt GSM8K rows of any 4B
checkpoint, 46.4. Its data hold no GSM8K row in the old layout, while the same procedural families
added to the final-recipe mix, which keeps those rows, reach 28.3. We read this as a sign that the
old rows teach the model to answer from the layout of the options.

\emph{More rows of the same families.} The twin-reserved families at all usable rows, 1.7 times as
many as with at most 3,000 rows per task, give 65.6 on the twins against 65.7 with the cap.

\emph{Data of the ``same'' skill with other labels.} Three of the four sources of the weak-area
sarcasm file take their label from a mark the writer set (a hashtag, ``/s'' on Reddit) or from the
site that published a headline. In that round the sarcasm twin is at 34.6 against 39.2 for the
released weights. An earlier round with other stance and irony data sets from the task collection
had lowered the stance twin from 44.9 to 36.9 and the sarcasm twin to 32.6.

\emph{Removing a suspected source of a bias.} Our checkpoints lean towards the answer ``none'' on
the stance twin, and VAST, a stance set in the final recipe, was the suspect. Without its 13,776
rows the index, the twins and the reused tasks do not move, and the stance twin falls from 38.7 to
29.5. When the target is not named in the text, the untrained 4B already answers ``none'' 65\% of
the time: the bias is older than our training.

\emph{Breadth rows alone.} A round on 642,628 rows from 343 task families with the core of the
release mix and no file aimed at the index stays where the released 4B is: +0.7 on the index, $-$0.6
on the reused tasks (interval $-$1.4 to +0.1), 0.0 on the generated tasks.

\subsection{The recipe as it stands}\label{sec:4.5}

The recipe for the next checkpoints has three steps. Start from the released weights. Train one data
round on the final-recipe mix with the full-coverage data, which holds neither sarcasm file, and
with four hygiene repairs: the GSM8K rows of the old layout removed and 1,452 clean GSM8K training
problems added in the rebuilt layout, ANLI cut to 8,000 rows with balanced labels, select-all rows
capped at 15,000 per family with the EuroVoc cases of fewer than two correct options removed, and 45
groups of rows dropped that the current leak scan flags \todo[TODO(r6\_4b\_kr28h)]{result of the
hygiene repairs on the final-recipe mix}. Then run the reasoning stages of Chapter~\ref{sec:5}.
Bidirectional attention over the prompt is the candidate for a fourth step, once the repeat of the
final recipe and the larger runs are in. A checkpoint of this recipe is in-family on the twins and
on 18 reused tasks, so its transfer has to be read on generated tasks. No 27B round is trained
before the recipe is settled at 4B.

Six questions were open when this was written, each with rounds running or queued at 4B unless
stated:

\begin{itemize}
\item bidirectional attention over the prompt at the size of the full-coverage round and in the first
stage of the release recipe \todo[TODO(r6\_4b\_kr23ebi, s1\_4b\_bi, r6\_4b\_kr23es1bi)]{the larger
runs with bidirectional prompt attention}
\item contrast pairs for stance and sarcasm written by other language models, in two versions (16,036
rows, and 8,859 rows filtered against surface cues) \todo[TODO(r6\_4b\_kr29d, r6\_4b\_kr29c)]{rounds
with the two contrast-pair files}
\item large files from the original training splits of the twin sources and their relatives (368,053 rows
from Corr2Cause, ProofWriter, VitaminC, WANLI and others), in-family on several twins
\todo[TODO(r6\_4b\_kr27b)]{round with the large original-source files}
\item ten families of the public procedural corpus from which the leading entry's procedural rows come,
9,000 rows each \todo[TODO(r6\_4b\_kr28p)]{round with the public procedural corpus}
\item a second run of the final recipe, for the spread between two runs on the measures of
Table~\ref{tab:3} \todo[TODO(r6\_4b\_kr20r2)]{repeat of the final-recipe round}
\item the full-coverage round at 9B \todo[TODO(r6\_9b\_kr23e)]{full-coverage round at 9B}
\end{itemize}


==> sections/05_reasoning.tex <==
\clearpage
\section{Reasoning}\label{sec:5}

A decision model answers from one forward pass, but some answers have to be worked out. This chapter
shows that decision training damages the ability to finish a line of reasoning, describes the three
stages that restore it in the same weights, measures where a thought helps and where it hurts, and
reports what reinforcement learning adds. In short: the repaired models gain 1.9 to 2.9 index points
with reasoning and far more where an answer is computed, and reinforcement learning makes thoughts
end and shortens them without making the answers better.

\subsection{Decision training breaks the end of a thought}\label{sec:5.1}

After the data rounds the models fail in two ways when they are asked to reason. On 5,710 diagnostic
items the 4B and the 27B close the thought at once: 42.4\% and 43.6\% of their thoughts are shorter
than 40 tokens. The 9B does the opposite: only 29.8\% of its thoughts end, and the median thought
runs to the 4,096-token limit with the answer letter repeated to the end.

To locate the damage we measure the probability that a model closes a thought at a point where the
thought is complete. A stored thought is fed to a model with the item's prompt, and we read the
probability that the closing tag follows within two tokens. The points are the natural ends of
thoughts that their writer closed, and control points inside the thoughts have a median of 0.00 for
every model. Every stage of a size reads the same thoughts, so differences are differences between
stages (Figure~\ref{fig:3}).

\begin{figure}[!htbp]
\renewcommand{\thefigure}{3}
\centering
\adjincludegraphics[max width=\linewidth,max height=0.5\textheight]{figures/fig10_closing.pdf}
\caption{Where the end of a thought is lost. (a--c) Probability of closing a thought at its natural end for every training stage of the 4B, 9B and 27B lines (median over thoughts and 95\% bootstrap interval, with circles for thoughts written by the base model and triangles for thoughts written by the replayed model). (d) Share of thoughts that end by themselves when each 4B stage writes its own thoughts on the same 3,021 held-out items (4,096-token limit, no loop detector).}\label{fig:3}
\end{figure}

A stage with a loss on the answer letter alone leaves the closing decision unsupervised, and it can
drift. At 9B the data rounds take the closing probability from 0.54 to 0.06. At 4B they leave it
where the base model has it (0.52), and the reader round that follows thinking replay takes it from
0.73 to 0.26. At 27B the same round takes it from 0.97 to 0.54. The one stage with a loss on the
closing tag, thinking replay, restores it at every size (0.73, 0.81 and 0.97). A longer limit does
not help: at 16,384 tokens 87.4\% of the 4B's thoughts are still running, 80.8\% of all thoughts are
in a loop, and the accuracy is unchanged at 3.9 times the tokens. Inside a loop no model closes the
thought, the base model included, so once a text repeats, the repetition sustains itself.

\subsection{Three stages that repair it}\label{sec:5.2}

\emph{Thinking replay} gives the decision model back the reasoning of the model it was trained from.
The starting model of the same size writes several thoughts for each training item, and the best one
that ended by itself and raised the decision model's answer is kept as a target (15,870 targets at
4B, 16,369 at 9B and 4,395 at 27B). The decision model is trained on these targets with a
language-model loss on the thought and its closing tag. At inference there is one model. The
\emph{reader round} then trains the answer that is read after a thought the model wrote itself, with
rows of the item and its own thought labelled by the item's gold answer, and holds the one-pass
answer in place with rows whose target is the earlier one-pass distribution. The \emph{stop step}
teaches the end. The model writes four thoughts for each of 14,911 items, its answer is read after
every eighth of each thought, and a thought counts as finished at the first eighth after which the
answer no longer changes. The best sample per item, cut at that point and closed, becomes a target
(5,311 targets with a mean of 555 tokens), and the model is trained on them for 82 steps at 4B.

\begin{table}[!htbp]
\renewcommand{\thetable}{4}
\centering
\caption{Decision Index 0.2.1 with reasoning after each stage (default threshold 0.9, own runs, one run each). Tokens: reasoning tokens per answer, averaged over all answers including those not thought about. At the limit: share of thoughts that reach the 4,096-token budget.}\label{tab:4}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrll}
\toprule
\textbf{size} & {\begin{tabular}[b]{@{}r@{}}\textbf{one}\\\textbf{pass}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{reader}\\\textbf{round only}\end{tabular}} & \textbf{replay, then reader round} & \textbf{+ stop step} \\
\midrule
4B & 64.78 & 66.38 & 67.72 (1,144 tokens, 57.5\% at the limit) & 67.37 (497 tokens, 10.4\%) \\
9B & 67.75 & 69.32 & 69.77 (1,049 tokens, 62.9\%) & \textbf{70.16} (552 tokens, 15.8\%) \\
27B & 70.43 & 70.89 and 71.12 \textsuperscript{a} & \textbf{72.34} (193 tokens, 6.0\%) & -- \textsuperscript{b} \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{a} two variants of the reader round on the final data round. \textsuperscript{b}
not needed at this size.\par}
\end{table}

Replay before the reader round adds 1.3 index points at 4B, 0.5 at 9B and 1.2 to 1.5 at 27B, almost
all in the knowledge and reasoning area (45.4 $\rightarrow$ 57.0 at 4B, 55.1 $\rightarrow$ 62.9 at
27B), and code execution rises from 28.7 to 80.5 skill points at 4B. The price at 4B and 9B is
thoughts that run to the limit. The stop step removes most of it (Table~\ref{tab:4}): on 3,021
held-out items routed to reasoning, 85.9\% of the 4B's thoughts end by themselves instead of 11.4\%,
at 1,413 instead of 3,764 tokens, with the default answer at 75.31 against 75.54 (difference
$-$0.23, interval $-$0.96 to +0.50). On the index the 4B keeps 67.37 of 67.72 with 43\% of the
reasoning tokens, and the 9B rises to 70.16 with 53\% of them. The 27B needs no stop step. Two
alternatives fall short of the sequence: one joint stage with thinking and read-out targets scores
67.11, and the base model writing thoughts for our model to read scores 67.62 at 438 reasoning
tokens per answer.

\subsection{Where a thought helps and where it hurts}\label{sec:5.3}

On the index a thought adds two to three points. Where the answer has to be computed it decides the
result (Table~\ref{tab:5}). On GSM8K rows rebuilt so that the options give nothing away, our models
have a one-pass skill of 25 to 52 and reach 92 to 99 after a thought. On three procedural tasks of
our benchmark the 27B goes from 0.758, 0.608 and 0.743 to 1.000, 0.993 and 0.985 in accuracy, and on
the harder versions of three generated tasks from 0.780 to 0.984, where the strongest one-pass entry
of the board has 0.866.

\begin{table}[!htbp]
\renewcommand{\thetable}{5}
\centering
\caption{What a thought is worth (own runs, 5 to 7 October 2026, one run each, 4,096-token limit). Index: Decision Index 0.2.1 with the gate at 0.9. GSM8K: the rows rebuilt for edition 0.3, a thought on every item, chance-corrected skill (mean of the benchmark's two tracks). Benchmark tasks: 6,019 items of ten tasks of our benchmark, a thought on every item, accuracy. Harder generated tasks: 1,800 items of three tasks, measured in the same way. ``Starting model'': the untrained model a size was built from, writing its own thought.}\label{tab:5}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.2305}}>{\raggedright\arraybackslash}p{\mdw{0.1984}}>{\raggedleft\arraybackslash}p{\mdw{0.1295}}>{\raggedleft\arraybackslash}p{\mdw{0.1428}}>{\raggedleft\arraybackslash}p{\mdw{0.1390}}>{\raggedleft\arraybackslash}p{\mdw{0.1467}}}
\toprule
\textbf{measure} & \textbf{model} & \textbf{one pass} & \textbf{after the thought} & \textbf{default answer} & \textbf{tokens per thought} \\
\midrule
index (points) & 4B, after the stop step & 64.78 & -- & 67.37 & 1,585 \\
 & 9B, after the stop step & 67.75 & -- & 70.16 & 1,900 \\
 & 27B, after replay and reader round & 70.43 & -- & 72.34 & 710 \\
rebuilt GSM8K (skill) & 4B starting model & 10.9 & 97.1 & 97.1 & 261--290 \\
 & 4B, after the stop step & 25.4 & 94.4 & 93.8 & 620--720 \\
 & 9B starting model & 18.3 & 98.6 & 98.5 & -- \\
 & 9B, after the stop step & 33.8 & 96.3 & 94.6 & 613--741 \\
 & 27B, after replay and reader round & 52.3 & 98.9 & 98.3 & -- \\
ten benchmark tasks (accuracy) & 4B / 9B / 27B & 0.709 / 0.735 / 0.836 & 0.876 / 0.880 / 0.948 & 0.855 / 0.862 / 0.930 & 1,687 / 1,909 / 567 \\
three harder generated tasks (accuracy) & 4B / 9B / 27B & 0.602 / 0.627 / 0.780 & 0.843 / 0.892 / 0.984 & 0.802 / 0.834 / 0.941 & 1,616 / 1,710 / 405 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

The starting models still think better on arithmetic than ours: the untrained 4B reaches 97.1 after
a thought and ours 94.4, with thoughts of 261 to 290 tokens of which 99.3 to 99.8\% end. Decision
training costs reasoning quality, and the three stages do not return all of it. A thought also
hurts. On held-out items of the training distribution the answer after a thought is worse than the
one-pass answer in 7 of 21 task families, most on select-all questions ($-$7.0), ANLI ($-$4.8) and
ContractNLI ($-$2.4). At 27B the home-appliance simulator (100.0 $\rightarrow$ 94.3), SATA-Bench
(59.0 $\rightarrow$ 55.0), MuSR (72.5 $\rightarrow$ 68.9) and the Habermas set (63.7 $\rightarrow$
60.3) lose with reasoning.

Where an answer is computed, the default answer gives part of the gain away: on the harder generated
tasks the 27B is right on 98.4\% of the items after the thought and on 94.1\% with the default
answer. The gate does not send a confidently wrong one-pass answer to reasoning, and the mixture
keeps half of a one-pass read-out that is near chance on such items. The other settings are where we
left them for good reasons. A limit of 8,192 tokens scores 67.52 against 67.72 at 4,096, and a gate
at 0.7, free on held-out items, costs half a point on the index (67.20). No rule that sets the
weight of the thought from the one-pass confidence beats the flat 0.5 / 0.5 mixture on held-out
items (90.12 at 4B, 92.96 at 9B).

\subsection{Reinforcement learning}\label{sec:5.4}

We also trained the thinker with a group-relative policy gradient. In one iteration the model writes
8 thoughts for each of 64 prompts, the answer is read after each, and a thought is reinforced by how
far its reward lies above that of the other thoughts for the same prompt. The reward is the gain of
the answer after the thought over the one-pass answer, measured with the log score or with a bounded
proper score, minus a price of 1e-4 per token. The prompts come from 26,931 items whose one-pass top
probability is below 0.9, mostly causal questions, code execution, chess, narrative reasoning and
generated arithmetic and rule tasks, on which the thought does change the answer. Table~\ref{tab:6}
has the arms on 3,021 held-out items.

\begin{table}[!htbp]
\renewcommand{\thetable}{6}
\centering
\caption{Reinforcement learning of the thinker on 3,021 routed held-out items of the training distribution (one thought per item with the decoding of inference, 4,096-token limit, accuracy in percent). Rollouts: sampled at temperature 1, or as at inference (temperature 0.6, top-p 0.95, top-k 20). Last column: paired difference to the arm's starting model with its 95\% interval, for the answer after the thought (T) and the default answer (D), on the test part of the items for the arms that start from a stop-trained model (2,132 test items at 4B).}\label{tab:6}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.1628}}>{\raggedright\arraybackslash}p{\mdw{0.1218}}>{\raggedleft\arraybackslash}p{\mdw{0.2204}}>{\raggedleft\arraybackslash}p{\mdw{0.1218}}>{\raggedleft\arraybackslash}p{\mdw{0.1170}}>{\raggedleft\arraybackslash}p{\mdw{0.1039}}>{\raggedleft\arraybackslash}p{\mdw{0.1395}}}
\toprule
\textbf{start and arm} & \textbf{rollouts} & \textbf{thoughts that end} & \textbf{tokens per thought} & \textbf{after the thought} & \textbf{default answer} & \textbf{difference to the start} \\
\midrule
4B after the data rounds (start) & -- & 92.4\% & 639 & 72.29 & 74.02 & -- \\
\ldots{} log score & temperature 1 & 97.6\% (66.3\% closed at once) & 255 & 74.25 & 75.41 & T +1.95 {[}+0.73, +3.21{]} \\
4B after the stop step (start) & -- & 85.9\% & 1,413 & 74.38 & 75.31 & -- \\
\ldots{} bounded proper score & as at inference & 99.7\% & 503 & 74.11 & 75.07 & T $-$1.17 {[}$-$2.11, $-$0.28{]} \\
\ldots{} control: accuracy reward & as at inference & 99.8\% & 433 & 73.78 & 74.71 & T $-$1.64 {[}$-$2.67, $-$0.66{]} \\
\ldots{} control: no price for length & as at inference & 59.4\% & 2,581 & 74.58 & 75.50 & T $-$0.70 {[}$-$1.69, +0.19{]} \\
\ldots{} control: noise as reward & temperature 1 & 99.2\% & 600 & 73.68 & 74.08 & T $-$1.22 {[}$-$2.25, $-$0.14{]} \\
4B after replay and reader round (start) & -- & 11.4\% & 3,764 & 75.04 & 75.54 & -- \\
\ldots{} bounded proper score & as at inference & 58.0\% & 2,753 & 74.18 & 74.94 & T $-$0.86 {[}$-$1.82, +0.03{]} \\
9B after the stop step (start) & -- & 77.7\% & 1,677 & 81.20 & 82.06 & -- \\
\ldots{} bounded proper score & as at inference & 99.8\% & 544 & 80.87 & 81.60 & D $-$0.75 {[}$-$1.27, $-$0.14{]} \\
\ldots{} control: accuracy reward & as at inference & \todo[TODO(rl9\_ei2\_acc\_t06)]{held-out result of the accuracy-reward control at 9B} &  &  &  &  \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\textbf{Started from a model that hardly reasons, the policy learns to skip.} From the data-round
4B, two thirds of the thoughts are closed at once. Its answers improve over that start, but what it
learned is where to skip, not how to reason: on the index it scores 67.18 with 57 reasoning tokens
per answer, and 78.5\% of its thoughts there have fewer than 16 tokens. We do not count it as a
model that reasons.

\textbf{Started from a model that reasons, it makes thoughts end and shortens them.} From the
stop-trained model, with rollouts sampled as at inference, 99.7\% of the 4B's thoughts end at 503
tokens instead of 1,413, and 99.8\% of the 9B's at 544 instead of 1,677, at an accuracy within a
third of a point of the start on all held-out items. On the index the two models lose 0.57 and 0.64
points (66.80 against 67.37, 69.52 against 70.16, one run each).

\textbf{Calibration follows the length of the thought.} Read before any temperature is fitted, the
answer after the thought of the stop-trained 4B is overconfident (calibration error 9.48 on the test
items). After training with the proper score it is 6.93. Two controls separate the factors. With the
accuracy of the answer as reward and the same price, the thoughts are as short and the error falls
to 7.79. With the proper score and no price, the thoughts grow to 2,581 tokens, 40.6\% of them reach
the limit, and the error rises to 11.19, above the start. The price shortens the thoughts, the
shorter thoughts make the answer after them less overconfident, and the proper score lowers the
error by a further 0.9 points in one run. \citet{gao2026openjev} report a much larger effect of the
reward for their 1.7B model (fitted temperature 1.4 against 7.2), with a correctness-reward arm that
has no length price, the factor that does the work here. The training does not improve the ranking
of right and wrong answers: the share of answers that can be accepted at an error of 5\% is 20.5\%
before and 18.0\% after at 4B. Started from the model after replay and reader round, without the
stop step, the same training ends only 58.0\% of the thoughts. Its answer after a thought is close
to calibrated (error 2.81), but the one-pass answer of the same weights becomes under-confident
(stated 62.3 at an accuracy of 71.2), which sends more questions to a thought.

No arm has raised accuracy over the supervised stages on any evaluation. A noise reward comes within
half a point to a point of the real one, and on the rebuilt GSM8K rows the 4B reaches 92.2 after the
thought against 94.4 before. Second runs of the two 4B arms were queued when this was written
\todo[TODO(rl4\_ei2\_dw\_t06\_s1, rl4\_ei2\_acc\_t06\_s1)]{second runs of the proper-score and the
accuracy-reward arm at 4B}.


==> sections/05_think.tex <==
\section{StartLux-Decision-Think: reasoning in the same weights}\label{sec:5}

Some answers have to be worked out, and a model trained to answer from one position loses the
ability to finish a line of reasoning. The -Think checkpoints get it back in the same weights, write
a thought only when the one-pass answer is unsure (Section~\ref{sec:2.2}), and gain two to three
index points with it, far more where an answer is computed (Table~\ref{tab:10}).

\subsection{Main results}\label{sec:5.1}

On Decision Index 0.2.1, in own runs of 5 to 7 October 2026 and in-domain for most benchmarks, the
-Think checkpoints gain 1.9 to 2.9 index points over one pass, almost all in the knowledge and
reasoning area: 72.34 at 27B, 69.77 at 9B and 67.72 at 4B, and 70.16 and 67.37 for the 9B and the 4B
after the stop step. Where the answer has to be computed a thought decides the result. On GSM8K rows
rebuilt so that the options give nothing away, our models have a one-pass skill of 25 to 52 and
reach 92 to 99 after a thought. On three procedural tasks of our benchmark
StartLux-Decision-27B-Think goes from 0.758, 0.608 and 0.743 to 1.000, 0.993 and 0.985 in accuracy,
and on the harder versions of three generated tasks from 0.780 to 0.984, where the strongest
one-pass entry of the board has 0.866. We trail in two places. The untrained starting models still
think better on arithmetic than ours (97.1 against 94.4 at 4B), we think because decision training
costs reasoning quality that the three stages do not fully return. And on NLI-like and select-all
questions a thought lowers accuracy.

\begin{table}[!htbp]
\renewcommand{\thetable}{10}
\centering
\caption{A thought adds two to three index points and decides the tasks whose answer has to be computed (own runs, 5 to 7 October 2026, one run each, 4,096-token limit). Index: Decision Index 0.2.1 with the gate at 0.9. GSM8K: the rows rebuilt for edition 0.3, a thought on every item, chance-corrected skill (mean of the benchmark's two tracks). Benchmark tasks: 6,019 items of ten tasks of our benchmark, a thought on every item, accuracy. Harder generated tasks: 1,800 items of three tasks, measured in the same way. ``Starting model'': the untrained model a size was built from, writing its own thought.}\label{tab:10}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.2473}}>{\raggedright\arraybackslash}p{\mdw{0.1506}}>{\raggedleft\arraybackslash}p{\mdw{0.1386}}>{\raggedleft\arraybackslash}p{\mdw{0.1497}}>{\raggedleft\arraybackslash}p{\mdw{0.1466}}>{\raggedleft\arraybackslash}p{\mdw{0.1541}}}
\toprule
\textbf{measure} & \textbf{model} & \textbf{one pass} & \textbf{after the thought} & \textbf{default answer} & \textbf{tokens per thought} \\
\midrule
index (points) & 4B-Think + stop step & 64.78 & -- & 67.37 & 1,585 \\
 & 9B-Think + stop step & 67.75 & -- & 70.16 & 1,900 \\
 & 27B-Think & 70.43 & -- & 72.34 & 710 \\
rebuilt GSM8K (skill) & 4B starting model & 10.9 & 97.1 & 97.1 & 261--290 \\
 & 4B-Think + stop step & 25.4 & 94.4 & 93.8 & 620--720 \\
 & 9B starting model & 18.3 & 98.6 & 98.5 & -- \\
 & 9B-Think + stop step & 33.8 & 96.3 & 94.6 & 613--741 \\
 & 27B-Think & 52.3 & 98.9 & 98.3 & -- \\
ten benchmark tasks (accuracy) & 4B / 9B / 27B & 0.709 / 0.735 / 0.836 & 0.876 / 0.880 / 0.948 & 0.855 / 0.862 / 0.930 & 1,687 / 1,909 / 567 \\
three harder generated tasks (accuracy) & 4B / 9B / 27B & 0.602 / 0.627 / 0.780 & 0.843 / 0.892 / 0.984 & 0.802 / 0.834 / 0.941 & 1,616 / 1,710 / 405 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

The starting models still think better on arithmetic than ours: the untrained 4B reaches 97.1 after
a thought and ours 94.4, with thoughts of 261 to 290 tokens of which 99.3 to 99.8\% end. Decision
training costs reasoning quality, and the three stages do not return all of it. A thought also
hurts. On held-out items of the training distribution the answer after a thought is worse than the
one-pass answer in 7 of 21 task families, most on select-all questions ($-$7.0), ANLI ($-$4.8) and
ContractNLI ($-$2.4). At 27B the home-appliance simulator (100.0 $\rightarrow$ 94.3), SATA-Bench
(59.0 $\rightarrow$ 55.0), MuSR (72.5 $\rightarrow$ 68.9) and the Habermas set (63.7 $\rightarrow$
60.3) lose with reasoning.

Where an answer is computed, the default answer gives part of the gain away: on the harder generated
tasks the 27B is right on 98.4\% of the items after the thought and on 94.1\% with the default
answer. The gate does not send a confidently wrong one-pass answer to reasoning, and the mixture
keeps half of a one-pass read-out that is near chance on such items. The other settings are where we
left them for good reasons. A limit of 8,192 tokens scores 67.52 against 67.72 at 4,096, and a gate
at 0.7, free on held-out items, costs half a point on the index (67.20). No rule that sets the
weight of the thought from the one-pass confidence beats the flat 0.5 / 0.5 mixture on held-out
items (90.12 at 4B, 92.96 at 9B).

\subsection{Diagnosis: decision training breaks the end of a thought}\label{sec:5.2}

After the data round the models fail in two ways when they are asked to reason. On 5,710 diagnostic
items the 4B and the 27B close the thought at once: 42.4\% and 43.6\% of their thoughts are shorter
than 40 tokens. The 9B does the opposite: only 29.8\% of its thoughts end, and the median thought
runs to the 4,096-token limit with the answer letter repeated to the end.

To locate the damage we measure the probability that a model closes a thought at a point where the
thought is complete. A stored thought is fed to a model with the item's prompt, and we read the
probability that the closing tag follows within two tokens. The points are the natural ends of
thoughts that their writer closed, and control points inside the thoughts have a median of 0.00 for
every model. Every stage of a size reads the same thoughts, so differences are differences between
stages (Figure~\ref{fig:3}).

\begin{figure}[!htbp]
\renewcommand{\thefigure}{3}
\centering
\adjincludegraphics[max width=\linewidth,max height=0.5\textheight]{figures/fig10_closing.pdf}
\caption{The probability of closing a finished thought falls in stages with a loss on the answer alone and returns in the one stage with a loss on the closing tag. (a--c) Probability of closing a thought at its natural end for every training stage of the 4B, 9B and 27B lines (median over thoughts and 95\% bootstrap interval, with circles for thoughts written by the base model and triangles for thoughts written by the replayed model). (d) Share of thoughts that end by themselves when each 4B stage writes its own thoughts on the same 3,021 held-out items (4,096-token limit, no loop detector).}\label{fig:3}
\end{figure}

A stage with a loss on the answer letter alone leaves the closing decision unsupervised, and it can
drift. At 9B the data rounds take the closing probability from 0.54 to 0.06. At 4B they leave it
where the base model has it (0.52), and the reader round that follows thinking replay takes it from
0.73 to 0.26. At 27B the same round takes it from 0.97 to 0.54. The one stage with a loss on the
closing tag, thinking replay, restores it at every size (0.73, 0.81 and 0.97). A longer limit does
not help: at 16,384 tokens 87.4\% of the 4B's thoughts are still running, 80.8\% of all thoughts are
in a loop, and the accuracy is unchanged at 3.9 times the tokens. Inside a loop no model closes the
thought, the base model included, so once a text repeats, the repetition sustains itself.

\subsection{Three stages that repair it}\label{sec:5.3}

\emph{Thinking replay} gives the decision model back the reasoning of the model it was trained from.
The starting model of the same size writes several thoughts for each training item, and the best one
that ended by itself and raised the decision model's answer becomes a target in Lux-Think (15,870
targets at 4B, 16,369 at 9B and 4,395 at 27B). The model is trained on these targets with a
language-model loss on the thought and its closing tag, so at inference there is one model. Replay
alone ends 74.6\% of the 4B's thoughts on held-out items, but it moves the one-pass answer by two to
five points.

The \emph{reader round} returns it. It trains the answer that is read after a thought the model
wrote itself, with rows of the item and its own thought labelled by the item's gold answer, and
holds the one-pass answer in place with rows whose target is the earlier one-pass distribution.
Replay and reader round give the -Think checkpoints. Replay adds 1.3 index points at 4B, 0.5 at 9B
and 1.2 to 1.5 at 27B over the reader round alone, almost all in knowledge and reasoning (45.4
$\rightarrow$ 57.0 at 4B, 55.1 $\rightarrow$ 62.9 at 27B), and code execution rises from 28.7 to
80.5 skill points at 4B. The price at 4B and 9B is that the reader round takes the end away again:
57.5\% and 62.9\% of the thoughts reach the budget.

The \emph{stop step} teaches the end from the model's own thoughts. The model writes four thoughts
for each of 14,911 items, its answer is read after every eighth of each thought, and a thought
counts as finished at the first eighth after which the answer no longer changes. The best sample per
item, cut at that point and closed, becomes a target (5,311 targets with a mean of 555 tokens), and
the model is trained on them for 82 steps at 4B. On 3,021 held-out items routed to reasoning, 85.9\%
of the 4B's thoughts then end by themselves instead of 11.4\%, at 1,413 instead of 3,764 tokens,
with the default answer at 75.31 against 75.54 (difference $-$0.23, interval $-$0.96 to +0.50). On
the index the 4B keeps 67.37 of 67.72 with 43\% of the reasoning tokens, and the 9B rises to 70.16
with 53\% of them. The 27B needs no stop step. Two alternatives fall short of the sequence: one
joint stage with thinking and read-out targets scores 67.11 at 4B, and the base model writing
thoughts for our model to read scores 67.62 at 438 reasoning tokens per answer.

On the final recipe (Section~\ref{sec:4.7}) the three stages run with bidirectional attention over
the prompt and causal attention over the thought, the attention the data round was trained with. The
4B then scores 68.33 on the index after replay and reader round, with 1,032 reasoning tokens per
question, and 67.99 after the stop step, with 478. The causal sequence on the -Rounds model scores
67.72 and 67.37 at similar costs. On the 3,021 held-out items 91.3\% of the thoughts end by
themselves after the stop step, at a median of 824 tokens, and the default answer is 75.80 (75.07
for the causal stop step). The 8.7\% that reach the limit are the hard items: their one-pass
accuracy is 55.0 against 74.2 for the rest, and the thought does not change it. A reader round that
also trains the closing tag, with no loss on the thought itself, collapses every thought to a single
token and lowers the default answer to 72.62. The end needs the text before it as a target, which
the stop step provides.

\subsection{Where a thought helps and where it hurts}\label{sec:5.4}

The starting models still think better on arithmetic than ours: the untrained 4B reaches 97.1 after
a thought and ours 94.4, with thoughts of 261 to 290 tokens of which 99.3 to 99.8\% end
(Table~\ref{tab:10}). Decision training costs reasoning quality, and the three stages do not return
all of it. A thought also hurts. On held-out items of the training distribution the answer after a
thought is worse than the one-pass answer in 7 of 21 task families, most on select-all questions
($-$7.0), ANLI ($-$4.8) and ContractNLI ($-$2.4). At 27B the home-appliance simulator (100.0
$\rightarrow$ 94.3), SATA-Bench (59.0 $\rightarrow$ 55.0), MuSR (72.5 $\rightarrow$ 68.9) and the
Habermas set (63.7 $\rightarrow$ 60.3) lose with reasoning.

Where an answer is computed, the default answer gives part of the gain away: on the harder generated
tasks the 27B is right on 98.4\% of the items after the thought and on 94.1\% with the default
answer. The gate does not send a confidently wrong one-pass answer to reasoning, and the mixture
keeps half of a one-pass read-out that is near chance on such items. The other settings stay where
they are for reasons we measured. A limit of 8,192 tokens scores 67.52 against 67.72 at 4,096, a
gate at 0.7, free on held-out items, costs half a point on the index (67.20), and no rule that sets
the weight of the thought from the one-pass confidence beats the flat 0.5 / 0.5 mixture on held-out
items (90.12 at 4B, 92.96 at 9B). Appendix~\ref{sec:F} has the measurements behind these settings.

\subsection{Reinforcement learning}\label{sec:5.5}

We also trained the thinker with a group-relative policy gradient. In one iteration the model writes
8 thoughts for each of 64 prompts, the answer is read after each, and a thought is reinforced by how
far its reward lies above that of the other thoughts for the same prompt. The reward is the gain of
the answer after the thought over the one-pass answer, measured with the log score or with a bounded
proper score, minus a price of 1e-4 per token. The prompts come from 26,931 items whose one-pass top
probability is below 0.9, mostly causal questions, code execution, chess, narrative reasoning and
generated arithmetic and rule tasks, on which the thought does change the answer. Table~\ref{tab:11}
has the arms on 3,021 held-out items. The first arms used a learning rate of 1e-5, a penalty of 0.02
towards the starting policy and 120 iterations, and each further arm changes one thing against an
earlier one: the start, the outcome term, the price or the sampling of the rollouts. Each row is one
run, and three repeats of one arm spread by about $\pm$0.3 points on these items.

\begin{table}[!htbp]
\renewcommand{\thetable}{11}
\centering
\caption{With a price for length, reinforcement learning makes nearly every thought end at about a third of the tokens, and no arm that starts from a model that reasons beats its start. Reinforcement learning of the thinker on 3,021 routed held-out items of the training distribution (one thought per item with the decoding of inference, 4,096-token limit, accuracy in percent). Rollouts: sampled at temperature 1, or as at inference (temperature 0.6, top-p 0.95, top-k 20). Last column: paired difference to the arm's starting model with its 95\% interval, for the answer after the thought (T) and the default answer (D), on the test part of the items for the arms that start from a stop-trained model (2,132 test items at 4B).}\label{tab:11}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.2054}}>{\raggedright\arraybackslash}p{\mdw{0.1228}}>{\raggedleft\arraybackslash}p{\mdw{0.1540}}>{\raggedleft\arraybackslash}p{\mdw{0.1281}}>{\raggedleft\arraybackslash}p{\mdw{0.1223}}>{\raggedleft\arraybackslash}p{\mdw{0.1082}}>{\raggedleft\arraybackslash}p{\mdw{0.1464}}}
\toprule
\textbf{start and arm} & \textbf{rollouts} & \textbf{thoughts that end} & \textbf{tokens per thought} & \textbf{after the thought} & \textbf{default answer} & \textbf{difference to the start} \\
\midrule
\mdourrow StartLux-Decision-4B-Rounds (start) & -- & 92.4\% & 639 & 72.29 & 74.02 & -- \\
\ldots{} log score & temperature 1 & 97.6\% (66.3\% closed at once) & 255 & 74.25 & 75.41 & T +1.95 {[}+0.73, +3.21{]} \\
\mdourrow StartLux-Decision-4B-Think + stop step (start) & -- & 85.9\% & 1,413 & 74.38 & 75.31 & -- \\
\ldots{} bounded proper score & as at inference & 99.7\% & 503 & 74.11 & 75.07 & T $-$1.17 {[}$-$2.11, $-$0.28{]} \\
\ldots{} control: accuracy reward & as at inference & 99.8\% & 433 & 73.78 & 74.71 & T $-$1.64 {[}$-$2.67, $-$0.66{]} \\
\ldots{} control: no price for length & as at inference & 59.4\% & 2,581 & 74.58 & 75.50 & T $-$0.70 {[}$-$1.69, +0.19{]} \\
\ldots{} control: noise as reward & temperature 1 & 99.2\% & 600 & 73.68 & 74.08 & T $-$1.22 {[}$-$2.25, $-$0.14{]} \\
\mdourrow StartLux-Decision-4B-Think (start) & -- & 11.4\% & 3,764 & 75.04 & 75.54 & -- \\
\ldots{} bounded proper score & as at inference & 58.0\% & 2,753 & 74.18 & 74.94 & T $-$0.86 {[}$-$1.82, +0.03{]} \\
\mdourrow StartLux-Decision-9B-Think + stop step (start) & -- & 77.7\% & 1,677 & 81.20 & 82.06 & -- \\
\ldots{} bounded proper score & as at inference & 99.8\% & 544 & 80.87 & 81.60 & D $-$0.75 {[}$-$1.27, $-$0.14{]} \\
\ldots{} control: accuracy reward & as at inference & 99.7\% & 612 & 81.17 & 82.03 & D $-$0.28 {[}$-$0.84, +0.28{]} \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

Started from a model that hardly reasons, the policy learns to skip. From
StartLux-Decision-4B-Rounds, two thirds of the thoughts are closed at once. Its answers improve over
that start, but what it learned is where to skip, not how to reason: on the index it scores 67.18
with 57 reasoning tokens per answer, and 78.5\% of its thoughts there have fewer than 16 tokens. We
do not count it as a model that reasons.

Started from a model that reasons, it makes thoughts end and shortens them. From the -Think
checkpoints after the stop step, with rollouts sampled as at inference, 99.7\% of the 4B's thoughts
end at 503 tokens instead of 1,413, and 99.8\% of the 9B's at 544 instead of 1,677, at an accuracy
within a third of a point of the start on all held-out items. On the index the two models lose 0.57
and 0.64 points (66.80 against 67.37, 69.52 against 70.16, one run each), a loss at the edge of what
one run can show. With the accuracy of the answer as reward and the same price, the 9B ends 99.7\%
of its thoughts at 612 tokens and keeps its accuracy (default answer $-$0.28 points, interval
$-$0.84 to +0.28), and the calibration error of the answer after the thought falls from 3.82 to 2.04
on the test items (1.82 with the proper score).

Calibration follows the length of the thought. Read before any temperature is fitted, the answer
after the thought of StartLux-Decision-4B-Think after the stop step is overconfident (calibration
error 9.48 on the test items). After training with the proper score it is 6.93. Two controls
separate the factors. With the accuracy of the answer as reward and the same price, the thoughts are
as short and the error falls to 7.79. With the proper score and no price, the thoughts grow to 2,581
tokens, 40.6\% of them reach the limit, and the error rises to 11.19, above the start. The price
shortens the thoughts, the shorter thoughts make the answer after them less overconfident, and the
proper score lowers the error by a further 0.9 points in one run. \citet{gao2026openjev} report a
much larger effect of the reward for their 1.7B model (fitted temperature 1.4 against 7.2), with a
correctness-reward arm that has no length price, the factor that does the work here. The training
does not improve the ranking of right and wrong answers: the share of answers that can be accepted
at an error of 5\% is 20.5\% before and 18.0\% after at 4B. Started from the model after replay and
reader round, without the stop step, the same training ends only 58.0\% of the thoughts. Its answer
after a thought is close to calibrated (error 2.81), but the one-pass answer of the same weights
becomes under-confident (stated 62.3 at an accuracy of 71.2), which sends more questions to a
thought.

All arms in this section were trained with a loop whose data-parallel ranks started from different
random adapter weights and averaged their gradients, so only rank 0's adapter was saved and served.
The fix broadcasts rank 0's initial weights once. Corrected runs (the accuracy-reward arm again with
our loop, and a full-parameter run in slime with the same prompts and reward) are under way, and the
conclusions below hold for the arms as trained. \todo[TODO(rl4\_ei2\_acc\_sync,
s4b\_acc\_r1)]{corrected RL results}

No arm has raised accuracy over the supervised stages on any evaluation. A noise reward comes within
half a point to a point of the real one, and on the rebuilt GSM8K rows the 4B reaches 92.2 after the
thought against 94.4 before. A second run of the proper-score arm repeats the picture: every thought
ends, at 491 tokens, the calibration error of the answer after the thought falls from 9.48 to 6.54
(6.93 in the first run), and its accuracy is 1.0 point below the start (interval $-$2.1 to $-$0.3,
first run $-$1.2). A second run of the accuracy-reward arm agrees as well: 99.8\% of the thoughts
end, at 439 tokens, the error is 7.28 (7.79 in the first run), and accuracy after the thought is 1.0
point below the start (interval $-$2.1 to $-$0.1). A third arm replaces the length price by a reward
of 0.1 for a thought that ends by itself after at least 64 tokens. It ends 98.4\% of the thoughts at
a median of 751 tokens, the length the stop step gives, with accuracy after the thought 0.75 points
below the start (interval $-$1.78 to +0.14) and a calibration error of 9.10. A reward for ending
makes the thoughts end without making them shorter, and it raises neither accuracy nor calibration.

\subsection{Key findings}\label{sec:5.6}

\begin{mdfindings}
\begin{itemize}
\item A loss on the answer alone leaves the end of a thought unsupervised. The probability of closing a
finished thought fell from 0.54 to 0.06 in the 9B data round and from 0.73 to 0.26 in the 4B reader
round, and only the stage with a loss on the closing tag restored it. Anyone who trains a decision
head on answer letters can run the same probe on stored thoughts to see whether a stage takes the
end away.
\item The end can be taught from the model's own thoughts. Eighty-two steps on thoughts cut where the
answer stops changing take the share of 4B thoughts that end from 11.4\% to 85.9\% at unchanged
accuracy on held-out items.
\item \textbf{A thought is worth two to three index points, and far more where the answer is computed}:
rebuilt GSM8K rows go from a skill of 25--52 to 92--99. On NLI-like and select-all questions it
lowers accuracy.
\item Reinforcement learning makes thoughts end and shortens them, and its calibration follows the length.
An accuracy reward with the same price reaches most of the calibration of the proper score, and no
arm raised accuracy (runs with a rank-initialisation fault, corrected runs pending).
\end{itemize}
\end{mdfindings}


==> sections/05_training.tex <==
\clearpage
\section{Training}\label{sec:5}

This chapter follows one model through its training stages (Figure~\ref{fig:2}).
Section~\ref{sec:5.1} gives the result after every stage, what a thought is worth (5.1.1) and how
long and how often to think (5.1.2). The release recipe and the decision data rounds come next, then
a diagnosis of what those rounds do to the model's ability to reason before it answers, then the
three stages that repair it. Two alternatives that we tested follow, and the chapter ends with
calibration and the findings.

\subsection{Results by stage}\label{sec:5.1}

Table~\ref{tab:5.1} reads from left to right in training order. ``One pass'' is the model answering
from a single forward pass. ``Reasoning'' is the default setting of the single control of
Section~\ref{sec:3.4}: the model writes a thought when the top probability of its one-pass answer is
below 0.9, reads the thought, and the two distributions are averaged.

\textbf{Names used in this chapter.} A \emph{thought} is the reasoning text a model writes before it
answers. A \emph{data round} takes typed decisions with their labels and trains an adapter on the
released weights, with a loss on the answer letter alone. \emph{Thinking replay} takes thoughts that
the starting model of the same size wrote for training items and trains the decision model to write
such thoughts and to close them. The \emph{reader round} takes thoughts written by the model itself
and trains the answer that is read after a thought. A second kind of row holds the one-pass answer
in place. The \emph{stop step} takes the model's own thoughts, cut where its answer stops changing,
and trains the model to close a thought at that point. The \emph{gate} decides which questions get a
thought: those whose one-pass answer has a top probability below a threshold, 0.9 unless stated. The
\emph{default answer} is what the model then returns: the one-pass read-out where the gate asks for
no thought, and elsewhere the equal mixture (weights 0.5 and 0.5) of the one-pass read-out and the
read-out after the thought. Tables~\ref{tab:5.5} and \ref{tab:5.7} head this answer ``default
control''.

\begin{table}[!htbp]
\renewcommand{\thetable}{5.1}
\centering
\caption{Decision Index 0.2.1 after each training stage (own runs of the public runner on all 38 benchmarks and 133,876 requests, coverage 1.0, chance-corrected skill, nothing submitted to the board). Each cell is one run. Two runs of one system with thoughts sampled anew differ by 0.05, and three training rounds of nearly the same recipe span 0.9 (Section~\ref{sec:6.1}).}\label{tab:5.1}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrrr}
\toprule
\textbf{size} & {\begin{tabular}[b]{@{}r@{}}\textbf{released,}\\\textbf{one pass}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{data}\\\textbf{rounds,}\\\textbf{one pass}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{+ reader round,}\\\textbf{reasoning}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{+ thinking replay}\\\textbf{and reader round,}\\\textbf{reasoning}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{+ stop}\\\textbf{step,}\\\textbf{reasoning}\end{tabular}} \\
\midrule
0.8B & 38.88 & 51.60 & -- & -- & -- \\
2B & 44.19 & 57.66 & -- & -- & -- \\
4B & 52.76 & 64.78 & 66.38 & 67.72 & 67.37 \\
9B & 58.64 & 67.75 & 69.32 & 69.77 & \textbf{70.16} \\
27B & 63.88 & 70.43 & 70.89 \textsuperscript{d}, 71.12 \textsuperscript{a}, 71.50 \textsuperscript{b} & \textbf{72.34} & -- \textsuperscript{c} \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{a} reader round on the routed items and the sources the data rounds added.
\textsuperscript{b} default reader round on the round before the last four select-all sources (70.08
in one pass). A second reader variant on that round scores 71.41. \textsuperscript{c} not needed at
this size: 6.0\% of the 27B's thoughts reach the limit. \textsuperscript{d} default reader round
with the sources the data rounds added, on the final recipe.\par}
\end{table}

With the reader round alone, reasoning adds 1.6 index points to the one-pass model at 4B and at 9B
and 0.5 to 0.7 at 27B on the final recipe (1.4 on the round before it). With thinking replay before
it the gain over one pass is 2.9 points at 4B, 2.0 at 9B and 1.9 at 27B, where the chain reaches
72.34: replay itself is worth 1.3 points at 4B, 0.5 at 9B and 1.2 to 1.5 at 27B. Almost all of it is
in the knowledge and reasoning area: 45.4 $\rightarrow$ 57.0 at 4B, 55.1 $\rightarrow$ 62.9 at 27B
(Section~\ref{sec:6.12}). The stop step keeps 67.37 at 4B with 43\% of the reasoning tokens and
raises the 9B to 70.16 with 53\% of them.

\subsubsection{What a thought is worth}\label{sec:5.1.1}

Table~\ref{tab:5.9} puts four measurements side by side: the public index with the gate at its
default, and three sets on which every item gets a thought. These are the GSM8K rows as rebuilt for
edition 0.3 of the index, whose wrong options no longer give the answer away
(Section~\ref{sec:6.2.1}), ten tasks of our own benchmark, and the harder versions of three of its
generated tasks (Section~\ref{sec:6.14}).

\begingroup
\renewcommand{\thetable}{5.9}
\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\begin{longtable}{>{\raggedright\arraybackslash}p{\mdw{0.2121}}>{\raggedright\arraybackslash}p{\mdw{0.1857}}>{\raggedleft\arraybackslash}p{\mdw{0.0919}}>{\raggedleft\arraybackslash}p{\mdw{0.1147}}>{\raggedleft\arraybackslash}p{\mdw{0.1003}}>{\raggedleft\arraybackslash}p{\mdw{0.1661}}>{\raggedleft\arraybackslash}p{\mdw{0.1164}}}
\caption{What a thought is worth, on four measures (own runs, 5 to 7 October 2026, one run each, 4,096-token limit). \emph{Index:} Decision Index 0.2.1 with the gate at 0.9, in index points. \emph{GSM8K:} the rows rebuilt for edition 0.3, a thought on every item. Chance-corrected skill is the mean of the benchmark's two tracks, and ranges are over the two tracks. \emph{Benchmark tasks:} 6,019 items of ten tasks of our own benchmark (the seven generated tasks and three reused ones), a thought on every item. Accuracy of the default answer with the gate at 0.9. \emph{Harder generated tasks:} the 1,800 items of the second versions of three generated tasks, measured in the same way. ``Starting model'' is the untrained model a size was built from. It writes its own thought and is read through the same read-out.}\label{tab:5.9}\\
\toprule
\textbf{measure} & \textbf{model} & \textbf{one pass} & \textbf{after the thought} & \textbf{default answer} & \textbf{thoughts that end by themselves} & \textbf{tokens per thought} \\
\midrule
\endfirsthead
\multicolumn{7}{l}{\textit{Table~\thetable{} (continued)}}\\
\toprule
\textbf{measure} & \textbf{model} & \textbf{one pass} & \textbf{after the thought} & \textbf{default answer} & \textbf{thoughts that end by themselves} & \textbf{tokens per thought} \\
\midrule
\endhead
\bottomrule
\endfoot
Decision Index 0.2.1, gate at 0.9 (index points) & 4B, after the stop step & 64.78 & -- & 67.37 & 10.4\% reach the limit & 1,585 \\
 & 9B, after the stop step & 67.75 & -- & 70.16 & 15.8\% reach the limit & 1,900 \\
 & 27B, after thinking replay and reader round & 70.43 & -- & 72.34 & 6.0\% reach the limit & 710 \\
GSM8K, rebuilt rows, a thought on every item (skill) & 4B starting model, untrained & 10.9 & 97.1 & 97.1 & 99.3--99.8\% & 261--290 \\
 & 4B, after the stop step & 25.4 & 94.4 & 93.8 & 95--96\% & 620--720 \\
 & 4B, stop step and reinforcement learning \textsuperscript{a} & 25.3 & 92.2 & 91.2 & 100\% & 415--462 \\
 & 9B starting model, untrained & 18.3 & 98.6 & 98.5 & \textsuperscript{b} & \textsuperscript{b} \\
 & 9B, after the stop step & 33.8 & 96.3 & 94.6 & 95--97\% & 613--741 \\
 & 9B, stop step and reinforcement learning \textsuperscript{a} & 34.1 & 96.6 & 95.2 & \textsuperscript{b} & \textsuperscript{b} \\
 & 27B, after thinking replay and reader round & 52.3 & 98.9 & 98.3 & \textsuperscript{b} & \textsuperscript{b} \\
Ten benchmark tasks, a thought on every item (accuracy) & 4B, after the stop step & 0.709 & 0.876 & 0.855 & 80.4\% & 1,687 \\
 & 9B, after the stop step & 0.735 & 0.880 & 0.862 & 72.8\% & 1,909 \\
 & 27B, after thinking replay and reader round & 0.836 & 0.948 & 0.930 & 96.1\% & 567 \\
\ldots{} of these: policy with exceptions and precedence & 4B / 9B / 27B & 0.552 / 0.557 / 0.758 & 0.938 / 0.978 / 1.000 & -- & -- & -- \\
\ldots{} count check on logs & 4B / 9B / 27B & 0.492 / 0.550 / 0.608 & 0.897 / 0.920 / 0.993 & -- & -- & -- \\
\ldots{} state after a sequence of operations & 4B / 9B / 27B & 0.590 / 0.612 / 0.743 & 0.860 / 0.907 / 0.985 & -- & -- & -- \\
Three harder generated tasks, a thought on every item (accuracy) & 4B, after the stop step & 0.602 & 0.843 & 0.802 & 83.0\% & 1,616 \\
 & 9B, after the stop step & 0.627 & 0.892 & 0.834 & 81.6\% & 1,710 \\
 & 27B, after thinking replay and reader round & 0.780 & 0.984 & 0.941 & 98.7\% & 405 \\
\ldots{} of these: filter match with computed constraints & 4B / 9B / 27B & 0.622 / 0.620 / 0.682 & 0.953 / 0.970 / 0.990 & -- & -- & -- \\
\ldots{} answerable facts over several hops \textsuperscript{c} & 27B & 0.823 & 0.983 & -- & -- & -- \\
\ldots{} tool-call validity with nested schemas \textsuperscript{c} & 4B / 27B & 0.573 / 0.835 & 0.702 / 0.980 & -- & -- & -- \\
\end{longtable}
\endgroup
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{a} Section~\ref{sec:5.9}. 4B: the arm whose rollouts are sampled as at inference.
9B: the arm whose rollouts are sampled at temperature 1, with thoughts of about 1,170 tokens on
held-out items. \textsuperscript{b} \todo[TODO(gsm3\_think)]{share of thoughts that end and tokens
per thought for these three models} \textsuperscript{c} \todo[TODO(bthink2)]{per-task values of the
4B and the 9B on answerable facts and of the 9B on tool-call validity}\par}

On the index a thought adds two to three points, and where the answer has to be computed it decides
the result. With the gate at 0.9 the default answer is 2.6 (4B), 2.4 (9B) and 1.9 (27B) index points
above one pass for the models of the table, and 2.9 for the 4B before its stop step. Our models have
a one-pass skill of 25 to 52 on the rebuilt GSM8K rows and reach 92 to 99 after a thought: on a task
that needs computation and offers no shortcut in its options, the thought is worth about 65 points
of skill at 4B and 9B. Accuracy on the ten benchmark tasks rises from 0.709--0.836 to 0.876--0.948.
Three of these tasks are the ones on which our one-pass models trail the first entry of the public
board (Section~\ref{sec:6.14}). On them the 27B goes from 0.758, 0.608 and 0.743 to 1.000, 0.993 and
0.985, and the 4B and the 9B reach 0.86 to 0.98, where that entry has about 0.985, 0.85 and 0.83 in
one pass. For the harder versions of three other generated tasks the 27B goes from 0.780 to 0.984,
the 9B from 0.627 to 0.892 and the 4B from 0.602 to 0.843, where that entry has 0.866 in one pass
(0.975, 0.703 and 0.920 on the three tasks). The largest step is on the filter match with computed
constraints, the task that is hardest for every one-pass model: 0.682 $\rightarrow$ 0.990 at 27B,
0.620 $\rightarrow$ 0.970 at 9B and 0.622 $\rightarrow$ 0.953 at 4B. The 4B gains least on tool-call
validity with nested schemas (0.573 $\rightarrow$ 0.702, against 0.835 $\rightarrow$ 0.980 at 27B).
The two sides of this comparison are not alike: the other entry's values are one-pass values, ours
cost a thought per item.

A thought helps where the answer needs several steps of computation over the record, and hurts on
NLI-like and select-all questions. On the 3,021 routed held-out items of the training distribution
(4B after thinking replay and reader round, 21 task families) the answer after the thought is better
than the one-pass answer in 9 families and worse in 7: code +38.0 points, medical questions +9.9 and
temporal and unit reasoning +9.8 on one side, select-all $-$7.0, ANLI $-$4.8 and ContractNLI $-$2.4
on the other. The largest gains of the default answer over one pass on the index are on CRUXEval
(+25.3), MMLU-Pro (+13.2), GPQA (+11.2), SGD (+7.6), PhishNChips (+5.1), BBH (+4.7) and GSM8K in its
old rows (+4.3), for the 4B after reinforcement learning (Section~\ref{sec:5.9}). In the benchmark
the reused tasks gain less than the three procedural ones (27B: FOLIO 0.760 $\rightarrow$ 0.828,
JudgeBench 0.782 $\rightarrow$ 0.851, ProcessBench 0.746 $\rightarrow$ 0.829), and the first version
of tool-call validity does not move.

Where the answer has to be computed, the default answer stays below the answer after the thought, by
four points at 27B. On the three harder generated tasks the 27B has 0.984 after the thought and
0.941 as its default answer. The 9B has 0.892 and 0.834, the 4B 0.843 and 0.802. The 9B has 96.3 and
94.6 on the rebuilt GSM8K rows. Both parts of the default control are involved. The gate does not
send a confidently wrong one-pass answer to reasoning. And where it does send a question, half of
the mixture is a one-pass read-out that is near chance on such items. On tasks of this kind the gate
and the weight limit the result, not the thought: at 27B the answer after the thought is right on
98.4\% of items on which the one-pass 27B models of Table~\ref{tab:6.14}, Clef apart, are right on
79 to 87\%. A rule that sets the weight from the one-pass confidence did not beat 0.5 on held-out
items of the training distribution, where such tasks are rare (Section~\ref{sec:5.1.2}). A rule for
them would have to be fitted on items of that kind, and none has been.

\textbf{Limits.} (1) The main ranking of the public board does not count models that may think. A
separate board for them is announced (edition 0.3, Section~\ref{sec:6.3.1}). That ranking counts
one-pass answers only, the first numeric column of the table. (2) The models we started from still
think better on arithmetic than ours. The untrained 4B reaches 97.1 after a thought, our 4B 94.4
after the stop step and 92.2 after reinforcement learning. The untrained 9B reaches 98.6, ours 96.3
and 96.6. The untrained 4B does this with thoughts of 261 to 290 tokens, of which 99.3 to 99.8\%
end. Decision training costs reasoning quality, and thinking replay, the reader round and the stop
step do not return all of it. (3) A thought costs about 400 to 1,900 tokens in the runs of the table
and the latency of writing them. Averaged over all answers of an index run, that is 193 reasoning
tokens per answer at 27B and 497 and 552 at 4B and 9B (Table~\ref{tab:5.6}). (4) Neither a longer
limit nor reinforcement learning has added accuracy (Sections~\ref{sec:5.1.2}
and \ref{sec:5.9}). All values of the table are single runs.

\subsubsection{How long and how often to think}\label{sec:5.1.2}

Four settings decide what reasoning costs and what it returns: the token limit of a thought, a loop
check that may end it early, the gate, and the weight of the thought in the default answer. This
section gives the measurement and a short conclusion for each. The model is the 4B after thinking
replay and reader round, the stage at which most thoughts do not end (Section~\ref{sec:5.4}), and,
for comparison, the 4B after the stop step.

\begin{table}[!htbp]
\renewcommand{\thetable}{5.10}
\centering
\caption{Token limit, loop check and gate (4B, accuracy in percent). \emph{Block A:} 3,021 routed held-out items of the training distribution, one thought per item. The loop check looks for repetition every 256 tokens and ends a thought that has begun to repeat. In brackets: paired difference of the default answer to the 4,096-token row of the same model without a check, with its 95\% bootstrap interval over items. Index: Decision Index 0.2.1 with the gate at 0.9, one run per row, and ``--'' means not measured. \emph{Block B:} the gate, for the 4B after thinking replay and reader round with a limit of 4,096 tokens. Held-out columns: the 8,598 held-out items of the training distribution, stored thoughts replayed at each threshold (Table~\ref{tab:6.11}). Index: one run per threshold.}\label{tab:5.10}
{\scriptsize\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrlrrrrrr}
\toprule
\textbf{4B model} & \textbf{limit} & {\begin{tabular}[b]{@{}l@{}}\textbf{loop}\\\textbf{check}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{after the}\\\textbf{thought}\end{tabular}} & \textbf{default answer} & {\begin{tabular}[b]{@{}r@{}}\textbf{open}\\\textbf{at the}\\\textbf{limit}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{cut}\\\textbf{at a}\\\textbf{loop}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{tokens}\\\textbf{per}\\\textbf{thought}\end{tabular}} & \textbf{index} \\
\midrule
thinking replay and reader round & cut at 1,024 & no & -- & 75.54 (+0.00 {[}$-$0.60, +0.63{]}) & -- & -- & 992 & 66.93 \\
 & 4,096 & no & 75.04 & 75.54 & 88.6\% & -- & 3,764 & 67.72 \\
 & 4,096 & yes & 74.91 & 75.54 & 24.1\% & 63.9\% & 2,916 & -- \\
 & 8,192 & yes & 74.61 & 75.11 ($-$0.43 {[}$-$1.09, +0.20{]}) & 6.9\% & 80.2\% & 3,367 & 67.52 \textsuperscript{c} \\
 & 16,384 & no & 74.54 & 75.31 \textsuperscript{a} & 87.4\% & -- & 14,512 & -- \\
 & 16,384 & yes \textsuperscript{b} & 75.14 & 75.60 \textsuperscript{a} & -- & 80.6\% & 4,287 & -- \\
\ldots{} and stop step & 4,096 & no & 74.38 & 75.31 & 14.1\% & -- & 1,413 & 67.37 \\
 & 4,096 & yes & 74.54 & 75.60 (+0.30 {[}$-$0.40, +0.99{]}) & 3.5\% & 12.6\% & 1,186 & -- \\
 & 8,192 & yes & 74.61 & 75.37 & 0.7\% & -- & 1,251 & -- \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{a} measured in a separate run against its own 4,096-token reference with the loop
detector (75.24): differences +0.07 {[}$-$0.56, +0.73{]} and +0.36 {[}$-$0.23, +0.96{]}.
\textsuperscript{b} the loop detector of Table~\ref{tab:5.5}, which is the guard of
Section~\ref{sec:3.4}. \textsuperscript{c} index run with a limit of 8,192 tokens. Our record of the
run gives the limit and not the state of the loop check \todo[TODO(rd4tfb8k\_di)]{whether the loop
check was on in the index run at a limit of 8,192}\par}
\par\medskip
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrr}
\toprule
{\begin{tabular}[b]{@{}l@{}}\textbf{B. gate: a thought is}\\\textbf{written when the one-pass}\\\textbf{top probability is below}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{held-out items:}\\\textbf{questions}\\\textbf{thought about}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{held-out items:}\\\textbf{default answer}\end{tabular}} & \textbf{index} \\
\midrule
never (one pass) & 0.0\% & 89.33 & -- \\
0.5 & 6.3\% & 90.20 & -- \\
0.7 & 18.9\% & 90.71 & 67.20 \\
0.9 (default) & 35.1\% & 90.71 & 67.72 \\
0.98 & -- & -- & \todo[TODO(rd4tfg98\_di)]{index with the gate at 0.98} \\
always & 100.0\% & 90.72 & -- \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\textbf{Limit.} A longer limit adds nothing: at 8,192 tokens with the loop check the default answer
is 0.43 points lower (interval $-$1.09 to +0.20), and at 16,384 tokens without it 87.4\% of the
thoughts are still open at four times the tokens. The index says the same: with a limit of 8,192
tokens the 4B scores 67.52, against 67.72 at 4,096. A shorter limit costs where thoughts have to be
long: the cut at 1,024 tokens is free on held-out items and takes 0.79 points from the index (66.93
against 67.72).

\textbf{Loop check.} A check every 256 tokens removes most of the open thoughts at no cost in
accuracy: before the stop step 24.1\% instead of 88.6\% stay open, after it 3.5\% instead of 14.1\%,
with the default answer at 75.54 and 75.60.

\textbf{Tokens spent.} Across the designs of Table~\ref{tab:5.6} the index follows the reasoning
tokens per answer (66.80 at 200, 67.23 at 330, 67.37 at 497 and 67.72 at 1,144, against 64.78 in one
pass), so every step that made more thoughts end has cost a few tenths of a point and saved a large
share of the tokens. These are single runs of separately trained models, and steps of this size are
inside the spread between training rounds.

\textbf{Gate.} On the 8,598 held-out items of the training distribution, never thinking gives 89.33,
thinking below 0.5 (6.3\% of the items) 90.20, below 0.7 (18.9\%) 90.71, below 0.9 (35.1\%) 90.71
and always thinking 90.72 (block B): there the gain is complete at 0.7, with about half as many
thoughts as at the default. The index does not agree. With the gate at 0.7 the same model scores
67.20, against 67.72 at 0.9: thinking only below 0.7 costs half an index point. The two runs are of
one model, and two runs of one system with thoughts sampled anew differed by 0.05, a tenth of this
difference. We read the half point as the index holding more items than the held-out set on which
the one-pass answer is confident and wrong. The count of such items is not in this report. The
default stays at 0.9, and a run with the gate at 0.98 is in progress (block B).

\textbf{Weight of the thought.} Where the gate asks for a thought, the default answer gives the
thought a fixed weight of 0.5. A weight that depends on the one-pass confidence does not do better
on held-out items of the training distribution. We split the 8,598 held-out items into two halves,
one to choose a rule and one to test it. For the 4B after thinking replay and reader round the flat
mixture has 90.12 on the test half, the thought alone 89.91, fitted log pools 90.05 to 90.07, and
rules that give the thought a weight of 0.75 or 1.0 when the one-pass top probability is below a
threshold between 0.4 and 0.7 reach 90.12 at best. One pass has 88.60. For the 9B after the stop
step the flat mixture has 92.96, the thought alone 92.52, log pools 92.71 to 92.82 and linear
weights 92.64 to 92.77. One pass has 91.99. No rule chosen on the first half beats the flat mixture
on the second. The loss of the mixture on tasks that need computation does not show here, because
such items are rare in this distribution. None of these rules was run on the index. For a caller who
accepts answers above a threshold the fitted log pool remains the better confidence at the same
accuracy: on the routed held-out items of the stop-trained 4B, 17.5\% of the answers can be accepted
at an error of 5\% with it, against 4 to 5\% with the mixture (Section~\ref{sec:7.1}).

\subsection{Release recipe}\label{sec:5.2}

\textbf{Purpose.} The release recipe turns a pretrained multimodal language model into a model that
answers a typed question in one forward pass, by reading the option letters at one position.

\textbf{Data.} Two mixes per size (Table~\ref{tab:4.2}, block A): a broad mix for full fine-tuning
(2,726,203 rows, 791,992 for the 27B) and a curated mix of hard decisions for the adapter (190,418
rows, 92,228 for the 4B).

\textbf{Method.} (1) \emph{Full fine-tuning.} All text parameters are trained for one epoch on the
broad mix. The loss is the soft cross-entropy between the target distribution of a row and the
softmax over its listed options, computed on the 26 letter rows of the model's own output layer at
the last prompt position. No parameter is added, and the quantity trained is the quantity served.
(2) \emph{Adapter fine-tuning.} From the same starting weights (not from the result of step 1), a
rank-64 adapter on every projection of the text layers is trained for two epochs on the curated mix
and merged. (3) \emph{Averaging.} The two models are averaged tensor by tensor with equal weights:
the fully fine-tuned model carries the index, the adapter model the hard public items, and the
average keeps most of both. (4) \emph{Calibration} (Section~\ref{sec:5.10}). The 0.8B is step 1
alone, from Qwen3.5-0.8B-Base. Both halves of the 2B and 4B start from the instruction-tuned
Qwen3.5-2B and Qwen3.5-4B, those of the 9B from the post-trained Qwen3.5-9B and those of the 27B
from Qwen3.8-27B. The 35B-A3B is, by our project notes, an average of the same kind on
Qwen3.6-35B-A3B \todo{verify starting model, mixes and settings of the 35B-A3B}.

\textbf{Settings.} The peak learning rate of full fine-tuning falls with size, from 2e-5 (0.8B) to
2e-6 (27B). The adapter uses 1e-4 (5e-5 at 27B). A run uses 8 to 56 H200 GPUs for 0.5 to 4.4 hours
(Table~\ref{tab:5.8}, Appendix~\ref{sec:F}).

\textbf{Result after the stage.} The released models score 38.88, 44.19, 52.76, 58.64 and 63.88 on
the Decision Index 0.2.1 from 0.8B to 27B (Table~\ref{tab:5.1}). Step 1 does most of it: read with
our read-out before any training, the 27B starting model scores 49.27, and 64.02 after step 1.
Averaging costs the fully fine-tuned model 0.1 to 0.5 index points (2.0 at 4B). On the 231 public
JevBench items the average is above both parents at 2B, 9B and 27B (27B: 208 against 207 and 205)
and one item below the adapter model at 4B (204 against 198 and 205). At 0.8B the Base checkpoint is
the better start (38.86 against 36.76), so the 0.8B is not an average.

\textbf{What did not work.} \emph{A second-stage adapter on the fine-tuned weights}, trained on rows
that the first-stage model gets wrong, human-labelled rows and replay rows with the first-stage
distribution as target: all eleven runs of the second and third day scored below their parent on the
index, by 0.50 to 2.86 points, while a development set from the source of their new rows rose in
every one. No released model contains this stage. \emph{One learning rate for all sizes:} at 2e-5
the 9B scored 51.68, below the 4B (54.82). At 1e-5 it scored 56.07, and from the post-trained
checkpoint at 5e-6 58.78. Lower is not always better: the 4B scored 51.79 at 5e-6 against 54.70 at
1e-5. \emph{More nodes for a small model:} the 4B on eight nodes used four times the GPUs for steps
that were 7\% faster.

See Tables~\ref{tab:F.1}, \ref{tab:F.2}, \ref{tab:F.7} and \ref{tab:F.8}, and for the mixes
Section~\ref{sec:4.4} and Appendix~\ref{sec:G}.

\subsection{Decision data rounds}\label{sec:5.3}

\textbf{Purpose.} A data round adds tasks that the released model was never shown and repairs faults
of the earlier mixes, while holding the model to what it already does.

\textbf{Data.} The final recipe has 1,078,788 rows: a sample of the release mix, anchor rows,
teacher-labelled decisions, general multiple choice and the targeted sources (Tables~\ref{tab:4.1}
and \ref{tab:4.2}, blocks B).

\textbf{Method.} A rank-64 adapter ($\alpha$ = 128) on every projection matrix of the text layers is
trained on the released weights for one epoch with the loss of Section~\ref{sec:5.2} and merged. The
vision tower, the tokenizer and the configuration stay those of the release. Anchor rows have the
released model's own distribution as their target and three times the weight of an ordinary row.
Rounds are not stacked: every round starts from the released weights and replaces the previous one.

\textbf{Settings.} Learning rate 5e-5, warm-up over 5\% of the steps, cosine decay to zero, eight
GPUs (Table~\ref{tab:5.8}).

\begin{table}[!htbp]
\renewcommand{\thetable}{5.8}
\centering
\caption{Training settings, stages as columns. AdamW with gradients clipped at norm 1 and no weight decay in every stage, bf16 computation, H200 GPUs and inputs up to 12,288 tokens. Per-size values: Appendix~\ref{sec:F}.}\label{tab:5.8}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.1204}}>{\raggedright\arraybackslash}p{\mdw{0.2184}}>{\raggedright\arraybackslash}p{\mdw{0.2962}}>{\raggedright\arraybackslash}p{\mdw{0.1456}}>{\raggedright\arraybackslash}p{\mdw{0.2060}}}
\toprule
 & \textbf{full fine-tuning} & \textbf{adapter fine-tuning} & \textbf{averaging} & \textbf{decision data round} \\
\midrule
starts from & starting model & starting model & the two models to the left & released weights \\
trained & all text parameters and the output layer & rank-64 adapter, $\alpha$ = 128, on attention, linear-attention and feed-forward projections & -- & the same adapter \\
data (rows) & 2,726,203 (27B 791,992) & 190,418 (4B 92,228) & -- & 1,078,788 \\
epochs & 1 & 2 & -- & 1 \\
peak learning rate & 2e-5 (0.8B), 1e-5 (2B, 4B), 5e-6 (9B), 2e-6 (27B) & 1e-4 (27B 5e-5) & -- & 5e-5 \\
schedule & 3\% warm-up, cosine to zero (27B: to 10\% of the peak) & cosine \todo{warm-up share} & -- & 5\% warm-up, cosine to zero \\
rows per step & 192--384 & 96--256 & -- & 184 (9B 96, 27B 128) \\
steps & 3,535--14,198 & 1,002--3,966 & -- & 5,862 (9B 11,235, 27B 8,408) \\
AdamW $\beta$2 & 0.95 & 0.999 & -- & 0.999 \\
GPUs $\times$ hours & 8 $\times$ 1.03 (0.8B) to 56 $\times$ 3.19 (27B) & 8 $\times$ 0.50 (4B) to 16 $\times$ 2.42 (27B) & CPU & 8 $\times$ 0.75 (0.8B), 8 $\times$ 1.05 (2B), larger sizes Table~\ref{tab:2.2} \\
weight in the average & 0.5 (0.8B: not averaged) & 0.5 & equal & -- \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\textbf{Result after the stage.} In one pass the final recipe scores 51.60, 57.66, 64.78, 67.75 and
70.43 from 0.8B to 27B, against 38.88, 44.19, 52.76, 58.64 and 63.88 for our own runs of the
released weights (Table~\ref{tab:5.1}). At 27B the largest steps are select-all questions (+49.1
skill points), phishing decisions (+44.1), causal reasoning (+34.6) and chords (+32.7). The rounds
add tasks, not knowledge: at 0.8B a multiple-choice knowledge benchmark does not move (22.9
$\rightarrow$ 22.5) and graduate-level science questions fall from 10.2 to 0.0.

Outside the index the rounds do not help. The final recipe was built with the index as development
set (Section~\ref{sec:6.1}), and what it adds is a fit to the index's benchmarks. Four measurements
on data the rounds were not aimed at agree. On the unseen items of 35 reused public test sets the
final round changes the score of the released weights by $-$1.0 at 27B (95\% interval $-$1.6 to
$-$0.4), by 0.0 at 9B ($-$0.6 to +0.7) and by +0.1 at 4B ($-$0.6 to +0.7) (Section~\ref{sec:6.14}).
On 20 twin test sets, which measure skills of index benchmarks on other data, the 27B scores 71.1
before the round and 71.3 after it, the 9B 66.4 and 66.9, and the 4B 63.3 and 62.9
(Section~\ref{sec:6.15}). On a third-party set of agent decisions the 4B and the 9B do not move
(Section~\ref{sec:6.9}). And on the GSM8K rows as rebuilt for edition 0.3 of the index, whose
options no longer give the answer away, the rounds are below the released weights at every size: by
6.8 skill points at 27B, 4.7 at 9B and 14.2 at 4B (Section~\ref{sec:6.2.1}). One measurement points
the other way at 27B and has no interval yet: on the tasks generated for this report the 27B after
the rounds is 1.1 points (first versions) and 2.0 points (second versions) above the released 27B.
At 4B the first versions give 55.1 after the rounds against 55.8 before (Table~\ref{tab:6.14}).
Index-targeted data rounds, as we built them, do not transfer to decisions outside the index.

\textbf{Blending the round with the released weights.} A blend needs no training: every tensor of
the 27B is a weighted average of the released model and the final round, and the temperatures are
fitted again. Table~\ref{tab:5.12} has two blends between the two models.

\begin{table}[!htbp]
\renewcommand{\thetable}{5.12}
\centering
\caption{Blends of the released 27B with the final round (one pass, own runs, 7 October 2026). Index: Decision Index 0.2.1. Unseen tasks: the 35 reused public test sets, restricted to items that our training data do not contain, reported as the paired difference to the released model with its 95\% bootstrap interval. Twins: the 20 twin test sets, chance-corrected, areas weighted as on the board without arts. GSM8K: the rows rebuilt for edition 0.3 of the index, chance-corrected skill.}\label{tab:5.12}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrr}
\toprule
{\begin{tabular}[b]{@{}l@{}}\textbf{share of the}\\\textbf{final round}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{Decision}\\\textbf{Index}\\\textbf{0.2.1}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{unseen tasks:}\\\textbf{difference to the}\\\textbf{released model}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{twin}\\\textbf{test}\\\textbf{sets}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{rebuilt}\\\textbf{GSM8K}\\\textbf{rows}\end{tabular}} \\
\midrule
0 (released weights) & 63.88 & -- & 71.1 & 60.5 \\
50\% & 69.23 & $-$0.3 {[}$-$0.8, +0.1{]} & 71.9 \textsuperscript{a} & 58.3 \\
75\% & 70.46 & $-$0.8 {[}$-$1.3, $-$0.2{]} & 71.7 \textsuperscript{a} & 56.1 \\
100\% (final round) & 70.43 & $-$1.0 {[}$-$1.6, $-$0.4{]} & 71.3 & 53.7 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{a} the 75\% blend was scored in an earlier pass, in which the half blend read 71.8.\par}
\end{table}

The half blend keeps 82\% of the gain on the public index and gives back about 70\% of the loss on
unseen tasks. It is 0.7 points above the final round there (interval +0.2 to +1.1). Its remaining
distance to the released model is inside its interval overall, but not on the layer of
after-generation checks ($-$1.4, interval $-$2.3 to $-$0.6, and guards +0.2). The 75\% blend has the
public score of the full round and most of its loss: +0.2 against the final round ($-$0.1 to +0.6)
and $-$0.4 against the half blend ($-$0.8 to $-$0.1). The public score is flat from 75\% on, and the
loss on unseen tasks grows with the share of the round: $-$0.3, $-$0.8 and $-$1.0 at 50\%, 75\% and
100\%. The rebuilt GSM8K rows give the same order: 60.5, 58.3, 56.1 and 53.7 skill points at 0\%,
50\%, 75\% and 100\% of the round. Where unseen tasks count for more than the public index (edition
0.3 of the index puts four fifths of its weight on private tests, Section~\ref{sec:6.3.1}), the half
blend is the better point of the three. This is a reading of our own measurements and not a board
result. We cannot run the private tests.

At 4B the half blend behaves in the same way (Table~\ref{tab:5.13}). It scores 62.45 on the index,
between the released weights (52.76) and the final round (64.78), which is about four fifths of the
public gain. On unseen tasks it is at +0.5 against the released weights (interval $-$0.1 to +0.9),
where the final round is at +0.1 ($-$0.6 to +0.7). On the generated tasks it has 56.8 against 55.8
and 55.1, on the twins 63.4 against 63.3 and 62.9, and on the rebuilt GSM8K rows 30.4 against 37.2
and 23.0. \todo[TODO(bl9\_k20\_r50)]{the half blend at 9B}

\textbf{What did not work.} \emph{A higher learning rate:} 1e-4 gives 55.06 against 56.11 at 4B and
61.04 against 61.24 at 9B. \emph{Averaging two rounds as a free gain:} the average is about half a
point above the mean of the two (9B +0.56, 4B +0.50) and beats the better round only when its
partner is as good. Interpolation towards the starting weights lowers the 9B from 61.24 to 60.85 at
weight 0.5 on the index, which does not show what such a blend returns on unseen tasks. \emph{A
short second adapter for one new source:} at 4B it matches the joint round (59.02 against 58.91). At
9B the chord benchmark goes from 24 to 79 while the other four areas lose 0.6 in total, so targeted
data goes into the full round. \emph{Targeted rows without general ones:} three 4B rounds answered
37 to 166 fewer questions of a multiple-choice knowledge benchmark than the round they extended. The
heavier anchor with 30,000 general multiple-choice rows wins back 139 answers at the same index
(60.98 against 60.94). \emph{Other kinds of round data:} documents up to 32,000 tokens lowered a
long-document benchmark from 0.448 to 0.428 at 4B, rows converted from visual question answering
lowered the mean of eight image benchmarks from 81.2 to 80.3, and three preference-judging sets cost
five of the 231 public items. None is in the final recipe. Section~\ref{sec:4.6} lists the data
faults.

\textbf{Breadth in place of index-targeted sources: three rounds at 4B.} According to their model
cards, the two entries with the highest private scores of edition 0.3 were trained on several
hundred task families with small caps per family, in one pass at a learning rate of 2e-6 on all
weights. Our recipe uses the training splits of the index's own data sets and targeted rounds, with
adapter rounds at larger rates. We put the first kind of data into our own recipe. The \emph{breadth
files} are built from the training files of a public collection of task families recast as typed
decisions (tasksource, Section~\ref{sec:4.1.1}): a core file of 343 tasks and 642,628 rows, with at
most 3,000 rows per task, and three \emph{single-skill files} for stance (18 tasks, 17,378 rows),
sarcasm (10 tasks, 18,158 rows) and select-all questions (3 tasks, 8,995 rows). Three rounds at 4B
use them. Each starts from the released weights with the settings of the final recipe (one epoch,
rank-64 adapter, learning rate 5e-5) and is followed by the index, our own benchmark, the twin test
sets and the rebuilt GSM8K rows. None of the three trains on a family from which a twin test set is
built, so for them the twins measure transfer.

\begin{table}[!htbp]
\renewcommand{\thetable}{5.13}
\centering
\caption{Breadth rounds at 4B, with the released weights, the final recipe and their half blend for comparison (one pass, own runs, 7 October 2026, one training round and one run per row). Index: Decision Index 0.2.1. Unseen tasks: the 35 reused public test sets, restricted to items that our training data do not contain, reported as the paired difference to the released 4B with its 95\% bootstrap interval. Generated tasks: chance-corrected mean of the seven first versions. Twins: the 20 twin test sets, chance-corrected, areas weighted as on the board without arts. No interval has been computed for them. GSM8K: the rows rebuilt for edition 0.3, chance-corrected skill. The last row trains on twin-reserved families and is in-family on the twins (``Two training lines'' below). The rounds that take the data apart one group at a time are in Table~\ref{tab:5.14}.}\label{tab:5.13}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.3115}}>{\raggedleft\arraybackslash}p{\mdw{0.2140}}>{\raggedleft\arraybackslash}p{\mdw{0.1564}}>{\raggedleft\arraybackslash}p{\mdw{0.1170}}>{\raggedleft\arraybackslash}p{\mdw{0.0748}}>{\raggedleft\arraybackslash}p{\mdw{0.1132}}}
\toprule
\textbf{4B checkpoint} & \textbf{Decision Index 0.2.1} & \textbf{unseen tasks: difference to the released 4B} & \textbf{generated tasks} & \textbf{twin test sets} & \textbf{rebuilt GSM8K rows} \\
\midrule
released weights & 52.76 & -- & 55.8 & 63.3 & 37.2 \\
final recipe & 64.78 & +0.1 {[}$-$0.6, +0.7{]} & 55.1 & 62.9 & 23.0 \\
half blend of the two rows above & 62.45 & +0.5 {[}$-$0.1, +0.9{]} & 56.8 & 63.4 & 30.4 \\
(1) breadth only: the core of the release mix (teacher files, replay, knowledge questions), the single-skill files and all 642,628 breadth rows, no index-targeted file & 53.44 & $-$0.6 {[}$-$1.4, +0.1{]} & 55.8 & 64.0 & 36.5 \\
(2) final-recipe mix + 200,000 breadth rows & 65.03 & $-$0.9 {[}$-$1.6, $-$0.3{]} & 52.5 & 64.3 & 27.8 \\
(3) final-recipe mix + the single-skill files + 200,000 breadth rows & 64.56 & \textsuperscript{a} & \textsuperscript{a} & \textsuperscript{a} & 25.4 \\
(3) + twin-reserved families, at most 3,000 rows per task & \todo[TODO(r6\_4b\_kr23d)]{index, unseen tasks, generated tasks, area-weighted twins and GSM8K rows of this round} &  &  &  &  \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{a} \todo[TODO(r6\_4b\_kr23c)]{unseen tasks, generated tasks and twin test sets of
this round}\par}
\end{table}

Breadth rows alone move no overall score at 4B. Round (1) has no index-targeted file. Against the
released weights it is +0.7 on the index (53.44 against 52.76), $-$0.6 on unseen tasks (interval
$-$1.4 to +0.1), 0.0 on the generated tasks, +0.7 on the twins and $-$0.7 on the rebuilt GSM8K rows.
Inside the unseen tasks the layers move both ways: before-generation $-$2.5 ($-$4.3 to $-$1.0),
agent control $-$3.6 ($-$5.8 to $-$1.3), search and matching +1.4 (+0.4 to +2.6). Against the final
recipe it is $-$0.7 on unseen tasks ($-$1.5 to +0.1). So 642,628 rows from 343 task families, added
in our adapter recipe, leave the overall scores of the 4B on tasks outside the index where they
were, with single layers moving in both directions. They also leave arithmetic where the released
weights have it (36.5 against 37.2), which the index-targeted round does not (23.0). This is one
size and one recipe. It is not a test of the recipe of the entries named above, which train all
weights of the untrained base model at a learning rate of 2e-6. Section~\ref{sec:5.3.1} runs that
recipe at 4B.

Added to the final recipe, breadth rows help sibling data sets by about a point and cost about a
point on unseen and generated tasks. Round (2) scores 65.03 on the index (final recipe 64.78) and
64.3 on the twins (62.9), with ProofWriter at 54.2 against 43.3 and FiQA sentiment at 53.4 against
45.7 for the final recipe, and phishing e-mail at 81.1 against 88.0. On unseen tasks it is 1.1 below
the final recipe (interval $-$1.7 to $-$0.4), with search and matching at $-$2.6 ($-$3.7 to $-$1.3)
and before-generation at $-$1.7 ($-$2.9 to $-$0.1), and 0.9 below the released weights ($-$1.6 to
$-$0.3). On the generated tasks it has 52.5, against 55.1 and 55.8. Its rebuilt GSM8K skill is 27.8,
between the final recipe (23.0) and the released weights (37.2). Round (3) adds the single-skill
files to the mix of round (2): 64.56 on the index and 25.4 on the rebuilt GSM8K rows. Its other
comparisons had not been read. The same round at 9B was stopped on 7 October and has no result.

Other data of the ``same'' skill lowered two twins. The stance and the sarcasm file hold other
stance and irony data sets. They were meant to repair two skills on which, by the board's data, a
third party's fine-tune of our released 27B is far behind the first entry on the private twins
(Table~\ref{tab:6.17}). In round (1), which trained on both files, the stance twin scores 36.9
against 44.9 for the released 4B and the sarcasm twin 32.6 against 39.2. The rest of the picture is
mixed: the knowledge area is at 64.2 against 62.4 (ProofWriter 51.8 against 41.2, Corr2Cause 35.3
against 30.5, CODAH +2.2) and the retrieval area at 67.0 against 63.1 (WANDS 47.5 against 31.9, MTOP
intent +2.5), while language is at 51.8 against 53.0, with FiQA sentiment +9.7, and tools at 77.5
against 79.3. These are single differences without intervals. We read the two falls as a sign that
data sets of the same skill with other label conventions do not transfer to these twins at 4B and
can hurt, and both files are left out of the full-coverage round described below.

\textbf{Two training lines.} A twin test set, and a reused task of our own benchmark, measures
transfer only for a model that has not trained on its family. Where the first entry of edition 0.3
leads on our twins, the training list in its repository holds the training split of the twin's
source or a sibling (Section~\ref{sec:6.15}). We therefore keep two lines. The \emph{measurement
line}, which is rounds (1) to (3), keeps the twin families out of training so that the twins measure
transfer. The \emph{release line} also trains on the training splits of those families, cleaned item
by item. Its checkpoints are in-family on the twins and on the reused tasks concerned, will be
marked as such, and have to show their transfer on the generated tasks. Three files make the
difference between the lines (Section~\ref{sec:4.1.1}). The first holds the twin-reserved families,
33 tasks and 72,426 rows with the twin test items removed
(\texttt{ts\_\allowbreak{}v1\_\allowbreak{}twinfam}). The second has three further twin-reserved
tasks whose training rows share text with twin items and were cleaned row by row: Corr2Cause 2,812
rows, CODAH 1,965 and ReClor 2,981 (\texttt{ts\_\allowbreak{}v1\_\allowbreak{}twinfam2}). The third
holds the families that had been held back only to protect the reused half of our own benchmark
(rating and preference data, safety sets, FOLIO, PAWS and others): 58 tasks and 143,157 rows, after
6,089 rows were left out at build and 1,164 removed by the scan (\texttt{ts\_v1\_v0fam}). Three
tasks of the last group were not written: SciFact entailment, WinoDict and IntentGrasp. The data
sets of the Decision Index itself and Chinese families stay out of both lines.

\textbf{Procedural families.} The generated tasks on which our one-pass models trail ask for a
procedure: apply a written policy with its exceptions, count over records, track a state. According
to its model card, the first entry of edition 0.3 trained on 14 procedurally generated decision
families of about 9.2 thousand rows each. Our mixes held none. We wrote fifteen families of our own,
with labels computed by code and templates that are independent of the benchmark's generators.
Twelve families have 108,005 rows (\texttt{kr\_proc4}): policy application, a policy with a missing
fact, claims about logs, aggregate choice, state tracking, reconstruction of a state from events,
table lookup, evidence sufficiency, taxonomy routing, deadlines and units, two reports against a
log, and needles in long states. Three more have 27,001 rows (\texttt{kr\_proc4b}): validation of a
call against a schema, multi-hop answerability, and arithmetic word problems whose wrong options are
the answers of other problems. \emph{Audit.} In every family a probe that sees only the options, and
one that sees the question and the options, stay within 3 points of the majority rate, also on the
yes/no half and on the multi-option half taken separately. Probes on length and on the number of
lines are at 0.50, and an independent second implementation re-solves all 135,006 rows. The leak
scan against the evaluation index flags no row, and a direct comparison of 13-grams with the 6,000
generated benchmark items of both versions finds none. An in-family development set of 15 tasks with
300 items each goes with the families. Two rounds that train on them are measured below.

\textbf{Weak-area training sets.} Six files from public training splits cover skills on which our
models are measurably weaker than other systems: answerability of a question from a passage (32,000
rows), arithmetic in one pass (19,954), sarcasm (29,750), financial sentiment (10,777), phishing
against legitimate e-mail (11,621) and paraphrase (13,065). The arithmetic file holds AQuA-RAT and
MathQA only. GSM8K's own training split could not be used: 6,017 of its 7,473 problems (80.5\%)
carry text of protected evaluation items, because the routing benchmark of the index (RouterBench,
Tables~\ref{tab:H.2} and \ref{tab:H.5}) takes GSM8K training problems as its prompts. The 1,456
problems without such text are held aside and are in no mix.

See Tables~\ref{tab:F.4} and \ref{tab:F.5}, and Table~\ref{tab:G.10} for the sources that were
tested and removed.

\subsubsection{Recipe ablations at 4B}\label{sec:5.3.1}

The rounds above change several things at once. On 7 and 8 October 2026 we took the data apart at
4B. Each adapter round below starts from the released weights with the settings of the final recipe
and adds one group of data to its mix or removes one. Every round was trained once. Two rounds
combine groups. The \emph{full-coverage} round adds every group we expected to help: 200,000 breadth
rows, the select-all file, the twin-reserved and the benchmark-source families, 97,001 procedural
rows (70,000 of the twelve families and all rows of the three added ones), and the arithmetic and
answerability files. It holds neither sarcasm file and no stance file. The other combined round adds
the single-skill files, 200,000 breadth rows and the twin-reserved families at all usable rows. Two
further runs follow the recipe of the leading entries of edition 0.3: all weights of the untrained
4B, one epoch at a learning rate of 2e-6 or 5e-6, on about 825,000 rows of breadth and procedural
data and nothing else. Every checkpoint is read on five measures in one pass: the index, the plain
mean of the 20 twin tasks, the 35 reused tasks of our benchmark on items that our training data do
not contain, the second versions of three generated tasks, and the rebuilt GSM8K rows.

\begin{table}[!htbp]
\renewcommand{\thetable}{5.14}
\centering
\caption{Recipe ablations at 4B (one pass, own runs of 7 and 8 October 2026, one training run per row). A row is an adapter round on the released weights with the settings of the final recipe, unless it says otherwise. Index: Decision Index 0.2.1. Twins: plain mean of the 20 twin tasks, chance-corrected (Table~\ref{tab:5.13} weights the areas as the board does, which gives 63.3 and 62.9 for the first two rows). Reused tasks: the 35 reused public test sets of our benchmark on items that our training data do not contain, as the paired difference to the final recipe with its 95\% bootstrap interval. Generated tasks: second versions, accuracy in percent, chance 50. GSM8K: the rows rebuilt for edition 0.3, chance-corrected skill.}\label{tab:5.14}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.3190}}>{\raggedleft\arraybackslash}p{\mdw{0.1150}}>{\raggedleft\arraybackslash}p{\mdw{0.0753}}>{\raggedleft\arraybackslash}p{\mdw{0.1571}}>{\raggedleft\arraybackslash}p{\mdw{0.2067}}>{\raggedleft\arraybackslash}p{\mdw{0.1139}}}
\toprule
\textbf{4B checkpoint} & \textbf{Decision Index 0.2.1} & \textbf{twin test sets} & \textbf{reused tasks: difference to the final recipe} & \textbf{generated tasks: answerable facts / filter match / tool-call validity} & \textbf{rebuilt GSM8K rows} \\
\midrule
released weights & 52.76 & 61.9 & -- & 65.5 / 57.5 / 56.0 & 37.2 \\
final recipe & 64.78 & 61.6 & 0 & 61.5 / 63.2 / 57.2 & 23.0 \\
full coverage (see text) & 64.82 & 67.6 \textsuperscript{f} & +0.8 {[}+0.1, +1.7{]} \textsuperscript{f} & 77.3 / 66.8 / 68.2 & 33.3 \\
+ procedural families only (97,001 rows) & 65.03 & 61.7 & $-$0.5 {[}$-$1.2, +0.2{]} & 75.8 / 66.3 / 67.0 & 28.3 \\
+ benchmark-source families only: rating, preference, safety and logic sets (143,157 rows) & 65.04 & 61.8 & +1.9 {[}+1.1, +2.6{]} \textsuperscript{f} & 61.2 / 62.7 / 57.2 & 26.4 \\
+ the six weak-area training sets only (117,167 rows) & 65.14 & 64.4 \textsuperscript{f} & $-$1.5 {[}$-$2.3, $-$0.9{]} \textsuperscript{f} & 59.0 / 62.5 / 58.0 & 34.1 \\
final recipe without its 13,776 rows of VAST & 64.77 & 61.6 & $-$0.3 {[}$-$0.8, +0.3{]} & 58.7 / 65.2 / 56.5 & 28.9 \\
+ the single-skill files, 200,000 breadth rows and the twin-reserved families at all usable rows (121,204 rows, 1.7 times the file with at most 3,000 rows per task) & 65.16 & 65.6 \textsuperscript{f} & $-$1.0 {[}$-$1.7, $-$0.3{]} & 61.7 / 65.2 / 60.2 & 28.1 \\
all weights from the untrained 4B, learning rate 2e-6, breadth and procedural rows only & 40.87 & 55.6 & $-$3.3 {[}$-$4.3, $-$2.2{]} & -- & 27.2 \\
the same at 5e-6 & 44.71 & 59.2 & $-$2.9 {[}$-$3.9, $-$1.8{]} & -- & 46.4 \\
half blend of the 2e-6 run with the released weights & 49.60 & 61.1 & $-$0.7 {[}$-$1.4, +0.1{]} & -- & 35.8 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{f} in-family: the round trains on the family or the training split of some of these
test sets (see text).\par}
\end{table}

\textbf{The public index cannot tell the adapter rounds apart.} Every adapter round lies within 0.4
points of the final recipe on the index (64.77 to 65.16 against 64.78), and three rounds of nearly
the same recipe have spanned 0.9. The other measures separate the rounds, but each has a floor of
its own. Rounds without procedural data move a generated task by $-$2.8 to +3.0 points. Rounds
without the arithmetic file lie 3.4 to 5.9 skill points above the final recipe on the rebuilt GSM8K
rows, so only the two rounds with that file (+10.3 and +11.1) and one run from the untrained model
stand out there. A second run of the final recipe, listed at the end of this section, will measure
these floors directly.

\textbf{Full coverage helps exactly the families it contains.} Against the final recipe the
full-coverage round is level on the index and gains 6.0 points on the twins (67.6 against 61.6),
15.8, 3.6 and 11.0 points on the three generated tasks and 10.3 on the rebuilt GSM8K rows. The
single-factor rounds show where each gain comes from. The procedural families alone give 14.3, 3.1
and 9.8 points on the generated tasks and nothing on the twins (61.7). The benchmark-source families
give nothing on either (61.8 on the twins, every generated task within 0.5 points). The other
combined round, which holds the twin-reserved families, gains 4.0 points on the twins (65.6, and
65.7 when the families are capped at 3,000 rows per task) and at most 3.0 on a generated task. Its
mix also holds breadth rows, which alone added 1.4 points on the area-weighted twins of
Table~\ref{tab:5.13}, and every adapter round without twin data stays within 0.2 points of the final
recipe there. The weak-area files give 11.1 skill points on the rebuilt GSM8K rows through their
arithmetic part (34.1 against 23.0) and 2.8 on the twins. They hold data of four twin skills, among
them the training split behind the financial-sentiment twin.

The gain on the generated tasks is a gain on the kind of task that the procedural families teach.
The families were written apart from the benchmark's generators and share no 13-gram with the
generated items of either task version. Two of the three added families, multi-hop answerability and
the validation of a call against a schema, are of the same kind as answerable facts and tool-call
validity, and those two tasks gain most. For checkpoints trained on these families, transfer has to
be read on generated tasks of new kinds (Section 6.14.1).

\textbf{On the reused tasks the gain is exposure.} The full-coverage round is 0.8 points above the
final recipe on the reused tasks (interval +0.1 to +1.7), and the benchmark-source families alone
are 1.9 points above it (+1.1 to +2.6). Both rounds hold the families of 18 of the 35 reused tasks:
preference and judging sets, safety and injection sets, FOLIO, PAWS, AmbigQA, two legal sets and a
vulnerable-code set. We split the reused tasks into these 18 and the 16 whose families no file of
the three rounds holds. The benchmark-source families give +8.6 on their 18 tasks (+7.1 to +10.1)
and +0.3 on the 16 others ($-$0.7 to +1.3). The full-coverage round gives +9.0 (+7.3 to +10.5) and
$-$1.3 ($-$2.5 to 0.0). The weak-area round, which holds none of the 18 families, gives $-$5.7 on
them ($-$7.1 to $-$4.5) and $-$0.8 on the 16 ($-$1.8 to +0.3). No group of data raised a reused task
whose family it does not contain. The items are unseen in every case, so for these checkpoints the
18 tasks measure exposure to a family, and it is worth about nine points. For the board, a round can
then be expected to raise the private tests only where its data hold their families.

\textbf{More rows per family add nothing.} With the twin-reserved families at all usable rows, 1.7
times as many as with at most 3,000 rows per task, the round scores 65.6 on the twins against 65.7
for the same mix with the capped file. On the reused tasks it is 1.0 below the final recipe ($-$1.7
to $-$0.3).

\textbf{VAST is not the cause of the stance bias.} On the stance twin our checkpoints lean towards
the answer ``none'', and VAST, a stance data set in the final recipe, was its suspected source.
Without its 13,776 rows the index, the twins and the reused tasks stay where they were (64.77, 61.6,
and $-$0.3 with interval $-$0.8 to +0.3), and the stance twin falls from 38.7 to 29.5. The bias is
older than our training: when the target is not named in the text, the untrained 4B already answers
``none'' 65\% of the time.

\textbf{Distantly labelled sarcasm data hurts.} Three of the four sources of the weak-area sarcasm
file take their label from a mark the writer set (a hashtag on Twitter, ``/s'' on Reddit) or from
the site that published a headline. In the weak-area round the sarcasm twin is at 34.6, against 39.2
for the released weights. The sarcasm file of the task collection had lowered it to 32.6 in the
breadth-only round. Neither file is in the recipe below.

\textbf{Training from the untrained model with the settings of the leading entries fails at 4B.} At
a learning rate of 2e-6 the run scores 40.87 on the index and at 5e-6 44.71, below the released
weights (52.76). On the twins it has 55.6 and 59.2 against 61.6 for the final recipe, and on the
reused tasks it is 3.3 and 2.9 points below the final recipe (intervals $-$4.3 to $-$2.2 and $-$3.9
to $-$1.8). A half blend of the first run with the released weights does not recover it: 49.60 on
the index, 61.1 on the twins and $-$0.7 on the reused tasks ($-$1.4 to +0.1). This is one size and
one data set. The leading entries train at 27B, and these runs do not show that the recipe fails
there.

One number of these runs points elsewhere. At 5e-6 the run has the highest skill on the rebuilt
GSM8K rows of any 4B checkpoint, 46.4, against 37.2 for the released weights and 23.0 for the final
recipe. Its data hold no GSM8K row in the layout of edition 0.2.1, and its procedural part holds
arithmetic word problems whose wrong options are the answers of other problems, as in the rebuilt
rows. The same procedural families added to the final-recipe mix, which keeps the old rows, reach
28.3. We read this as one more sign that the old GSM8K rows of our release mix and data rounds teach
the model to answer from the layout of the options (Section~\ref{sec:6.2.1}). The hygiene repairs
below remove them.

\textbf{The recipe.} As these rounds leave it, the recipe for the next checkpoints has three steps.

\begin{enumerate}
\item Start from the released weights. A start from the untrained model with the settings of the leading
entries has not worked at 4B.
\item Train one data round on the final-recipe mix with the full-coverage data, which holds neither
sarcasm file, and with the hygiene repairs: the GSM8K rows of the old layout removed and 1,452 clean
GSM8K training problems added in the rebuilt layout (the 1,456 problems held aside, less four that
share text with a protected prompt), ANLI cut to 8,000 rows with balanced labels, select-all rows
capped at 15,000 per family with the EuroVoc cases of fewer than two correct options removed, and 45
groups of rows dropped that the current leak scan flags. \todo[TODO(r6\_4b\_kr28h)]{result of the
hygiene repairs on the final-recipe mix} A checkpoint of this recipe is in-family on the twins and
on 18 reused tasks, so its transfer has to be read on generated tasks.
\item Then the reasoning stages of Sections~\ref{sec:5.5} to \ref{sec:5.7}.
\end{enumerate}

No 27B round is trained before the recipe is settled at 4B, and a 27B round with full coverage was
cancelled before it started. Six questions were open when this was written, each with rounds running
or queued at 4B unless stated:

\begin{itemize}
\item Bidirectional attention over the prompt (Section~\ref{sec:3.6}). \todo[TODO(r6\_4b\_kr20bi,
r6\_4b\_kr23ebi, ft4\_abi, s1\_4b\_bi against s1\_4b\_ca, r6\_4b\_kr23es1bi against
r6\_4b\_kr23es1ca)]{rounds with bidirectional prompt attention against their causal counterparts}
\item Contrast pairs for stance and sarcasm written by other language models, in two versions: 16,036
rows, and 8,859 rows filtered against surface cues. \todo[TODO(r6\_4b\_kr29d, r6\_4b\_kr29c)]{rounds
with the two contrast-pair files}
\item Large files from the original training splits of the twin sources and their relatives (368,053 rows
from Corr2Cause, ProofWriter, RuleTaker, PARARULE-Plus, VitaminC, FEVER-NLI, MTOP, MASSIVE, LogiQA
2.0, ReClor, ConTRoL and WANLI, after 8,385 rows were removed by the protection of the evaluation
sets), with the twin-reserved families at all usable rows. Its checkpoint is in-family on several
twins. \todo[TODO(r6\_4b\_kr27b)]{round with the large original-source files}
\item The public corpus of procedural families from which the leading entry's procedural rows come: ten of
its families, 9,000 rows each, without the two policy families whose templates come close to two
generated tasks of our benchmark. \todo[TODO(r6\_4b\_kr28p)]{round with the public procedural
corpus}
\item A second run of the final recipe, for the spread between two runs on the measures of
Table~\ref{tab:5.14}. \todo[TODO(r6\_4b\_kr20r2)]{repeat of the final-recipe round}
\item The full-coverage round at 9B. \todo[TODO(r6\_9b\_kr23e)]{full-coverage round at 9B}
\end{itemize}

\subsection{Diagnosis: decision training removes the end of reasoning}\label{sec:5.4}

\textbf{Purpose.} The decision data rounds put a loss on one position, the answer letter. Nothing in
them asks the model to write a thought or to end one. This section measures what happens to that
ability, stage by stage, and locates where it is lost.

\textbf{What we observed first.} After the data rounds the three sizes fail in two different ways
when asked to reason. The 4B and the 27B close the thought at once: 42.4\% and 43.6\% of their
thoughts on 5,710 diagnostic items are shorter than 40 tokens. The 9B does the opposite: 29.8\% of
its thoughts end, and the median thought is at the 4,096-token limit, the answer letter repeated to
the end. Thinking replay removes both symptoms. The reader round that follows it brings the second
one back at 4B and 9B: with reasoning on, 57.5\% of the 4B thoughts and 62.9\% of the 9B thoughts in
a full index run reach the limit, at 3,439 and 3,517 tokens per thought.

A longer limit does not help. On 3,021 held-out items that the 4B routes to reasoning, raising the
limit from 4,096 to 16,384 tokens changes the share of thoughts that end by themselves from 11.4\%
to 12.6\%, and 87.4\% are still running at 16,384 tokens (80.8\% of all thoughts in a loop, and half
of the loops have begun after a fifth of the text). Accuracy is unchanged (+0.07 points, interval
$-$0.56 to +0.73, against a 4,096-token run with the loop detector) at 3.9 times the tokens (14,512
against 3,764 per thought). A typical thought has reached its answer and then repeats a line such as
``Wait, I'll choose D.'' until it is cut. The limit is not what keeps these thoughts from ending. A
limit of 8,192 tokens with a loop check gives the same picture on these items, and on the index a
limit of 8,192 tokens scores 67.52 against 67.72 at 4,096 (Table~\ref{tab:5.10}).

\textbf{Probe.} We measure the probability that a model closes a thought at a point where the
thought is complete. For a stored thought we feed the item's prompt and the thought to a model and
read the probability that the closing tag follows within two tokens (directly, or after a line
break). The points are the natural ends of thoughts that their writer closed. Control points at
25\%, 50\% and 75\% of a thought, where no model should close, have a median of 0.00 for every
model. Every stage of a size reads the same thoughts, so differences are differences between stages.

\begin{table}[!htbp]
\renewcommand{\thetable}{5.2}
\centering
\caption{Median probability of closing a thought at its natural end, by training stage (95\% bootstrap interval over thoughts in brackets, based on 400, 300 and 200 thoughts for 4B, 9B and 27B). First line of each size: thoughts written by the base model. Second line: thoughts written by the replayed model. The base 27B could not be loaded for this probe.}\label{tab:5.2}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrrr}
\toprule
{\begin{tabular}[b]{@{}l@{}}\textbf{size, writer of}\\\textbf{the thoughts}\end{tabular}} & \textbf{base model} & \textbf{data rounds} & \textbf{+ reader round} & {\begin{tabular}[b]{@{}r@{}}\textbf{+ thinking}\\\textbf{replay}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{replay +}\\\textbf{reader round}\end{tabular}} \\
\midrule
4B, base & 0.52 {[}0.50, 0.54{]} & 0.52 {[}0.49, 0.54{]} & 0.47 {[}0.43, 0.50{]} & 0.73 {[}0.68, 0.76{]} & 0.26 {[}0.20, 0.30{]} \\
4B, replayed & 0.72 {[}0.68, 0.74{]} & 0.59 {[}0.56, 0.61{]} & 0.64 {[}0.60, 0.66{]} & 0.89 {[}0.87, 0.91{]} & 0.39 {[}0.32, 0.45{]} \\
9B, base & 0.54 {[}0.52, 0.58{]} & 0.06 {[}0.05, 0.06{]} & 0.02 {[}0.01, 0.02{]} & 0.81 {[}0.76, 0.85{]} & 0.18 {[}0.13, 0.21{]} \\
9B, replayed & 0.65 {[}0.61, 0.70{]} & 0.05 {[}0.04, 0.05{]} & 0.02 {[}0.02, 0.02{]} & 0.93 {[}0.90, 0.95{]} & 0.27 {[}0.18, 0.38{]} \\
27B, base & -- & 0.84 {[}0.82, 0.86{]} & -- & 0.97 {[}0.93, 0.98{]} & 0.54 {[}0.50, 0.61{]} \\
27B, replayed & -- & 0.86 {[}0.83, 0.88{]} & -- & 0.98 {[}0.97, 0.99{]} & 0.87 {[}0.83, 0.91{]} \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\begin{figure}[!htbp]
\renewcommand{\thefigure}{5.1}
\centering
\adjincludegraphics[max width=\linewidth,max height=0.5\textheight]{figures/fig10_closing.pdf}
\caption{Where the end of a thought is lost. (a--c) Probability of closing a thought at its natural end for every training stage of the 4B, 9B and 27B lines (median over thoughts and 95\% bootstrap interval, with circles for thoughts written by the base model and triangles for thoughts written by the replayed model). (d) Share of thoughts that end by themselves when each 4B stage writes its own thoughts on the same 3,021 held-out items (4,096-token limit, no loop detector).}\label{fig:5.1}
\end{figure}

A stage with a loss on the answer letter only leaves the closing decision unsupervised, and it can
drift. At 9B the data rounds alone take the probability from 0.54 to 0.06, with no thought above
0.5. At 4B the data rounds leave it where the base model has it (0.52), and the reader round that
follows replay takes it from 0.73 to 0.26. At 27B the same round takes it from 0.97 to 0.54 on
base-written thoughts. The one stage that has a loss on the closing tag, thinking replay, restores
it at every size (0.73, 0.81, 0.97). The final 27B also drifts the other way: a quarter of the way
into a thought the closing tag is its most likely next token in 22\% of the cases (0\% after
replay), which is the ``closes at once'' symptom.

The behaviour agrees with the probe. Table~\ref{tab:5.3} lets every 4B stage write its own thoughts
on the same items. The base model ends 91.1\% of them. After thinking replay 74.6\% end and 2.5\%
loop. After the reader round that follows, 11.4\% end and 63.6\% loop. Without replay the reader
round does no such harm (96.5\% end), but those thoughts are a few lines long.

\begin{table}[!htbp]
\renewcommand{\thetable}{5.3}
\centering
\caption{Thoughts of each 4B stage on the 3,021 held-out items that the replay-and-reader model routes to reasoning (own thoughts, 4,096-token limit, no loop detector).}\label{tab:5.3}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrr}
\toprule
\textbf{4B stage} & {\begin{tabular}[b]{@{}r@{}}\textbf{thoughts}\\\textbf{that end}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{in a loop}\\\textbf{at the}\\\textbf{limit}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{tokens per}\\\textbf{thought, mean}\\\textbf{/ median}\end{tabular}} \\
\midrule
base model & 91.1\% & 0.4\% & 1,093 / 564 \\
data rounds & 92.4\% & 2.8\% & 639 / 265 \\
data rounds + reader round & 96.5\% & 3.0\% & 336 / 163 \\
data rounds + thinking replay & 74.6\% & 2.5\% & 2,397 / 2,435 \\
data rounds + thinking replay + reader round & 11.4\% & 63.6\% & 3,764 / 4,096 \\
\ldots{} + stop step & 85.9\% & 10.1\% & 1,413 / 768 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

A loop sustains itself. Inside a loop no model closes the thought, the base model included: at the
start of the loop and at its end the median closing probability is 0.00 for all five stages (311
looping thoughts), and so it is at the point just before the looping line is written for the first
time (497 thoughts). Once a text repeats, repetition is what every model of the family predicts
next. What differs between stages is whether the thought is closed at its first conclusion. After
that the stages are alike.

What the reader round changes is not the reverse of what replay changed. The weight update of the
reader round has a cosine of $-$0.0022 with the update of thinking replay (200 adapted matrices of
the 4B). A reader round trained without replay has $-$0.0002. The two updates are close to
orthogonal: the reader round does not undo the replay, it moves something else that the closing
decision depends on. We have not identified what.

\subsection{Restoring reasoning before the answer: thinking replay}\label{sec:5.5}

\textbf{Purpose.} Give the decision model back the reasoning of the model it was trained from, in
the same weights.

\textbf{Data.} The base model of the same size writes reasoning samples for training items (several
per item, 4,096-token limit). The decision model reads its answer after each sample. For every item
we keep the best sample that ended by itself within 3,000 tokens, if it raises the bounded log score
of the decision model's readout by more than a margin after a price per token. The target is that
reasoning followed by the closing tag. This gives 15,870 targets at 4B, 16,369 at 9B and 4,395 at
27B, where the decision model is already sure on more than half of the items and the base model
writes short thoughts.  At inference there is one model. The base model appears only in this
training data.

\textbf{Method and settings.} A rank-64 adapter on all projection matrices, language-model loss on
the reasoning and the closing tag only, one epoch at a learning rate of 1e-4 (247 steps of 64
sequences at 4B), merged into the weights. Settings of this and the following stages: \todo{Table
F.10, from the trainer logs}.

\textbf{Result after the stage.} Table~\ref{tab:5.4} compares each final model with its replayed
version before any reader round. Replay removes both ways in which a decision-trained model stops
reasoning, and costs two to five points of the one-pass answer, which the next stage returns.

\begin{table}[!htbp]
\renewcommand{\thetable}{5.4}
\centering
\caption{Reasoning before and after thinking replay (5,710 diagnostic items of benchmark type, each model reading its own thought, one sample per item, 4,096-token limit). Knowledge families: the 1,350 items of ten knowledge and reasoning benchmarks.}\label{tab:5.4}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrrrr}
\toprule
\textbf{writer} & {\begin{tabular}[b]{@{}r@{}}\textbf{tokens per}\\\textbf{thought, mean}\\\textbf{/ median}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{under}\\\textbf{40}\\\textbf{tokens}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{thoughts}\\\textbf{that end}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{one}\\\textbf{pass}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{after}\\\textbf{thought}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{knowledge}\\\textbf{families: one pass}\\\textbf{$\rightarrow$ after thought}\end{tabular}} \\
\midrule
4B after data rounds & 473 / 139 & 42.4\% & 94.3\% & 72.9 & 74.1 & 63.6 $\rightarrow$ 67.5 \\
4B after replay & 1,976 / 1,399 & 0.0\% & 78.4\% & 70.1 & 74.4 & 55.5 $\rightarrow$ 71.3 \\
9B after data rounds & 2,970 / 4,096 & 7.4\% & 29.8\% & 75.0 & 75.6 & 65.6 $\rightarrow$ 68.9 \\
9B after replay & 1,803 / 1,110 & 0.0\% & 81.5\% & 69.7 & 75.7 & 56.8 $\rightarrow$ 71.9 \\
27B after data rounds & 434 / 135 & 43.6\% & 97.3\% & 77.4 & 78.1 & 69.0 $\rightarrow$ 74.6 \\
27B after replay & 881 / 236 & 0.1\% & 90.4\% & 75.6 & 78.3 & 65.5 $\rightarrow$ 76.7 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\subsection{Reading one's own reasoning: the reader round}\label{sec:5.6}

\textbf{Purpose.} After replay the model reasons, but its one-pass answer has moved and it has never
been trained to give its answer after a thought of its own. The reader round trains both readouts.

\textbf{Data.} Two kinds of rows from training items, one reasoning sample per item written by the
model itself. The first has the item with the last 4,000 characters of the thought, with the item's
label as target. The second is the item alone, with the one-pass distribution of the model before
replay as a soft target, which holds the one-pass answer in place. A reader that has not seen
thoughts cannot use them: on the held-out items of Table~\ref{tab:5.3}, the final 4B reading the
base model's thoughts is 8.4 points below the reader-round model reading the same thoughts (67.06
against 75.47, Table~\ref{tab:5.5}).

\textbf{Method and settings.} The decision trainer of the data rounds: a rank-64 adapter, soft
cross-entropy on the option letters, one epoch at 5e-5 (481 steps at 4B). The loss is on the answer
letter only.

\textbf{Result after the stage.} On the diagnostic items the 4B has its one-pass answer back (72.7
against 70.1 after replay and 72.9 before it), a thought answer of 75.6 and 75.9 for the default
control, against 74.0 for the reader round without replay. The 9B has 76.9 against 75.6. The chain
scores 67.72 at 4B and 69.77 at 9B on the index: against one pass, code execution rises from 28.7 to
80.5 skill points at 4B and from 37.1 to 81.6 at 9B (with the reader round alone: 37.1 at 4B and
56.0 at 9B), a graduate-level science set from 23.1 to 51.7 at 4B. At 27B the chain scores 72.34
against 70.43 in one pass: in raw scores code execution rises from 76.5 to 96.1, the graduate-level
science set from 50.0 to 69.4, MMLU-Pro from 69.5 to 82.3 and API-Bank from 81.5 to 88.2. The
largest losses are the home-appliance simulator (100.0 $\rightarrow$ 94.3), SATA-Bench (59.0
$\rightarrow$ 55.0), MuSR (72.5 $\rightarrow$ 68.9) and the Habermas set (63.7 $\rightarrow$ 60.3).

\textbf{What it costs.} This is the stage that removes the end of the thought at 4B and 9B. The gain
above is obtained there with thoughts of 3,439 (4B) and 3,517 (9B) tokens, 57.5\% and 62.9\% of them
cut at the limit (1,144 and 1,049 reasoning tokens per answer), and with small losses on tool and
language benchmarks (Section~\ref{sec:6.12}). The 27B is not affected in the same way: its thoughts
have 710 tokens, 6.0\% reach the limit, and an answer costs 193 reasoning tokens on average, with
27.2\% of the answers thought about. This agrees with the probe of Table~\ref{tab:5.2}, where the
reader round leaves the 27B a closing probability of 0.54 against 0.26 and 0.18 for the smaller
sizes.

\subsection{Stopping when finished: the stop step}\label{sec:5.7}

\textbf{Purpose.} Teach the model to end a thought when it is finished. No written example exists
for this: the base model's thoughts were written for the base model, and an item on which a thought
loops gives no target. The signal has to come from the outcome: whether the answer still changes,
and what the tokens cost.

\textbf{Data.} The model writes four thoughts for each of 14,911 training items. We read its answer
after every eighth of each thought. A thought is finished at the first eighth after which the
readout no longer changes (same top answer, total variation at most 0.1 to the final readout). Of
59,644 thoughts, 58,357 are finished before their end, and in 61\% of the selected targets the
answer is final after the first eighth. For every item the sample with the best score (the gain of
the readout at the finishing point over the one-pass answer, minus a price per token) is kept if the
score exceeds a margin, cut at its finishing point at the end of the line, and given the closing
tag: 5,311 targets with a mean of 555 tokens, 2,950 of them from thoughts that had run to the limit.

\textbf{Method and settings.} As thinking replay, on the model after the reader round: rank-64
adapter, language-model loss on the target, one epoch at 5e-5, 82 steps at 4B.

\textbf{Result after the stage.} On the held-out items 85.9\% of the thoughts end by themselves
instead of 11.4\%, at 1,413 instead of 3,764 tokens, and the accuracy of the default control is
75.31 against 75.54 (difference $-$0.23, interval $-$0.96 to +0.50). Of the 2,678 thoughts the model
had left open, 84.1\% now end, with unchanged accuracy on those items (73.38 $\rightarrow$ 73.23).
For the diagnostic items 88.2\% end (median 615 tokens), the one-pass answer is 72.9 and the default
control 75.2 against 75.9. The 4B after the stop step scores 67.37 on the index against 67.72 before
it: 10.4\% of its thoughts reach the limit instead of 57.5\%, a thought has 1,585 tokens instead of
3,439, and an answer costs 497 reasoning tokens instead of 1,144. The 0.35 points are lost in the
knowledge area (55.7 against 57.0). At 9B the stop step raises the index from 69.77 to 70.16: 15.8\%
of the thoughts reach the limit instead of 62.9\%, a thought has 1,900 tokens instead of 3,517, an
answer costs 552 reasoning tokens instead of 1,049, and the areas that long loops had cost come back
(tools 86.9 against 85.2, knowledge 59.1 against 58.6).

\textbf{With a loop check at inference.} The stop step leaves 14.1\% of the 4B's thoughts open at
the limit on the held-out items. A check for repetition every 256 tokens, which needs no training,
takes most of them: 83.9\% of the thoughts end by themselves, 12.6\% are cut at a loop and 3.5\%
stay open, at 1,186 instead of 1,413 tokens per thought, and the default answer is 75.60 against
75.31 (+0.30, interval $-$0.40 to +0.99). With the limit at 8,192 tokens and the check, 0.7\% stay
open (75.37, 1,251 tokens). On the model before the stop step the same check leaves 24.1\% open
instead of 88.6\% at an unchanged default answer (75.54), but at 2,916 tokens per thought: the check
ends a loop after it has begun, while the stop step ends the thought before it. These are held-out
measurements. The check has not been measured on the index.

\textbf{What else we tried at this stage.} Table~\ref{tab:5.5} lists inference-time measures on the
same items. Cutting every thought at 1,024 tokens and reading the answer there gives the reference
accuracy at a quarter of the tokens on these items. On the index the same cut costs 0.79 points
(66.93), all of it in the knowledge area (53.8 against 57.0), so the long thoughts of the hard
knowledge benchmarks are not all repetition, and the held-out items under-represent them. A
repetition penalty with a loop detector ends more thoughts and loses half a point. A variant of the
stop step with additional short ``check and close'' targets ends as many thoughts and is 0.6 lower
on the diagnostic items (74.6 against 75.2). Table~\ref{tab:5.6} compares the designs on the full
index.

\begin{table}[!htbp]
\renewcommand{\thetable}{5.5}
\centering
\caption{Ways to deal with thoughts that do not end, 4B after thinking replay and reader round, 3,021 held-out items (differences to the first row with 95\% bootstrap intervals over items).}\label{tab:5.5}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.3964}}>{\raggedleft\arraybackslash}p{\mdw{0.1729}}>{\raggedleft\arraybackslash}p{\mdw{0.1438}}>{\raggedleft\arraybackslash}p{\mdw{0.1198}}>{\raggedleft\arraybackslash}p{\mdw{0.1537}}}
\toprule
\textbf{setting} & \textbf{thoughts that end} & \textbf{tokens per thought} & \textbf{default control} & \textbf{difference} \\
\midrule
limit 4,096 (reference) & 11.4\% & 3,764 & 75.54 & -- \\
limit 16,384 & 12.6\% & 14,512 & 75.31 \textsuperscript{c} & +0.07 {[}$-$0.56, +0.73{]} \textsuperscript{c} \\
limit 16,384 with loop detector & 12.9\% (80.6\% cut at a loop) & 4,287 & 75.60 \textsuperscript{c} & +0.36 {[}$-$0.23, +0.96{]} \textsuperscript{c} \\
thought cut at 1,024 tokens & -- & 992 & 75.54 & +0.00 {[}$-$0.60, +0.63{]} \\
thought cut at 512 tokens & -- & 508 & 75.21 & $-$0.33 {[}$-$1.06, +0.36{]} \\
repetition penalty 1.1 with loop detector & 27.6\% (29.0\% cut at a loop) & 3,360 & 75.01 & $-$0.53 {[}$-$1.16, +0.10{]} \\
stop step (trained) & 85.9\% & 1,413 & 75.31 & $-$0.23 {[}$-$0.96, +0.50{]} \\
base model writes the thought, a model with the reader round (no replay) reads it & 91.1\% & 1,093 & 75.47 & $-$0.07 {[}$-$1.19, +1.06{]} \\
base model writes the thought, the model of the first row reads it & 91.1\% & 1,093 & 74.98 & $-$0.56 {[}$-$1.42, +0.30{]} \\
base model writes the thought, the data-round model reads it (no reader round) & 91.1\% & 1,093 & 67.06 & $-$8.47 {[}$-$9.96, $-$6.95{]} \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{c} measured in a separate run with its own reference with the loop detector
(75.24). The difference is to that reference.\par}
\end{table}

\begin{table}[!htbp]
\renewcommand{\thetable}{5.6}
\centering
\caption{Every reasoning design of this chapter on the full index, 4B (Decision Index 0.2.1, default control, 4,096-token limit, one run each). ``Reasoning tokens per answer'' is the mean over all answers, including those that are not thought about. One pass: 64.78 (knowledge 45.4, tools 86.0).}\label{tab:5.6}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.2466}}>{\raggedleft\arraybackslash}p{\mdw{0.0701}}>{\raggedleft\arraybackslash}p{\mdw{0.1148}}>{\raggedleft\arraybackslash}p{\mdw{0.0639}}>{\raggedleft\arraybackslash}p{\mdw{0.1189}}>{\raggedleft\arraybackslash}p{\mdw{0.1120}}>{\raggedleft\arraybackslash}p{\mdw{0.1219}}>{\raggedleft\arraybackslash}p{\mdw{0.1394}}}
\toprule
\textbf{design (4B)} & \textbf{index} & \textbf{knowledge} & \textbf{tools} & \textbf{answers thought about} & \textbf{tokens per thought} & \textbf{thoughts at the limit} & \textbf{reasoning tokens per answer} \\
\midrule
reader round only (no replay) & 66.38 & 50.0 & 86.1 & 32.2\% & 388 & 0.6\% & 125 \\
replay, then reader round & \textbf{67.72} & 57.0 & 85.3 & 33.3\% & 3,439 & 57.5\% & 1,144 \\
\ldots{} thought cut at 1,024 tokens & 66.93 & 53.8 & 85.2 & 33.2\% & 1,003 & -- & 333 \\
\ldots{} + stop step & 67.37 & 55.7 & 85.2 & 31.3\% & 1,585 & 10.4\% & 497 \\
\ldots{} + stop step + reinforcement learning, rollouts sampled at temperature 1 (Section~\ref{sec:5.9}) \textsuperscript{f} & 67.23 & 55.1 & 84.8 & 31.4\% & 1,053 & 3.2\% & 330 \\
\ldots{} + stop step + reinforcement learning, rollouts sampled as at inference & 66.80 & \textsuperscript{g} & \textsuperscript{g} & 32.5\% & 617 & 0.4\% & 200 \\
\ldots{} + stop step + readout trained on thoughts sampled by the current model & 67.43 & 55.6 & 85.4 & 31.1\% & 1,845 & 13.9\% & 574 \\
base model writes the thought, the model of row 2 reads it & 67.62 & 57.7 & 84.3 & 33.2\% & 1,316 & 8.7\% & 438 \\
joint stage from the data-round model (Section~\ref{sec:5.8}) & 67.11 & 57.0 & 84.0 & 47.0\% & 2,666 & 39.9\% & 1,254 \\
\ldots{} + stop step & 66.42 & 55.7 & 83.0 & 44.3\% & 1,631 & 13.6\% & 723 \\
reinforcement learning from the data-round model \textsuperscript{e} & 67.18 & 53.5 & 86.2 & 31.1\% & 184 & 0.7\% & 57 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{e} 78.5\% of this model's thoughts on the index have fewer than 16 tokens: it skips
most of the questions it is asked to reason about, and its row is the score of a system that mostly
does not reason. \textsuperscript{f} 2.1\% of the thoughts have fewer than 16 tokens (0.9\% after
the stop step alone, none before it), and 57\% have 128 to 1,023 tokens. \textsuperscript{g}
\todo[TODO(rl4t06s6\_di)]{knowledge and tools values of this run}\par}
\end{table}

\subsection{The joint variant}\label{sec:5.8}

\textbf{Purpose.} Sections~\ref{sec:5.5} to \ref{sec:5.7} are repairs in sequence, each of which
moves what the previous one fixed. The joint variant replaces them by one stage in which every step
holds thinking targets and readout targets.

\textbf{Data and method.} 15,870 thinking targets, 16,000 readouts after a thought and 16,000
one-pass readouts with soft targets. A rank-64 adapter with a language-model loss on the thinking
rows and a soft cross-entropy on the option letters for the readout rows, each row counting once,
for 747 steps. Before training we check that the starting model gives the target's top answer at the
readout position (97.8\% of the one-pass rows, 96.4\% of the rows after a thought). Two arms: from
the 4B after the data rounds (1e-4), and from the replayed 4B (5e-5).

\textbf{Result.} Table~\ref{tab:5.7}. On the diagnostic items the second joint arm gives the best
default control of all designs (76.5 for the second arm against 75.9 for the sequence), with a
one-pass answer within a point of the starting model and no reader round. They are below the
sequence on the held-out items, the first arm significantly ($-$1.95, interval $-$3.11 to $-$0.76):
its one-pass answer on the sources that the data rounds added is about one point lower. A stage with
32,000 readout rows does not hold what 1.1 million decision rows taught. The joint stage improves
reasoning on benchmark-type questions and pays on the training distribution. It belongs inside the
full data round, which we have not run. The index agrees with the held-out items: the first arm
scores 67.11, with the knowledge area level with the sequence (57.0) and retrieval 3.7 points lower
(67.5 against 71.2). Its gate fires on 47\% of the answers instead of 33\%, a sign that the one-pass
answer moved. A stop step on top of it ends more thoughts and scores 66.42. The second arm was not
run on the index.

\begin{table}[!htbp]
\renewcommand{\thetable}{5.7}
\centering
\caption{Joint stage against the sequence (4B).}\label{tab:5.7}
{\footnotesize\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrrrr}
\toprule
\textbf{4B model} & {\begin{tabular}[b]{@{}r@{}}\textbf{diagnostic}\\\textbf{items: thoughts}\\\textbf{that end}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{one}\\\textbf{pass}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{default}\\\textbf{control}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{held-out items:}\\\textbf{thoughts that}\\\textbf{end}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{tokens}\\\textbf{per}\\\textbf{thought}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{default}\\\textbf{control}\end{tabular}} \\
\midrule
replay, then reader round & -- \textsuperscript{d} & 72.7 & 75.9 & 11.4\% & 3,764 & 75.54 \\
replay, reader round, stop step & 88.2\% & 72.9 & 75.2 & 85.9\% & 1,413 & 75.31 \\
joint stage from the data-round model & 67.8\% & 72.0 & 75.6 & 57.3\% & 2,740 & 73.58 \\
joint stage from the replayed model & 72.7\% & 73.2 & 76.5 & 64.3\% & 2,613 & 74.91 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{d} the diagnostic thoughts of this row were written by the replayed model before
its reader round (78.4\% end).\par}
\end{table}

\subsection{Reinforcement-learning variants}\label{sec:5.9}

\textbf{Purpose.} Training on outcomes instead of examples is the natural tool for the two things no
example shows: when to stop and whether to think. The stop step is its simplest form (sample, score
by outcome, keep the best, imitate). We also trained the thinker with a policy gradient, in several
arms with controls. The result in two sentences: started from a model that reasons, and with a
proper score as reward, this training makes nearly every thought end at about a third of the tokens
and, mostly through the shorter thoughts, calibrates the answer that is read after the thought, at
an accuracy within a third of a point of the start on held-out items and about 0.6 points lower on
the index. In no arm has it made the answers better than those of the supervised stages.

\textbf{Method.} Group-relative policy gradient on the tokens of the thought. In one iteration the
model writes 8 thoughts (rollouts) for each of 64 prompts, and the answer is read after each. A
thought is reinforced by how far its reward lies above that of the other thoughts for the same
prompt. The reward is an outcome term minus a price for length. The outcome term is the gain of the
read-out after the thought over the one-pass read-out, measured with the log score or with a bounded
proper score that gives partial credit for a near miss. The first arms used a price of 1e-4 per
token, a learning rate of 1e-5, a penalty of 0.02 towards the starting policy and 120 iterations.
Unless stated, only the thinker is trained and the read-out stays as it is. The prompts are drawn
from a pool of 26,931 items whose one-pass top probability is below 0.9. What the pool holds is
described at the end of this section. Results are on the 3,021 routed held-out items of the training
distribution (Table~\ref{tab:5.11}) and, for four 4B arms and one 9B arm, on the index
(Table~\ref{tab:5.6} and the text below).

\textbf{What we ran earlier.} Group-relative policy gradient on the reasoning tokens with the
readout's log-score gain as reward. With a length penalty and normalisation by the group's standard
deviation the thoughts collapsed to about 230 tokens with negative value. Without that normalisation
and with a penalty towards the starting policy, training was stable and slow: the share of thoughts
that end rose from 31\% to 37\% in 49 iterations. In those runs 12.5\% of the prompts had samples
that differed in correctness. On 4,997 common index items the answer after thinking was 72.7 and
72.4 at two checkpoints against 73.2 before training (Section~\ref{sec:9.1}). \todo{the four numbers
of this paragraph are from the notebook of 3 to 5 October; attach the trainer logs}

From a model that hardly reasons, the policy learns to skip. The first arm starts from the 4B after
the data rounds (reinforcement learning in place of the three repair stages). On the held-out items
it closes the thought at once on 66.3\% of them, writes 65 to 512 tokens on 22.1\% and more than 512
on 11.4\%, most on medical questions, code tracing and the hard pool (700 to 870 tokens on average).
Against its starting model the answer after the thought rises from 72.29 to 74.25 (+1.95, interval
+0.73 to +3.21) and the default answer from 74.02 to 75.41 (+1.39, +0.26 to +2.48), at 255 instead
of 639 tokens per thought. Against the sequence of replay and reader round it is level (75.41
against 75.54, $-$0.13, $-$1.32 to +1.09). This is the one arm whose answers improved over its own
start, and what it learned is where to skip, not how to reason: on the questions where it does
write, its answers are weaker than those of the replayed thinker (81.6 against 85.0 on the same
held-out items). Its index score is 67.18 with 57 reasoning tokens per answer, 0.80 above the
reader-round-only model and 0.54 below the sequence, with 53.5 against 57.0 in the knowledge area,
and 78.5\% of its thoughts there have fewer than 16 tokens. Two things produce the skipping. The
start is a model that already closed 42\% of its thoughts at once, so its samples offer skipping far
more often than good reasoning. And in the reward an empty thought scores exactly zero, while a
written one can lose and pays for its tokens. We do not count this arm as a model that reasons
before it answers. Two further starts gave nothing: from the joint model the result is 73.75, and
from the model after thinking replay and reader round, whose rollouts close in 43\% of the cases,
the reward did not move in 120 iterations: a policy whose samples do not end gives the gradient
nothing to choose from.

\begingroup\renewcommand{\thetable}{5.11}\captionsetup{hypcap=false}
\par\medskip
\captionof{table}{Reinforcement learning of the thinker on held-out items (the 3,021 routed held-out items of the training distribution, one thought per item with the decoding of inference, 4,096-token limit, accuracy in percent). \emph{Block A:} thoughts and accuracy. ``Rollouts'': how the thoughts were sampled in training, at temperature 1 or with the decoding of inference (temperature 0.6, top-p 0.95, top-k 20). Last column: paired difference to the arm's starting model with its 95\% interval, T for the answer after the thought and D for the default answer. For the arms that start from a stop-trained model it is computed on the test part of the items, after a temperature has been fitted on the other part (2,132 test items at 4B). Rows with an open-item marker are arms that were running when this was written. \emph{Block B:} calibration of the answer after the thought for the starting models and the arms with the bounded proper score, on the same items. Stated confidence, overconfidence (stated confidence minus accuracy), calibration error, Brier score and log score are read before any temperature is fitted. ``Fitted temperature'' is the temperature that calibrates this read-out. The area under the risk--coverage curve (lower is better) and the share of answers that can be accepted at an error of 5\% are read after the temperature has been fitted, on the test part of the items.}\label{tab:5.11}
\endgroup
\begingroup
\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\begin{longtable}{>{\raggedright\arraybackslash}p{\mdw{0.1238}}>{\raggedright\arraybackslash}p{\mdw{0.1342}}>{\raggedright\arraybackslash}p{\mdw{0.1190}}>{\raggedleft\arraybackslash}p{\mdw{0.1657}}>{\raggedleft\arraybackslash}p{\mdw{0.1039}}>{\raggedleft\arraybackslash}p{\mdw{0.1031}}>{\raggedleft\arraybackslash}p{\mdw{0.0955}}>{\raggedright\arraybackslash}p{\mdw{0.1424}}}
\toprule
\textbf{size and start} & \textbf{outcome term of the reward} & \textbf{rollouts} & \textbf{thoughts that end} & \textbf{tokens per thought} & \textbf{after the thought} & \textbf{default answer} & \textbf{paired difference to the start} \\
\midrule
\endhead
\bottomrule
\endfoot
4B after the data rounds (start) & -- & -- & 92.4\% & 639 & 72.29 & 74.02 & -- \\
\ldots{} trained & log score & temperature 1 & 97.6\% (66.3\% of all thoughts closed at once) & 255 & 74.25 & 75.41 & T +1.95 {[}+0.73, +3.21{]}, D +1.39 {[}+0.26, +2.48{]} \\
4B after the stop step (start) & -- & -- & 85.9\% & 1,413 & 74.38 & 75.31 & -- \\
\ldots{} trained & log score, first run & temperature 1 & 80.3\% & 1,752 & -- & 75.31 & -- \\
\ldots{} trained & log score, repeat \textsuperscript{a} & temperature 1 & 74.5\% & 1,953 & -- & -- & T $-$1.08 {[}$-$2.02, $-$0.28{]} \\
\ldots{} trained & bounded proper score, three runs & temperature 1 & 96.7 / 98.2 / 97.9\% & 853 / 733 / 798 & 74.25 / 74.28 / 74.68 & 75.11 / 75.04 / 75.84 & first run: T $-$0.70 {[}$-$1.59, +0.14{]} \\
\ldots{} control & none (price only) & temperature 1 & 99.3\% & 482 & 73.49 & 74.54 & -- \\
\ldots{} control & noise & temperature 1 & 99.2\% & 600 & 73.68 & 74.08 & T $-$1.22 {[}$-$2.25, $-$0.14{]}, D $-$1.64 {[}$-$2.81, $-$0.80{]} \\
\ldots{} trained & bounded proper score & as at inference & 99.7\% & 503 & 74.11 & 75.07 & T $-$1.17 {[}$-$2.11, $-$0.28{]}, D $-$0.75 {[}$-$1.74, 0.00{]} \\
\ldots{} control & accuracy of the answer in place of the proper score & as at inference & 99.8\% & 433 & 73.78 & 74.71 & T $-$1.64 {[}$-$2.67, $-$0.66{]}, D $-$1.36 {[}$-$2.30, $-$0.56{]} \\
\ldots{} trained & bounded proper score, no price for length & as at inference & 59.4\% (40.6\% at the limit) & 2,581 & 74.58 & 75.50 & T $-$0.70 {[}$-$1.69, +0.19{]}, D $-$0.42 {[}$-$1.22, +0.33{]} \\
4B after thinking replay and reader round (start) & -- & -- & 11.4\% & 3,764 & 75.04 & 75.54 & -- \\
\ldots{} trained & bounded proper score & as at inference & 58.0\% (42.0\% at the limit) & 2,753 & 74.18 & 74.94 & T $-$0.86 {[}$-$1.82, +0.03{]}, D $-$0.60 {[}$-$1.32, +0.13{]} \textsuperscript{b} \\
9B after the stop step (start) & -- & -- & 77.7\% & 1,677 & 81.20 & 82.06 & -- \\
\ldots{} trained & bounded proper score & temperature 1 & 91.4\% & 1,169 & 80.97 & 81.99 & T $-$0.28 {[}$-$0.84, +0.23{]}, D 0.00 {[}$-$0.61, +0.52{]} \\
\ldots{} trained & bounded proper score & as at inference & 99.8\% & 544 & 80.87 & 81.60 & T $-$0.14 {[}$-$0.84, +0.56{]}, D $-$0.75 {[}$-$1.27, $-$0.14{]} \\
\ldots{} control & accuracy of the answer in place of the proper score & as at inference & \todo[TODO(rl9\_ei2\_acc\_t06)]{held-out result and calibration of the accuracy-reward control at 9B} &  &  &  &  \\
\end{longtable}
\endgroup
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{a} share of thoughts that end and tokens per thought on the test part of the items.
\textsuperscript{b} against its own start, the model after thinking replay and reader round. Its
calibration is discussed in the text.\par}
\begingroup
\scriptsize\setlength{\tabcolsep}{3pt}\renewcommand{\arraystretch}{1.1}
\begin{longtable}{>{\raggedright\arraybackslash}p{\mdw{0.0790}}>{\raggedright\arraybackslash}p{\mdw{0.0970}}>{\raggedleft\arraybackslash}p{\mdw{0.0816}}>{\raggedleft\arraybackslash}p{\mdw{0.0959}}>{\raggedleft\arraybackslash}p{\mdw{0.1283}}>{\raggedleft\arraybackslash}p{\mdw{0.0982}}>{\raggedleft\arraybackslash}p{\mdw{0.0575}}>{\raggedleft\arraybackslash}p{\mdw{0.0690}}>{\raggedleft\arraybackslash}p{\mdw{0.1104}}>{\raggedleft\arraybackslash}p{\mdw{0.0857}}>{\raggedleft\arraybackslash}p{\mdw{0.0845}}}
\toprule
\textbf{B. answer after the thought} & \textbf{rollouts} & \textbf{accuracy} & \textbf{stated confidence} & \textbf{overconfidence} & \textbf{calibration error} & \textbf{Brier score} & \textbf{log score} & \textbf{fitted temperature} & \textbf{area under the risk--coverage curve} & \textbf{accepted at an error of 5\%} \\
\midrule
\endhead
\bottomrule
\endfoot
4B after the stop step (start) & -- & 74.38 & 83.70 & +9.32 & 9.43 & 0.3713 & $-$0.7302 & 1.55 & 0.1172 & 20.5\% \\
\ldots{} trained, bounded proper score & as at inference & 74.11 & 80.27 & +6.15 & 6.38 & 0.3642 & $-$0.6918 & 1.35 & 0.1201 & 18.0\% \\
9B after the stop step (start) & -- & 81.20 & 84.27 & +3.07 & 3.77 & -- & -- & 1.23 & 0.0528 & 63.1\% \\
\ldots{} trained, bounded proper score & temperature 1 & 80.97 & -- & -- & 3.76 & -- & -- & -- & -- & -- \\
\ldots{} trained, bounded proper score & as at inference & 80.87 & 81.91 & +1.04 & 2.14 & 0.2577 & $-$0.4848 & 1.05 & 0.0527 & 60.2\% \\
\end{longtable}
\endgroup

``--'' in block B: not given in our record of the run.

From a model that reasons, the price shortens the thoughts and the outcome term holds the accuracy.
With the bounded score, three runs from the stop-trained 4B end 96.7 to 98.2\% of the thoughts
instead of 85.9\%, at 733 to 853 tokens instead of 1,413, with the default answer at 75.04 to 75.84
against 75.31. Two controls show which part of the reward does this. With the price alone 99.3\% of
the thoughts end at 482 tokens, and the default answer falls to 74.54. With noise in place of the
outcome term 99.2\% end at 600 tokens, and the default answer falls to 74.08. On the test part the
noise arm loses 1.22 points after the thought (interval $-$2.25 to $-$0.14) and 1.64 on the default
answer ($-$2.81 to $-$0.80), and its area under the risk--coverage curve rises by 0.011. So the
shortening comes from the price, and the outcome term keeps about half a point to a point of
accuracy over the controls. The paired intervals of these two differences have not been computed
\todo[TODO(paired intervals of the outcome reward against the price-only control and against the
noise control)]{}. The score has to be bounded: with the log score the thoughts grow, to 1,752
tokens with 80.3\% ending in the first run and to 1,953 tokens with 74.5\% ending in its repeat.
Most of what these runs change is the length of the thought.

Sampling the rollouts as at inference makes nearly every thought end. At temperature 1, 99\% of the
rollouts end from the first iteration and their length hardly changes in training (563 to 530
tokens), so the gradient does not see the loops that occur with the decoding of the served model. In
the next arm the rollouts are sampled with that decoding and its token limit. The gradient estimate
is then biased, because the samples come from a truncated distribution, so we judge the arm by its
held-out result. At 4B 99.7\% of the thoughts end by themselves, 0.3\% are open at the limit and
0.7\% are closed at once without text. A thought has 503 tokens on average (median 435, 90th
percentile 812) against 1,413 before. The answer after the thought is 74.11 against 74.38 and the
default answer 75.07 against 75.31. On the test part the differences are $-$1.17 (interval $-$2.11
to $-$0.28) and $-$0.75 ($-$1.74 to 0.00). At 9B the same arm ends 99.8\% of the thoughts (77.7\%
before, 91.4\% with rollouts at temperature 1) at 544 tokens (1,677 and 1,169), with 80.87 after the
thought against 81.20 and a default answer of 81.60 against 82.06 (on the test part $-$0.75, $-$1.27
to $-$0.14).

With a proper score as reward, the same training calibrates the answer after the thought. The
accuracies above hide a second effect. It shows when the read-out after the thought is taken as the
model gives it, before any temperature is fitted (Table~\ref{tab:5.11}, block B). The stop-trained
4B is right on 74.38\% of the routed held-out items and states 83.70\% on average: it is
overconfident by 9.32 points, with a calibration error of 9.43. After training with the bounded
proper score and rollouts sampled as at inference it is right on 74.11\% and states 80.27\%. The
overconfidence is 6.15 points and the calibration error 6.38, the Brier score falls from 0.3713 to
0.3642, the log score rises from $-$0.7302 to $-$0.6918, and the temperature that has to be fitted
afterwards falls from 1.55 to 1.35. At 9B the overconfidence falls from 3.07 to 1.04 points, the
calibration error from 3.77 to 2.14 and the fitted temperature from 1.23 to 1.05, at 81.20\% and
80.87\% right. The calibration error is a third lower at 4B ($-$32\%) and more than two fifths lower
at 9B ($-$43\%), while the accuracy stays within a third of a point of its start.
\citet{gao2026openjev} report this for a proper-score reward: a calibrated read-out at the accuracy
of the baseline. Two limits belong next to the result. The reward alone does not produce it: with
the same reward and rollouts sampled at temperature 1, the 9B's calibration error stays where it was
(3.76). And the training does not improve the ranking of right and wrong answers. The area under the
risk--coverage curve is 0.1172 before and 0.1201 after at 4B, and 0.0528 and 0.0527 at 9B. The share
of answers that a caller can accept at an error of 5\%, once a temperature is fitted, is 20.5\%
before and 18.0\% after at 4B, and 63.1\% and 60.2\% at 9B. A better-calibrated read-out helps a
caller who takes the stated probability as it is. It does not let more answers through a fixed error
bound. On the rebuilt GSM8K rows, where every item gets a thought, the read-out is near the ceiling
before and after (at 4B accuracy 95.2 $\rightarrow$ 93.4 and share accepted at an error of 5\% 100\%
$\rightarrow$ 97.9\%, at 9B accuracy 96.7 before and after), so those rows cannot show the effect.

\emph{The two controls.} What calibrates (the proper score, or the sampling and the shorter thoughts
that come with this arm) is not shown by a comparison with the starting model. Two 4B arms separate
the factors. Both start from the stop-trained model and sample as at inference. All values of this
paragraph are read on the 2,132 test items before any temperature is fitted. There the start has a
calibration error of 9.48 after the thought (9.43 on all items, block B) and the proper-score arm
6.93. The first control keeps the price for length and replaces the proper score by the accuracy of
the answer. Its thoughts end as often (99.8\%) and are as short (433 tokens), and the raw
calibration error of the answer after the thought falls to 7.79. Its accuracy is lower (T $-$1.64
{[}$-$2.67, $-$0.66{]} against the start, $-$0.47 below the proper-score arm). The second keeps the
proper score and drops the price: thoughts grow to 2,581 tokens, 40.6\% of them reach the
4,096-token limit, and the raw calibration error rises to 11.19, above the start. Calibration
therefore follows the length of the thought: the price shortens the thoughts, and the shorter
thoughts make the answer after them less over-confident (stated confidence 80.3 at an accuracy of
73.5 with the price, 85.0 at 74.0 without it). Over an accuracy reward with the same price, the
proper score lowers the calibration error by about 0.9 points more and adds half a point of
accuracy, in one run each. Gao and Wang report a much larger effect of the reward for their 1.7B
model (fitted temperature 1.4 against 7.2, 81\% against 19\% of the items decidable at an error of
5\%). Their correctness-reward arm has no length price, which is the factor that does the work here.
A second run of each 4B arm and the accuracy-reward arm at 9B were queued when this was written
\todo[TODO(rl4\_ei2\_dw\_t06\_s1, rl4\_ei2\_acc\_t06\_s1)]{second runs of the proper-score and the
accuracy-reward arm at 4B}.

On the index the 4B of the proper-score arm with rollouts sampled as at inference scores 66.80 with
200 reasoning tokens per answer: 32.5\% of the answers get a thought, a thought has 617 tokens, and
0.4\% of the thoughts reach the 4,096-token limit. Against the stop-trained model it starts from,
that is 0.57 index points less for 60\% fewer reasoning tokens and 25 times fewer thoughts cut at
the limit. The arm with rollouts at temperature 1 lies between the two: 67.23 at 330 tokens, with
3.2\% of the thoughts at the limit and 2.1\% empty. The 9B of the arm with rollouts sampled as at
inference scores 69.52, against 70.16 for the stop-trained 9B it starts from: 0.64 points less
\todo[TODO(rl9t06s6\_di)]{reasoning tokens per answer and share of thoughts at the limit in the 9B
index run}. These are single runs. The three repeats above spread by about $\pm$0.3 on held-out
items, so one such difference is at the edge of what a run can show. The two sizes agree on a loss
of about 0.6 index points. On the rebuilt GSM8K rows, where every answer depends on the thought,
this 4B reaches 92.2 after the thought against 94.4 for its starting model. The 9B arm with rollouts
at temperature 1 reaches 96.6 against 96.3.

\emph{Without the stop step.} Reinforcement learning does not replace the stop step. Started from
the model after thinking replay and reader round, whose thoughts end in 11.4\% of the cases, the
training with rollouts at temperature 1 had not moved (see above). With the bounded score, the price
for length and rollouts sampled as at inference it does move: 58.0\% of the thoughts end and 42.0\%
reach the limit, at 2,753 tokens against 3,764. The answer after the thought is at 74.18 against
75.04 ($-$0.86, interval $-$1.82 to +0.03) and the default answer at 74.94 against 75.54 ($-$0.60,
$-$1.32 to +0.13). From the stop-trained model the same training ends 99.7\% of the thoughts. The
read-outs of this arm move apart. Before any temperature is fitted, the answer after the thought is
close to calibrated, with an error of 2.81 at a stated confidence of 74.9. The one-pass answer of
the same weights becomes under-confident: it states 62.3 on average at an accuracy of 71.2 (error
8.99). Because the gate acts on the one-pass top probability, an under-confident one-pass answer
sends more questions to a thought.

\textbf{Training the read-out in the same step, and the two-stage arms.} In a second trainer the
read-out losses are added to the policy gradient, so that the answer after a thought is trained on
the thoughts the current policy writes. From the stop-trained 4B this gives 75.27 with 78.9\% of the
thoughts ending at 1,679 tokens. The calibration error of the read-out after the thought falls from
9.4 to 7.1 and its overconfidence from 9.3 to 6.8 points, while the calibration error of the default
answer stays where it was (2.1). On the index it scores 67.43 at 574 reasoning tokens per answer. A
measurement changed how this arm is to be read. The policy gradient is averaged over the tokens of
the thoughts (about 2,000 each) and the read-out loss over the rollouts. Measured separately, the
policy-gradient part of the update has 1.5\% of the norm of the read-out part (0.12 against 7.8 at
the first iteration). The arm therefore trained the read-out on sampled thoughts and hardly
reinforced the thinker. \citet{gao2026openjev}, who sum over the tokens of a rationale, report the
opposite ratio (7 to 12) and separate the two into stages for that reason. We followed them,
starting from the 4B after thinking replay. \emph{Calibrate:} only the read-out is trained, on
thoughts sampled by the current model (5,120 items), with a penalty that holds the thinker to its
starting policy. With the penalty 72.2\% of the thoughts end afterwards, without it 35.5\%.
\emph{Reinforce:} the policy gradient is added with a weight set from the measured norms. Four arms
of the second stage (two weights, a Brier-score variant, and a reward for correctness as a control)
end 71.5 to 72.5\% of the thoughts at 2,450 to 2,490 tokens, with 70.2 to 71.2 after the thought,
72.4 to 73.6 for the default answer and 68.2 to 68.4 in one pass. The supervised chain has 85.9\%,
1,413 tokens, 74.38, 75.31 and 71.43 on the same items. Training the read-out on 5,120 items of
sampled thoughts costs three points of the one-pass answer, and nothing is gained after the thought.
We closed this line.

\textbf{Thinking again when unsure.} A different use of the outcome is a rule at inference: if the
confidence after a thought is below 0.6, think again. We measured the rule before building any
training on it. The stop-trained 4B wrote four independent thoughts for each of 2,794 routed
held-out items and, for the first thought, up to two further rounds that continue it after a cue.
The first thought is right in 73.44\% of the items at a stated confidence of 82.50. \emph{With
context:} after the further rounds the accuracy is 73.41 ($-$0.04, interval $-$0.50 to +0.43).
15.6\% of the first thoughts are below 0.6. On them the accuracy goes from 44.60 to 44.37, and the
answer changes on 49 of 435 such items, 19 times to the right answer and 20 times away from it. The
53 items that reach 0.6 in a further round are right in 47.2\% at a stated 64.2\%. The first thought
was right on 52.8\% of them. The further rounds end by themselves in 93.0\% of the cases and have
241 tokens. \emph{Without context:} drawing a new independent thought until one reaches 0.6, at most
three, gives 73.62 (+0.18, $-$0.43 to +0.75) at 1.28 thoughts per item. Averaging the same thoughts
gives 73.94. The retry is 0.32 below it ($-$0.68 to 0.00) and 1.05 points more overconfident. The
average of all four gives 73.98. The most confident of four gives 74.02, with 4.75 points more
overconfidence than the average. Inside one item the thoughts above 0.6 are right in 57.1\% against
51.0\% for those below (+6.2, +1.3 to +11.1), and all four thoughts give the same answer on 88.1\%
of the items. A first replay on stored thoughts of an intermediate 4B, on 7,860 routed items of the
training set, had given the same order: first thought 84.25, retry up to four thoughts 84.72 (+0.47,
$-$0.01 to +0.84) at 2.2 times the tokens, average of the same thoughts 84.92, average of four
85.70. The confidence does separate better from worse thoughts of one question. But a new draw is no
better than averaging at equal cost, a second round with context changes nothing, and reaching the
threshold in a second round says nothing about being right. A reward for reaching it would train
assertion, and we built no arm on this mechanism. For an item of low confidence, a second
independent thought averaged with the first is the better use of the tokens. What retrying does to
the stated confidence is taken up in Section~\ref{sec:7.3}.

\textbf{What the data support, and what is not tested.} Reinforcement learning of the thinker with a
bounded proper score, started from a model that reasons and with rollouts sampled as at inference,
does two things. It makes thoughts end: 99.7\% at 4B and 99.8\% at 9B, at about a third of the
tokens (503 against 1,413, and 544 against 1,677). And it calibrates the answer after the thought:
before any temperature is fitted the calibration error is 32\% lower at 4B and 43\% lower at 9B,
with the accuracy after the thought at 74.11 against 74.38 and at 80.87 against 81.20. The costs are
small and not zero: 0.24 and 0.46 points of the default answer on all held-out items, 0.75 on the
test part at both sizes, 1.17 points of the answer after the thought on the 4B's test part (interval
$-$2.11 to $-$0.28), 0.57 and 0.64 index points at 4B and 9B in one run each, and two points on
arithmetic at 4B. It has not raised accuracy over the supervised chain in any arm or on any
evaluation, and it has not improved the ranking of right and wrong answers. A noise reward comes
within half a point to a point of the real one in accuracy. The two-stage arms are worse. The one
gain over an arm's own start came from skipping. Most of the calibration comes with the shorter
thoughts. An accuracy reward with the same price takes the error two thirds of the way (from 9.48 to
7.79 on the test items, against 6.93 with the proper score), and without the price the proper score
makes the answer after the thought more overconfident than at the start. Without the stop step
before it, the same training ends 58\% of the thoughts. The second runs at 4B and the
accuracy-reward control at 9B were queued when this was written.

The flat accuracy is not explained by the items. An earlier version of this section offered an
explanation: on the held-out items few answers depend on the thought, so most rollouts would carry
no outcome signal and the price would be what remains. It does not hold. The pool from which the
arms draw their prompts is not ordinary classification. Its largest families are causal questions
(4,913 items), code execution (3,926), chess (2,296), murder-mystery reasoning (1,561) and generated
arithmetic and rule tasks (business days, eligibility, order budgets, invoices, deadlines, unit
thresholds and percent change, about 6,000 items in all), besides rating tasks. During training the
accuracy on these items is about 0.75 in one pass and about 0.85 after the thought. The agreement
between the thoughts of one item (the same answer from all four on 88.1\% of the items, see the
paragraph on thinking again above) was measured on the routed held-out items of the whole training
distribution, not on this pool. So the arms did train on items on which the thought changes the
answer. And no arm has raised accuracy on any evaluation, those that need computation included: on
the rebuilt GSM8K rows with a thought on every item the skill is 92.2 after training against 94.4
before at 4B, and 96.6 against 96.3 at 9B for the arm with rollouts at temperature 1
(Table~\ref{tab:5.9}). We have no tested explanation for this.

\subsection{Calibration}\label{sec:5.10}

\textbf{Purpose.} Calibration makes the probability of a one-pass answer usable as a confidence. It
changes how sure the model says it is, never which option it chooses.

\textbf{Data.} The development splits of three sets of an open decision-model project: 3,077 rows,
of which 2,069 choice, 973 yes/no and 35 score questions. No training stage uses these rows, but
training files of the same project are in the adapter mixes, so the fit set comes from a source the
models have seen.

\textbf{Method.} One temperature per question type divides the letter scores before the softmax.
Each temperature minimises the negative log-likelihood of the targets of its type, by search over
1,201 values between 0.2 and 5. A type with fewer than 200 fit rows (the score questions) takes the
temperature fitted on all rows pooled. The temperatures belong to a checkpoint: they are fitted
after every merge or average and written into the configuration file that ships with the weights,
and a data round gets a fit of its own.

\textbf{Settings.} Released temperatures, yes/no / choice / score: 3.29 / 1.756 / 1.893 (0.8B),
2.291 / 1.532 / 1.616 (2B), 1.591 / 1.387 / 1.417 (4B), 1.724 / 1.229 / 1.294 (9B), 1.421 / 1.21 /
1.229 (27B) \todo{35B-A3B; the checkpoints after the data rounds}.

\textbf{Result after the stage.} Every temperature is above 1: the models are overconfident on the
fit source, the small ones most. Over the 47 checkpoints of the release campaign the mean
calibration error falls from 0.0956 to 0.0246 on the test splits of the fit source, for all 47, and
from 0.1219 to 0.0924 on the 111 hard public JevBench items, for 37 of them (Table~\ref{tab:F.6},
and Table~\ref{tab:6.11} for the released models).

\textbf{What did not work.} \emph{One fit source.} On a 17,402-row check set close to the training
distribution the mean error rises from 0.0285 to 0.0491, and it is worse for 36 of the 47
checkpoints: at temperature 1 the models are already close to calibrated on their own distribution.
The released 0.8B is the visible case: its temperature raises the error on the hard public items
from 0.094 to 0.124. \emph{One temperature for two targets.} Sharpening by 1.25 lowers the
divergence from the soft labels of the typed-decisions set from 0.091 to 0.078 and raises the error
on the hard public items from 0.063 to 0.120. A fit on several sources that must pass a
leave-one-source-out test is planned and not done.

See Appendix~\ref{sec:F.4}. Reasoned answers and answers selected by a policy need their own
calibration: Sections~\ref{sec:5.6}
and \ref{sec:7.5}.

\subsection{Key findings}\label{sec:5.11}

\begin{mdfindings}
\textbf{A group of training data helps only the task families it contains.} At 4B the procedural
families add 3.1 to 14.3 points on three generated tasks of their kind, the rounds that train on
twin families or their training splits 2.8 to 6.0 points on the twins, and a file of rating,
preference, safety and logic families 8.6 points on the 18 reused tasks of its families and 0.3 on
the 16 others. No adapter round moves the public index by more than 0.4 points, and all weights
trained from the untrained model with the settings of the leading entries end 8.1 and 11.9 points
below the released 4B on it (Section~\ref{sec:5.3.1}).

\textbf{A thought is worth two to three index points, and far more where the answer has to be
computed.} With the gate at 0.9, reasoning adds 1.9 to 2.9 points to the one-pass index. On GSM8K
rows without a shortcut in the options it takes our models from a skill of 25--52 to 92--99, on
three procedural benchmark tasks from an accuracy of 0.49--0.76 to 0.86--1.00, and on three harder
generated tasks from 0.60--0.78 to 0.84--0.98. On NLI-like and select-all families it lowers
accuracy (Section~\ref{sec:5.1.1}).

\textbf{On such tasks the default answer gives part of the gain away.} On the harder generated tasks
the 27B is right on 98.4\% of the items after the thought and on 94.1\% with the default answer: the
gate does not send a confidently wrong one-pass answer to reasoning, and the mixture keeps half of a
one-pass read-out that is near chance.

\textbf{The reasoning stages do not return all of the starting model's reasoning.} On the same
arithmetic items the untrained 4B and 9B reach 97.1 and 98.6 after a thought and ours 94.4 and 96.3
after the stop step, and the untrained 4B needs fewer than half the tokens (Table~\ref{tab:5.9}).

\textbf{A decision loss leaves the end of a thought unsupervised, and the end is what breaks.} The
closing probability fell in the 9B data rounds and in the reader round after replay at all three
sizes, stayed where it was in the 4B data rounds, and returned in the one stage that trains the
closing tag (Table~\ref{tab:5.2}).

\textbf{What the reader round does depends on what came before it.} Replay alone ends 74.6\% of the
4B's thoughts and the reader round after it leaves 11.4\%. Without replay before it the same round
leaves 96.5\%, of thoughts a few lines long (Table~\ref{tab:5.3}).

\textbf{A thought is usually finished long before it stops, but not on the hardest questions.} In
61\% of the selected thoughts the answer is final after the first eighth, and cutting every thought
at 1,024 tokens costs nothing on held-out items (Table~\ref{tab:5.5}). On the index the same cut
costs 0.8 points, all in the knowledge area. Across designs the index follows the reasoning tokens
spent: 66.80 at 200 per answer, 67.23 at 330, 67.37 at 497 and 67.72 at 1,144.

\textbf{The end can be taught from the model's own thoughts.} Eighty-two training steps on thoughts
cut where the readout stops changing take the share of thoughts that end from 11.4\% to 85.9\% at
unchanged accuracy on held-out items. On the index the 4B keeps 67.37 of 67.72 with 43\% of the
reasoning tokens, and the 9B rises from 69.77 to 70.16 with 53\% of them (Section~\ref{sec:5.7}). A
loop check every 256 tokens at inference takes most of the thoughts that are still open afterwards
(3.5\% stay open instead of 14.1\%) at unchanged accuracy on held-out items.

\textbf{The largest model needs no stop step.} At 27B the reader round lowers the closing
probability too (0.97 to 0.54), but replay and the reader round give 72.34 with 6.0\% of the
thoughts at the limit. Thoughts that do not end are a problem of the 4B and the 9B
(Sections~\ref{sec:5.4} and \ref{sec:5.6}).

\textbf{Reinforcement learning with a proper score makes thoughts end and calibrates the answer
after the thought, and it has not made the answers better.} From the stop-trained model, with
rollouts sampled as at inference, 99.7\% (4B) and 99.8\% (9B) of the thoughts end at about a third
of the tokens, and the calibration error of the answer after the thought is 32\% and 43\% lower
before any temperature is fitted. The accuracy after the thought stays within a third of a point on
held-out items. The default answer loses a quarter to three quarters of a point there, and the index
0.57 (4B) and 0.64 points (9B) in one run each. The ranking of right and wrong answers does not
improve. The calibration follows mostly the length of the thought: an accuracy reward with the same
price reaches 7.8 (proper score 6.9, start 9.5), and the proper score without the price makes
thoughts longer and the answer after them more over-confident (11.2). Without the stop step before
it, the same training ends 58\% of the thoughts, and the one-pass answer of those weights becomes
under-confident. The price for length does the shortening. The outcome term holds half a point to a
point over a price-only and a noise control. Started from a model that hardly reasons, the policy
learns to skip: 67.18 with 57 reasoning tokens per answer, two thirds of the thoughts closed without
a word. Two-stage training and thinking again on low confidence gained nothing. The item pool does
not explain the flat accuracy: it is mostly made of questions that have to be worked out
(Section~\ref{sec:5.9}, Table~\ref{tab:5.11}).

\textbf{A longer limit adds nothing.} At 8,192 tokens with a loop check, and at 16,384 with or
without one, accuracy stays inside its interval on held-out items, and on the index a limit of 8,192
tokens scores 67.52 against 67.72. Without a check the longer limit multiplies the cost, and a
repetition penalty loses half a point (Tables~\ref{tab:5.5} and
\ref{tab:5.10}).

\textbf{The gate cannot be lowered for free, and a confidence-dependent weight does not beat the
flat mixture.} On held-out items the gain of reasoning is complete with the gate at 0.7, at about
half as many thoughts as at the default of 0.9. On the index the same gate costs half a point (67.20
against 67.72). No rule that sets the weight of the thought from the one-pass confidence beats the
0.5 / 0.5 mixture on held-out items (90.12 at 4B, 92.96 at 9B) (Section~\ref{sec:5.1.2}).

\textbf{The base model's thoughts need a trained reader.} The untouched base model ends 91.1\% of
its thoughts on the same items, and a model that has had a reader round is level with our
single-model system when it reads them ($-$0.07 and $-$0.56 points for two readers). The data-round
model, which was never trained to read thoughts, is 8.5 points below it (Table~\ref{tab:5.5}).
\end{mdfindings}


==> sections/07_serving_cost.tex <==
\clearpage
\section{Serving and cost}\label{sec:7}

A decision model is used inside other systems, so what it costs is part of what it is.
Table~\ref{tab:12} gives the latency of every size. A request with three questions takes 12 ms on
the 0.8B and 102 ms on the 27B, and the 35B-A3B, with about 3B of its 35B parameters active per
token, answers in half the time of the 27B on one 80 GB GPU.

\begin{table}[!htbp]
\renewcommand{\thetable}{12}
\centering
\caption{Latency and throughput of the released models on one H200 in bf16 with the released runtime. Latency: end to end over HTTP, one request at a time, 20 warm-up and 200 timed requests. The three-question request holds one choice, one yes/no and one score question about a support ticket (891 prompt tokens), answered in one forward pass. Throughput and memory: one call with 256 yes/no questions about a 316-token document.}\label{tab:12}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrr}
\toprule
\textbf{model} & {\begin{tabular}[b]{@{}r@{}}\textbf{three questions:}\\\textbf{mean / P95}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{one}\\\textbf{yes/no}\\\textbf{question}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{decisions}\\\textbf{per}\\\textbf{second}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{peak GPU}\\\textbf{memory in}\\\textbf{that test}\end{tabular}} \\
\midrule
StartLux-Decision-0.8B & 12.2 / 14.2 ms & 8.3 ms & 370 & 6.99 GiB \\
StartLux-Decision-2B & 15.5 / 17.2 ms & 9.6 ms & 241 & 9.72 GiB \\
StartLux-Decision-4B & 26.0 / 27.3 ms & 14.7 ms & 113 & 17.75 GiB \\
StartLux-Decision-9B & 35.7 / 37.4 ms & 17.6 ms & 72 & 27.53 GiB \\
StartLux-Decision-27B & 102.3 / 104.3 ms & 50.7 ms & 23 & 64.96 GiB \\
StartLux-Decision-35B-A3B & 52.5 / 54.5 ms & 36.4 ms & \todo{} & about 71 GiB \textsuperscript{a} \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{a} peak stated with the release of this model, not measured in this test.\par}
\end{table}

Three things make the one-pass path fast. The linear-attention layers need two kernel packages, and
without them the model library falls back, without an error, to an implementation that is more than
ten times slower, so the server refuses to start where they are not active. Nothing is generated,
and only the output rows of the option letters are multiplied. And short requests are replayed from
recorded CUDA graphs, which removes the kernel-launch overhead that dominates short inputs (26.0
against 90.3 ms at 4B). For long inputs the runtime reads the shared beginning of a request once and
runs all questions on top of it: 128,000 tokens with three questions take 19.3 s instead of 146.8 s
on the 27B, with probabilities unchanged within $\pm$0.001.

\textbf{Capacity of one node.} On one node with eight H200 GPUs and the request mix of the index (a
mean of 880 tokens), the batched offline runner answers 576,000 requests per hour with the 4B,
402,000 with the 9B and 136,000 with the 27B. 8-bit weight formats were slower than bf16 on this
hardware, by 8 to 20\% at 1,024 to 16,384 tokens for the 9B, because the GPU is limited by
computation and not by memory.

\textbf{Cost of reasoning.} Reasoning multiplies the cost of the questions it is used for and leaves
the others at the cost of one pass. In every index run with reasoning 27 to 33\% of the answers were
reasoned about, while the tokens per thought differed by a factor of thirteen between models. The
cost is therefore set by how much a model writes, not by how often it reasons. With reasoning at the
default threshold, the 9B after the stop step answers 41,600 index requests per hour on the node,
about a tenth of its one-pass rate, and one index run of the 27B with reasoning took 8.8 node-hours.
The threshold is the user's lever on this cost, and it should be checked on the user's own data.

\textbf{Settings that change results.} The read-out is deterministic, so two paths that serve the
same weights must agree, and they did not always. Prefix caching in a widely used inference server
moved 2.6\% of the one-pass read-outs by more than 0.05, and its default chunked prefill cost
reasoning runs 1.4 index points at 4B (65.01 instead of 66.38), which we first misread as a cost of
reasoning. Both are off in every run of this report (Appendix~\ref{sec:E}).


==> sections/07_using_probabilities.tex <==
\clearpage
\section{Using the probabilities: selection, certificates and policy-aware calibration}\label{sec:7}

This chapter is for users who act on the probabilities the models return. A probability decides
which answers are acted on without review, and it decides where more computation is spent: reason
when the one-pass answer is unsure, escalate to a larger model, or draw several candidate responses
and keep the one a verifier scores highest. In each of these designs a probability chooses the
answer that the system returns, and the system then reports a probability for that answer. The
chapter is about the second number: what it means, how large its error is, how to test it, and how
to repair it without retraining the model that answers. Appendices~\ref{sec:A} to \ref{sec:E} hold
the proofs and the full evidence.

All results are own runs on the item sets named with each exhibit, not index runs. Models of other
teams were run by us from their public weights and code. \emph{Overconfidence} is mean reported
confidence minus accuracy, in points. The readouts predate the serving correction of
Section~\ref{sec:8.4}. A re-read of the stored 4B and 9B traces on the corrected path leaves the
accuracy within 0.1 points and the route effect where it was (Appendix~\ref{sec:C.6}).

\subsection{The rule in plain words}\label{sec:7.1}

This section states the rule, shows it on one measurement and names the policies it applies to.

\textbf{The rule.} A reported probability is reliable for the kind of answers it was calibrated on.
A policy that uses a probability to choose the answer (the winner among candidates, the answer after
a route) returns another kind of answers. Calibrate the probability, and certify any threshold on
it, on answers that the same policy returned.

\textbf{A worked example.} StartLux-Decision-9B is used as a verifier: it is asked whether a
candidate response is correct. When it says ``80 to 90\% sure'' about a single response, it is right
92\% of the time. When the response is the one it scored highest among 32 candidates, the same
statement is right 78\% of the time. Nothing about the verifier changed. The answer was chosen by
the number that is then reported for it. The usual calibration does not repair this, because it
looks at single responses (Figure~\ref{fig:7.1}): answers that the calibrated verifier reports at
80--90\% are right 86\% of the time for one candidate, 76\% for the best of four and 63\% for the
best of 32. Under a calibration map that is told what the selection looked at (the scores of the
other candidates and how many there were), they are right 88\%, 87\% and 79\% of the time
(Section~\ref{sec:7.5}).

\begin{figure}[!htbp]
\renewcommand{\thefigure}{7.1}
\centering
\adjincludegraphics[max width=\linewidth,max height=0.5\textheight]{figures/fig0_meaning.pdf}
\caption{What a reported confidence means after selection: share of correct answers among the answers that a verifier selects from N candidates and reports inside a confidence bin (grey band). Unseen datasets (5,761 problems, 2B generator), StartLux-Decision verifiers of three sizes. Open, orange: the usual calibration, an isotonic map fitted on single judged responses. Filled, blue: the policy-aware map, fitted at N = 1, 4 and 16. Pooled over 20 splits by source problem. Bars: 10th--90th percentile of the splits.}\label{fig:7.1}
\end{figure}

\textbf{The four policies} (Figure~\ref{fig:7.2}). A \emph{think-gate} reasons if and only if the
one-pass (``plain'') confidence c0 is below a threshold $\tau$ and then reports the answer after
reasoning (the ``thought'' answer) with its confidence c1, otherwise the plain answer with c0. The
default control is a think-gate. A \emph{cascade} escalates if and only if the small model's
confidence is below $\tau$ and reports the large model's answer with the large model's confidence.
\emph{Best-of-N} draws N responses, returns the one to which a verifier gives the highest
probability of being correct, and reports that probability. \emph{Select-then-think} is best-of-N
after which the verifier reasons about its k favourites. On top of any of these a user may accept an
answer without review when its confidence is at least a threshold.

\todo{the style guide lists the four policies of this figure as ``threshold \textperiodcentered{}
best of N \textperiodcentered{} routing and cascades \textperiodcentered{} think-gate''
(tech\_report\_style.md:1098); the manuscript and the figure file have think-gate, cascade,
best-of-N and select-then-think (part2.md:10-23). The text follows the manuscript.} The default
control reports a mixture. The think-gate measured in this chapter reports the thought distribution
alone. The control of Section~\ref{sec:3.4} reports the equal mixture of the plain and the thought
distribution, with weights 0.5 and 0.5 (the \emph{default answer} of Chapter~\ref{sec:5}). On 3,021
held-out items that a 4B routes to reasoning, measured for four training designs, the plain read-out
is under-confident on the routed items (confidence minus accuracy $-$3.5 to $-$7.1 points), the
read-out after the thought is over-confident (+5.1 to +9.3, calibration error 5.6 to 9.4), and their
mixture is within $-$0.7 to $-$2.7 with a calibration error of 2.1 to 3.1. The two biases have
opposite signs on the routed answers and largely cancel. This is a side effect of a mixture that was
chosen for accuracy, measured at one size on one item set, and it is not guaranteed: for the thinker
trained with reinforcement learning, which closes many thoughts at once, the mixture is 6.5 points
under-confident. The certificate per route remains the tool when a threshold is applied.

\textbf{What the mixture costs a caller who automates above a threshold.} A small calibration error
does not make the mixture's confidence useful for ranking. On the routed held-out items of the
stop-trained 4B (889 items to fit temperatures and weights, 2,132 to measure), the mixture is the
most accurate rule (75.4\%, against 74.7\% for the read-out after the thought) and the worst for
selective use: the area under its risk-coverage curve is .130 against .117, and the share of answers
that can be accepted at an error of 5\% is 5\% against 21\% (at 10\%: 37\% against 43\%). Half of
the mixture is a read-out that is unsure by construction on these items, which caps the confidence
of every answer. A linear pool of forecasts is under-confident in this way in general
\citep{ranjan2010combining}. A log-linear pool with two exponents fitted on the 889 items (0.3 for
the one-pass and 0.5 for the after-thought read-out) keeps the accuracy within noise (75.1\%,
difference $-$0.23, interval $-$0.56 to +0.14) and restores the ranking (area .115, difference to
the mixture $-$.015, interval $-$.022 to $-$.007, acceptable at 5\% error: 18\%, at 10\%: 49\%,
calibration error 1.7). A second 4B, before its stop step, gives the same picture on its 3,021
routed items: the fitted pool keeps the accuracy of the mixture ($-$0.14, interval $-$0.33 to 0.00),
lowers the area under the risk-coverage curve by .013 (.008 to .018) and raises the share acceptable
at 5\% error by 11.6 points (3.1 to 16.0). Across the 4B designs we measured, the share of answers
that can be accepted at 5\% error is 20 to 23\% with the read-out after the thought, 4 to 5\% with
the default mixture, and 17.5\% with the fitted pool of the stop-trained 4B. Applied to the stored
answers of the index run of the same model without a new model call, the pool gives 67.49 against
67.37 for the mixture: the index does not separate the rules.

For accuracy the equal mixture is not beaten. We also asked whether a weight that depends on the
one-pass confidence gives better answers. On the 8,598 held-out items of the training distribution,
with one half to choose a rule and the other half to test it, the 4B after thinking replay and
reader round has 90.12 on the test half with the flat 0.5 / 0.5 mixture, 89.91 with the thought
alone, 90.05 to 90.07 with fitted log pools, and at best 90.12 when the thought gets a weight of
0.75 or 1.0 wherever the one-pass top probability is below a cut-off between 0.4 and 0.7 (one pass:
88.60). The stop-trained 9B has 92.96 with the flat mixture, 92.52 with the thought alone, 92.71 to
92.82 with log pools and 92.64 to 92.77 with linear weights (one pass: 91.99). No rule chosen on the
first half beats the flat mixture on the second. The choice between the mixture and the fitted pool
is therefore not a choice about accuracy: at the same accuracy, the pool is the better confidence
for a caller who thresholds. One kind of task lies outside this test. Where an answer has to be
computed, the one-pass read-out is near chance and the default answer falls below the thought alone:
94.6 against 96.3 for the 9B on the rebuilt GSM8K rows, and 0.941 against 0.984 for the 27B on three
generated tasks, where the gate also keeps one-pass answers that are confident and wrong
(Section~\ref{sec:5.1.1}). Such items are rare among the held-out items, and a weight for them would
have to be fitted on items of their kind. The released servers return the mixture.
\todo[TODO(voc\_th9ei2\_hoall, voc\_rd27tf\_hoall)]{risk-coverage area and acceptable share of the
fitted pool at 9B and 27B, before the default is changed}

\begin{figure}[!htbp]
\renewcommand{\thefigure}{7.2}
\centering
\adjincludegraphics[max width=\linewidth,max height=0.5\textheight]{figures/fig2_policies.pdf}
\caption{The four policies. Orange marks the score that routes or selects, shaded boxes the answer that is returned and the confidence reported with it.}\label{fig:7.2}
\end{figure}

\textbf{Two calibrations.} The \emph{usual} calibration is fitted on what a calibration set gives by
default: all thought answers, all answers of the large model, single judged responses. Calibration
\emph{per policy} is fitted on what the deployed policy returns on the calibration problems: only
the routed second answers, or the winners. For a threshold on the one-pass answer alone the two
coincide. Appendix~\ref{sec:A.8} describes a reference implementation of the certificate and of the
maps.

\todo{confirm what is released --- v4 describes the script (part2.md:427-428, part3b.md:368) and
lists only checkpoints and inference code as public (part3b.md:285); the style guide expects
``calibration maps and certificate script'' in the links block (tech\_report\_style.md:967).}

\subsection{Why it happens}\label{sec:7.2}

The reason is given here in words. Propositions 1 to 4 and their proofs are in Appendix~\ref{sec:A}.

\textbf{Proposition (in words).} If a confidence is calibrated given everything the policy looked at
when it chose the answer, it is calibrated on the answers the policy returns. If the policy looked
at something the confidence leaves out, and that something still says whether the answer is right,
the returned answers are miscalibrated in a direction that can be predicted.

\emph{Selection.} The winner has score s. Its N $-$ 1 rivals all scored lower. The more rivals fell
below s, the more likely the problem is one on which scores run low, a hard one, and on a hard
problem a response with score s is right less often. The losing candidates are data about the
problem, and a confidence calibrated on single responses has not seen them. Such a verifier is
overconfident on its selected responses, more so with more candidates.

\emph{Routing.} A gate routes on c0 and the system reports c1. What matters is what c0 still knows
about the reported answer once c1 is given. We measure it as the \emph{residual AUROC}: the AUROC of
c0 for the correctness of the reported answer within quintiles of c1. At 0.5 the reported confidence
already contains what the routing confidence knows. Above 0.5 the routed answers are overconfident
relative to the kept ones, and below 0.5 the reverse. Across 36 pairs of a model and an item set it
predicts the size and the sign of the route effect (Figure~\ref{fig:7.3}: Spearman $-$0.88
{[}$-$0.92, $-$0.77{]}, same sign in 31 of 36).

\subsection{Evidence in four policies}\label{sec:7.3}

The size of the effect is given for each policy in turn. Table~\ref{tab:7.1} is a selection from the
tables of Appendices~\ref{sec:B} and \ref{sec:C}, which list every run with its protocol.

\begin{table}[!htbp]
\renewcommand{\thetable}{7.1}
\centering
\caption{The effect in numbers. (a) Best-of-N, 2B generator, released checkpoints as verifiers: accuracy of the returned answer (\%), and overconfidence of the selected response after calibration on single responses (points) from N = 4 to the largest N, one entry per problem set (Appendix~\ref{sec:B.1}). (b) Accuracy of the reported answer at matched reported confidence, routed minus kept {[}95\% interval{]}. Negative = routed answers overconfident. Think rate = share of the items routed. The 5,710 decisions, the \emph{decision suite}, are diagnostic items of 39 task families (benchmark type, 150 per family, not held-out). ``Ours'' = StartLux-Decision. Best accuracy in bold. Own runs.}\label{tab:7.1}
\par\medskip\noindent{\small\textbf{(a)}}\par\smallskip
{\footnotesize\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrl}
\toprule
\textbf{verifier} & {\begin{tabular}[b]{@{}r@{}}\textbf{held-out,}\\\textbf{best-of-64}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{unseen}\\\textbf{datasets,}\\\textbf{best-of-32}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{reasoning,}\\\textbf{best-of-16}\end{tabular}} & \textbf{overconfidence, N = 4 $\rightarrow$ max} \\
\midrule
ours 4B & 92.52 & 82.07 & 77.32 & +1.6 $\rightarrow$ +3.8, +4.7 $\rightarrow$ +9.4, +3.5 $\rightarrow$ +6.4 \\
ours 9B & 94.19 & 83.34 & 78.02 & +1.5 $\rightarrow$ +2.9, +4.2 $\rightarrow$ +8.4, +3.4 $\rightarrow$ +6.1 \\
ours 27B & \textbf{95.48} & \textbf{86.04} & \textbf{82.97} & +0.5 $\rightarrow$ +1.4, +1.8 $\rightarrow$ +3.8, +2.4 $\rightarrow$ +3.2 \\
Clef 27B (another team's decision model) & 93.01 & 83.13 & 77.01 & +1.0 $\rightarrow$ +3.5, +3.0 $\rightarrow$ +7.0, +2.4 $\rightarrow$ +5.3 \\
Phi-4-mini-instruct (chat model as judge) & 83.17 & 74.16 & 66.45 & +4.3 $\rightarrow$ +11.4, +6.8 $\rightarrow$ +14.9, +5.7 $\rightarrow$ +10.8 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\medskip\noindent{\small\textbf{(b)}}\par\smallskip
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.1672}}>{\raggedright\arraybackslash}p{\mdw{0.2674}}>{\raggedright\arraybackslash}p{\mdw{0.2280}}>{\raggedleft\arraybackslash}p{\mdw{0.3237}}}
\toprule
\textbf{policy} & \textbf{models} & \textbf{items} & \textbf{routed minus kept {[}95\%{]}} \\
\midrule
think-gate, 30\% think rate & ours 4B / 9B & 5,710 decisions & $-$.194 {[}$-$.230, $-$.158{]} / $-$.214 {[}$-$.254, $-$.171{]} \\
think-gate, 30\% & Phi-4 (14B) / Gemma-3-4b, zero-shot chain of thought & same & $-$.176 {[}$-$.203, $-$.149{]} / $-$.028 {[}$-$.057, .000{]} \\
think-gate, 30\% & Jeeves-9B (another team's decision model) & same & $-$.037 {[}$-$.071, $-$.006{]} \\
think-gate, 10\% / 20\% / 40\% & ours 4B & CJ-Bench, 304,822 hard decisions (Chinese) & $-$.114 {[}$-$.122, $-$.108{]} / $-$.163 {[}$-$.168, $-$.156{]} / $-$.241 {[}$-$.245, $-$.236{]} \\
think-gate, 30\% / 50\% & ours 4B, Jeeves-9B & 4,648 reasoning decisions & +.057 / +.021, +.032 / +.025 (reversed) \\
cascade, $\tau$ = .7 & Clef-flash $\rightarrow$ Clef 27B, ours 4B $\rightarrow$ ours 27B & 5,710 decisions & $-$.123 {[}$-$.164, $-$.083{]}, $-$.139 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\todo{name the checkpoints behind ``ours 4B / 9B'' in (b) --- one model that decides and reads its
own reasoning, ``single model'' in v4 (part2.md:153) --- and add the in-domain marker for the 39
task families (Appendix C.1).}

\textbf{The selected answer is overconfident, and more candidates make it worse.} After calibration
on single responses the selected response is overconfident in 111 of 113 pairs of a generator and a
verifier at N = 16, the gap grows with N in all 126, and it is larger the weaker the verifier
(Table~\ref{tab:7.1}a, Figure~\ref{fig:B.3}). Large N does not wash it out: at N = 256 on the unseen
datasets it reaches +15.1 / +12.8 / +6.5 points for the 4B / 9B / 27B verifier (0.8B generator).

\textbf{After a think-gate or a cascade, routed answers are less accurate than kept ones at the same
reported confidence.} This holds for eleven of twelve models on the decision suite and for every
model on the third-party benchmark, CJ-Bench (Table~\ref{tab:7.1}b). Size and sign follow the
residual AUROC: .69 and .64 for our 9B and 4B, .49--.50 for three models whose differences lie
between $-$.038 and +.021. Ten cascades fall on the same line (residual AUROC .58--.71, differences
$-$.10 to $-$.17).

\begin{figure}[!htbp]
\renewcommand{\thefigure}{7.3}
\centering
\adjincludegraphics[max width=\linewidth,max height=0.5\textheight]{figures/fig6_gate_info.pdf}
\caption{What the route effect is made of. Horizontal: residual AUROC of the routing confidence for the correctness of the thought answer, given the thought confidence (0.5 = nothing left). Vertical: accuracy of thought answers at matched thought confidence, routed minus kept. One point per model and item set. Triangles are cascades of a small and a large model.}\label{fig:7.3}
\end{figure}

Decision training makes the route effect larger. The base models ours are tuned from show little of
it on the decision suite ($-$.069 and +.021). After decision training it is $-$.214 and $-$.194.
Training sharpens the plain confidence (its AUROC for the plain answer rises from .78 to .87 at 9B),
and the thought confidence does not absorb what the plain one now knows.

\textbf{The sign is not universal.} On reasoning items a low plain confidence marks the items that
thinking solves: the residual AUROC is below .5 for five models, whose routed answers are the more
accurate ones, and above .5 for four others, which stay negative. One decision model of another team
has almost no effect (Jeeves: residual AUROC .56, difference $-$.037): the route-dependence comes
from how the confidence after reasoning was trained and is not a law of gates
(Appendix~\ref{sec:C.4}).

Select-then-think gains accuracy and adds the route whose confidence can be trusted least. With the
4B as verifier of 64 samples, reasoning about its three favourites raises accuracy from 92.3 to 93.5
(2B generator). After calibration on single responses the thought route is overconfident by +4.2 to
+10.4 points at N = 64, the fast route by less than two points at any N (Appendix~\ref{sec:C.5}).

\textbf{Thinking again until the answer is confident is selection too, and it inflates the stated
confidence.} A rule that draws a new thought when the confidence after the first is below 0.6, or
that keeps the most confident of several thoughts, chooses the returned answer by the number that is
then reported for it. We measured both with the stop-trained 4B on 2,794 routed held-out items of
the training distribution (Section~\ref{sec:5.9}). Retrying up to three times is 1.05 points more
overconfident than the average of the same thoughts, and 0.32 points less accurate (interval $-$0.68
to 0.00). The most confident of four thoughts is 4.75 points more overconfident than the average of
the four, at an accuracy of 74.02 against 73.98. An earlier replay on items of the training set gave
4.2 points. When the first thought is continued for up to two further rounds, the 53 items whose
confidence then reaches 0.6 are right in 47.2\% of the cases at a stated 64.2\%. All of this comes
on top of a read-out after one thought that already states 82.50 at an accuracy of 73.44. It is the
selection effect described above, with the model's own thoughts as candidates. The remedy is the
same as for the other policies (calibrate and certify on the answers the retry policy returns, and
give the map the number of thoughts and their mean confidence), but we have not fitted such a map
for these policies. Averaging the thoughts is at least as accurate at the same cost and does not
select by confidence.

\subsection{Certificates per policy}\label{sec:7.4}

A certificate is a threshold on the reported confidence with a tested bound on the error of the
answers it accepts. We give the protocol and show where the calibration data must come from.

\textbf{Protocol.} A threshold is certified for error $\leq$ $\alpha$ on a calibration half of the
problems (fixed-sequence Clopper--Pearson test at 95\% on a fixed grid of thresholds, at least 100
accepted answers) and applied to the answers the system returns on the other half, over 20 splits by
source problem.

\begin{table}[!htbp]
\renewcommand{\thetable}{7.2}
\centering
\caption{Error of the accepted answers when the threshold is certified on the usual calibration data (first line of a setting) and on the answers of the same policy or route (second line), with the number of splits in which the error is above $\alpha$. Selection from Table~\ref{tab:D.1}. Own runs.}\label{tab:7.2}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.3828}}>{\raggedright\arraybackslash}p{\mdw{0.1758}}>{\raggedright\arraybackslash}p{\mdw{0.2641}}>{\raggedleft\arraybackslash}p{\mdw{0.1635}}}
\toprule
\textbf{setting} & \textbf{threshold certified on} & \textbf{error of accepted answers} & \textbf{splits above the level} \\
\midrule
best-of-N, unseen datasets, $\alpha$ = .05, N = 32, ours 4B / 9B / 27B & single responses & 10.05\% / 9.27\% / 7.57\% & 19 / 20 / 20 of 20 \\
 & the same policy & 3.5--4.3\% & 0--4 of 20 \\
best-of-16, all 67 pairs with coverage, $\alpha$ = .05 & single responses & above the level in 44 of 67 pairs & $\geq$ 10 of 20 in 32 pairs \\
 & the same policy & above the level in 0 of 67 pairs & $\geq$ 10 of 20 in 0 pairs \\
think-gate, CJ-Bench, $\alpha$ = .05, ours 4B, 10\% / 20\% think rate & all answers & thought answers 27.9\% / 27.3\% & 20 / 20 \\
 & per route & no thought answer accepted, system 4.6\% & 0 \\
select-then-think, reasoning sets, $\alpha$ = .10, 9B, N = 2 / 4 / 8 & all returned answers & thought answers 22.2 / 18.6 / 15.8\% & 20 / 20 / 14 \\
 & per route & 6.9--7.8\% & 0 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\textbf{A threshold certified on the usual data is exceeded by the answers the policy acts on, but
one certified on the policy's own answers is not.} For best-of-16 at $\alpha$ = .05 the first is
above the level in 44 of 67 pairs, the second in none (Table~\ref{tab:7.2}, Figures~\ref{fig:B.1},
\ref{fig:B.3}).

\textbf{A certificate for all answers is silent about the route.} The error of all accepted answers
is the weighted mean of the errors of the routes, and the kept answers are many and safe
(Proposition 3). With one threshold for all answers, the thought answers (the ones the system paid
extra for) are accepted at several times the level. Certified per route, the think-gate accepts
none. A per-policy certificate can refuse, and a route with no certifiable threshold is information
about the system.

\subsection{Policy-aware calibration}\label{sec:7.5}

Per-policy thresholds have to be certified again for every N and every think rate. The map described
here is fitted once, because it is told what the policy looked at (Proposition 4).

\textbf{Recipe.} Three steps, and no knowledge of a threshold is needed.

\begin{enumerate}
\item Run the policy on calibration problems and record, with every returned answer, its confidence and
what the policy looked at: for selection, the mean score of the candidates and N. For a gate or a
cascade, the confidence that decided the route. For select-then-think, the fast score of the
returned candidate, the mean fast score and N.
\item Fit the map: for a single routing score, an isotonic map of the reported confidence within eight
quantile strata of that score. For selection, a logistic model in the logits of the quantities and
log N, followed by an isotonic map.
\item Report the mapped confidence and certify thresholds per route.
\end{enumerate}

\begin{table}[!htbp]
\renewcommand{\thetable}{7.3}
\centering
\caption{Overconfidence of the returned answers (points) under the usual calibration and under the policy-aware map, which is given what step 1 records. Own runs, except the last row, which uses the public records of another group (Appendix~\ref{sec:D.6}).}\label{tab:7.3}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.2033}}>{\raggedright\arraybackslash}p{\mdw{0.4194}}>{\raggedright\arraybackslash}p{\mdw{0.2286}}>{\raggedleft\arraybackslash}p{\mdw{0.1350}}}
\toprule
\textbf{pipeline} & \textbf{settings} & \textbf{usual calibration} & \textbf{policy-aware map} \\
\midrule
best-of-N & unseen datasets, five verifiers, N = 2 \ldots{} 32, fitted at N = 1, 4, 16 & +0.8 \ldots{} +14.6, growing with N & $-$1.2 \ldots{} +0.3 \\
think-gate & decision suite, nine models, think rates 10--50\% & up to +16 on the routed answers & $-$1.5 \ldots{} +2.1 \\
cascade & decision suite, seven pairs of models of two teams, 30\% escalated & +2.3 \ldots{} +8.4 on the escalated answers & $-$0.6 \ldots{} +0.5 \\
select-then-think & ten settings: two verifiers on held-out, unseen and reasoning problems, fitted at the two or three smallest N & +2.1 \ldots{} +7.3 at the largest N, growing with N & $-$1.4 \ldots{} +0.7 at every N \\
actor $\rightarrow$ reasoner, records of another group & 21 settings: eleven actors, two option orders, 30\% deferred, 180 deferred questions each & $-$10.7 \ldots{} +18.1 on the deferred answers & $-$7.4 \ldots{} +4.4 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\begin{figure}[!htbp]
\renewcommand{\thefigure}{7.4}
\centering
\adjincludegraphics[max width=\linewidth,max height=0.5\textheight]{figures/fig9_recipe.pdf}
\caption{One calibration recipe in four pipelines: overconfidence of the returned answers under the usual calibration (open, orange) and under the policy-aware map (filled, blue). Grey band: $\pm$2 points. Best-of-N: unseen datasets, two generators, three verifiers, up to N = 256. Think-gate: thought answers on routed items, nine models on three item sets at three think rates each. Cascade: seven pairs. Select, then think: ten settings.}\label{fig:7.4}
\end{figure}

\textbf{One recipe repairs the reported confidence in all four pipelines.} Over the 184 settings of
Figure~\ref{fig:7.4} and Table~\ref{tab:7.3} the usual calibration is off by $-$11.7 to +20.5 points
and the policy-aware map by $-$2.7 to +2.1. On the public records of another group's system, an
actor that defers to a reasoner, the same construction brings the error of the reasoner's stated
accuracy on the deferred questions from 8.3 to 2.1 points (Appendix~\ref{sec:D.6}).

For selection the map is calibrated at values of N it never saw. Fitted at N = 1, 4 and 16, it stays
within $-$0.7 \ldots{} +0.3 points up to N = 32 for our three verifiers and Clef 27B, where the
single-response map reaches +9.4 for the 4B verifier. At N = 256 it is underconfident by 0.1 to 2.6
points. The rule ``accept iff confidence $\geq$ .95'' at N = 32 accepts answers at 5.4\% to 8.0\%
error under the single-response map (above the level in 17 to 20 of 20 splits) and at 1.0--2.9\%
under the set-aware map (in none).

\textbf{For gates and cascades the map repairs the calibration, not the certificate.} One threshold
for all answers still lets thought answers through above the level: for our 4B at $\alpha$ = .10 and
a 30\% think rate at 12.6\% error with a map of c1 alone and at 10.7\% with the route-aware map
(above the level in 16 and in 9 of 20 splits). The mapped confidence is the number to report. The
guarantee is certified per route (Appendix~\ref{sec:D.4}).

\textbf{Limits.} The map needs the same calibration problems as a per-policy certificate. It saves
the repetition per N. Fitted on the held-out set and applied to the unseen datasets it is
overconfident by up to +6.1 points: it has to be fitted on problems from the deployment
distribution. A threshold certified on it does not extrapolate far beyond the fitted N: for N = 32
\ldots{} 256 with the weakest generator the accepted answers run at 4.4--5.2\% for $\alpha$ = .05,
above the level in 5--14 of 20 splits (Appendix~\ref{sec:D.3}).

\subsection{Routing by value of computation}\label{sec:7.6}

The route effect exists because the gate routes on a score that still knows something about the
answer the system reports. The gate described here asks another question: is reasoning worth its
cost on this item? It is a typed yes/no question of the same model, read in the same pass as the
one-pass answer, with a cost level as input. Its labels are exact, because for every training item
both readouts exist. It is a research result on diagnostic items, not the default control.
\todo{release status of the gate (Appendix E).}

\textbf{The answers it routes can be used.} At an equal think rate, the thought answers on the items
the value gate routes are 75\% accurate where those routed by uncertainty are 30\% accurate, and
they become certifiable: 192 thought answers per split are accepted at 5.5\% error where a rule on
uncertainty certifies none (Table~\ref{tab:E.1}, Appendix~\ref{sec:E.4}). In a two-model control its
score has a residual AUROC of .48--.51 at 4B, against .69 for the plain confidence: it says where
thinking pays, not where the thought answer will be wrong (Table~\ref{tab:E.2}).

\textbf{It does not raise the accuracy of the whole system at a middling think rate.} At 45\% it is
within half a point of routing by confidence at all three sizes (+0.35, $-$0.20, $-$0.45). It asks
for shorter reasoning (349 against 436 tokens per item at 4B) and is ahead at a low think rate at 4B
(+1.26 points at 16\%).

\textbf{Ask about value, not about difficulty.} A public system routes with a typed question about
how much reasoning an item needs. On trained decision models the value gate is +1.23 {[}+0.76,
+1.71{]} (4B) and +0.76 {[}+0.42, +1.11{]} (9B) points above that question at a 20\% think rate. On
untrained base models, where nearly every item gains from reasoning, the two are level
(Appendix~\ref{sec:E.7}).

Which training items set the confidence after reasoning (the items the gate routes) is tested in
Appendix~\ref{sec:E.8}.

\subsection{Decision models as verifiers}\label{sec:7.7}

Here the released models, used as verifiers without training for verification, are compared with
other judges (Appendix~\ref{sec:B.6}).

\textbf{A decision model is a better judge than a chat model of three times its size.} Our 4B is 8
to 11 points above Phi-4-mini-instruct used as judge on the three problem sets
(Table~\ref{tab:7.1}a). Gemma-3-12b reaches 89.9 / 78.3 and Phi-4 (14B) 90.6 / 78.4 on the first
two, against the 4B's 92.5 / 82.1.

Against another team's decision models the 27B is ahead: by +2.5 {[}+1.6, +3.4{]} and +2.9 {[}+2.3,
+3.5{]} points over Clef 27B, and by 6.0 points on the reasoning sets (82.97 against 77.01). Our 9B
is at least level with Clef 27B.

\textbf{Eight verified samples beat a 64-sample vote.} A 9B verifying 8 samples of a 2B generator
reaches 91.0 against 89.1 for the majority vote over 64 (Figure~\ref{fig:B.1}). On five unseen
datasets verification adds 5.6 (9B) to 8.3 (27B) points. With a weak verifier more samples can lower
accuracy: from N = 8 to 256 on one unseen dataset the 4B loses 6.0 points {[}$-$7.4, $-$4.6{]} while
the 27B gains 1.7 {[}+0.7, +2.8{]} on the same samples (Appendix~\ref{sec:B.3}).

A verifier that does not know the fact cannot check it. In closed-book question answering (8,000
questions, N = 16) best-of-16 is 0.1--2.7 points above the vote with the 4B generator and 0.9--2.3
points below it with Phi-4 as generator. The selection effect is at its largest there: +6.9 to +17.5
points.

\subsection{Recommendations}\label{sec:7.8}

\begin{mdbox}{7.1}{box:7.1}
\textbf{Box~\ref{box:7.1}. Acting on a reported probability after selecting or routing.}

\begin{enumerate}
\item \textbf{Calibrate on what the system returns.} Run the deployed policy (the same N, the same
generator, the same gate threshold) on labelled calibration problems, and fit or certify on the
answers it returns, separately per route.
\item \textbf{Certify with a finite-sample test, split by source problem} (Section~\ref{sec:7.4}). Expect
the certificate to refuse some routes.
\item \textbf{Before building a gate, measure the residual AUROC} of the routing score for the answer that
will be reported, within bins of the reported confidence. At 0.5 the usual calibration is safe. Away
from 0.5 its sign says which side will be overconfident.
\item \textbf{For selection among samples, give the calibration map the candidate set:} the selected
score, the mean score of the candidates and N. Fit it at a few values of N, and do not rely on a
certified threshold far beyond them.
\item \textbf{Repeat steps 1 and 2 when the policy changes}: another N, another think rate, another
generator, another task family. A certificate is marginal over the calibration distribution.
\end{enumerate}

\textbf{What transfers:} the set-aware map to values of N near the fitted ones, one temperature for
the thought path to unseen task families, and a value gate trained on the 4B's labels to the 27B.
\textbf{What does not:} a certified threshold to another N, think rate or task family, a map to
another problem distribution, and a guarantee for all answers to the answers of one route.
\end{mdbox}


==> sections/08_limitations.tex <==
\clearpage
\section{Limitations and negative results}\label{sec:8}

\textbf{Limitations.}

\begin{itemize}
\item \emph{The index is mostly in-domain for the later checkpoints.} After the data rounds 33 of its 38
benchmarks have training data aimed at them, and the gain from 63.9 to 70.4 at 27B measures the fit
of the recipe to the suite. On decisions the rounds were not aimed at they change the score by
$-$1.0 at 27B and by nothing at 9B and 4B.
\item \emph{Every index value includes GSM8K rows that can be answered from the layout of their options},
about 0.8 index points for the released 27B and 1.2 for the released 4B. No value has been
recomputed with the rebuilt rows.
\item \emph{No measurement on the private tests of edition 0.3.} Our local stand-ins have limits of their
own: the generated tasks are ours and new, the reused tasks favour whoever trained on related
material, and a twin measures transfer only for a model that has not trained on its family.
\item \emph{Decontamination at the release was partial.} Rebuilt training splits were scanned and not
filtered, and 68 rows repeat a test item. The comparison finds equal text, not paraphrases.
\item \emph{Single rounds.} Most comparisons between training rounds rest on one round per condition. The
same recipe trained twice differs by 0.18 index points and by up to 7 points on one benchmark, and a
second run of the final recipe at 4B was still running when this was written.
\item \emph{Reasoning is incomplete and costly at 4B and 9B.} The untrained starting models still think
better on arithmetic than ours (97.1 and 98.6 against 94.4 and 96.3), the 0.8B and 2B have no
reasoning stages, and a thought lowers accuracy on select-all and NLI-like questions. One threshold
and one mixture weight serve all task families.
\item \emph{Images and long inputs are inherited abilities.} Decision training used text only, and long
inputs were measured on documents up to 128K tokens and retrieval items up to 248K, not at the full
context.
\item \emph{Certificates are marginal and local.} A certificate holds for the calibration distribution,
the policy and the number of candidates it was computed for, and it does not transfer across task
families.
\item \emph{Data.} No person has audited the written and generated training data, teacher-written rows
were filtered by two verifier models, and several sources carry share-alike, non-commercial or
research-only terms.
\end{itemize}

\textbf{What did not work.} Each item is reported where it occurred. They are results for our
models, data and settings and do not show that an idea cannot work elsewhere.

\begin{itemize}
\item \emph{Training the one-pass model.} A second-stage adapter on rows the first model gets wrong (all
eleven runs below their parent). All weights trained from the untrained 4B with the settings of the
leading entries (40.87 and 44.71 against 52.76 for the released 4B). More rows of the same families
(65.6 against 65.7 on the twins at 1.7 times the rows). Distantly labelled sarcasm data and other
stance data sets, which lowered their twins. Removing VAST against the stance bias (the stance twin
fell from 38.7 to 29.5). Breadth rows alone at 4B, which moved no overall score.
\item \emph{Data that looked right.} An official training set whose label prior differs from the
benchmark's (63.3 $\rightarrow$ 36.5 on that benchmark at 4B), generated code-execution rows
(24.9--27.1 $\rightarrow$ 13.4--15.1), and a duplicate filter keyed on the wrong fields.
\item \emph{Reasoning.} A longer token limit (87.4\% of the thoughts still running at 16,384 tokens), a
lower gate on the index (67.20 against 67.72), one joint stage in place of three (67.11),
reinforcement learning as a way to better answers (no arm above the supervised stages), two-stage
``calibrate, then reinforce'' training (three points of the one-pass answer lost), and thinking
again when the confidence is below 0.6 (73.41 against 73.44 with the first thought in context).
\item \emph{Serving.} Prefix caching and chunked prefill in a third-party server changed results
(Chapter~\ref{sec:7}), and 8-bit weight formats were slower than bf16 on H200.
\end{itemize}

\textbf{Intended use.} Typed decisions inside a system that a person or a program has framed:
routing and triage, checks on inputs and outputs, relevance and matching, verification of an answer
against evidence, choosing among candidate responses. A threshold should be set on labelled examples
of the deployment's own data, and a probability that was used to select an answer should not be
reported as the accuracy of the selected answers without the calibration of Section~\ref{sec:6.5}.
The models are not meant for decisions about individuals in medicine, law, credit, employment or
safety without review by a qualified person, nor as the only guard against harmful content, and the
weights may not be used commercially.


==> sections/08_serving.tex <==
\clearpage
\section{Inference and serving}\label{sec:8}

A decision model is used inside other systems, so what it costs and how it is served are part of
what it is. Table~\ref{tab:8.1} gives the latency of every size, and the next subsection the number
of requests one node answers per hour. The sections after it cover requests with many questions
(8.2), long inputs (8.3), engine settings that changed our results (8.4), the operation of long runs
(8.5) and the cost of reasoning (8.6). Versions, flags and the tests that reproduce those faults are
in Appendix~\ref{sec:J}.

\subsection{Latency and throughput}\label{sec:8.1}

\begin{table}[!htbp]
\renewcommand{\thetable}{8.1}
\centering
\caption{Latency and throughput of the released models on one H200 in bf16 with the released runtime (PyTorch 2.11, transformers 5.8.1, linear-attention kernels, recorded CUDA graphs). Latency: end to end over HTTP, one request at a time, 20 warm-up and 200 timed requests, measured between 2026-09-27 and 2026-10-01. The three-question request holds one choice, one yes/no and one score question about a support ticket, 891 prompt tokens in all, answered in one forward pass. Throughput and memory: one call with 256 yes/no questions about a 316-token document, 2026-10-06.}\label{tab:8.1}
{\footnotesize\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrr}
\toprule
\textbf{model} & {\begin{tabular}[b]{@{}r@{}}\textbf{three questions:}\\\textbf{mean / P50 / P95}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{one}\\\textbf{yes/no}\\\textbf{question}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{decisions}\\\textbf{per}\\\textbf{second}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{peak GPU}\\\textbf{memory in}\\\textbf{that test}\end{tabular}} \\
\midrule
StartLux-Decision-0.8B & 12.2 / 12.2 / 14.2 ms & 8.3 ms & 370 & 6.99 GiB \\
StartLux-Decision-2B & 15.5 / 15.5 / 17.2 ms & 9.6 ms & 241 & 9.72 GiB \\
StartLux-Decision-4B & 26.0 / 26.0 / 27.3 ms & 14.7 ms & 113 & 17.75 GiB \\
StartLux-Decision-9B & 35.7 / 36.2 / 37.4 ms & 17.6 ms & 72 & 27.53 GiB \\
StartLux-Decision-27B & 102.3 / 102.5 / 104.3 ms & 50.7 ms & 23 & 64.96 GiB \\
StartLux-Decision-35B-A3B & 52.5 / 52.9 / 54.5 ms & 36.4 ms & \todo{} & about 71 GiB \textsuperscript{a} \\
StartLux-Decision-4B without recorded graphs & 90.3 / 89.5 / 92.5 ms & 87.5 ms & -- & -- \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{a} peak stated with the release of this model, not measured in this test.
\todo{Figure 8.1, latency against size, redrawn from this table under the figure rules of the
report}\par}
\end{table}

A request with three questions takes 12 ms on the 0.8B and 102 ms on the 27B. The 35B-A3B, a mixture
of experts with about 3B of its 35B parameters active for each token, answers in half the time of
the 27B and fits one 80 GB GPU. For the same two requests the gateway of the hosted reference
reports 64.0 and 63.5 ms of server time (means of 100 requests each, own API run of 2026-09-29). End
to end from our cluster the time is about 330 ms, of which about 260 ms is the network. The authors
of Intern-Decision report 34.0, 33.3 and 44.2 ms for their 0.8B, 2B and 4B on an RTX 4090 for a
request of the same shape. The hardware is different, so this is a rough reference only.

Three things make the one-pass path fast. The linear-attention layers need two kernel packages.
Without them the model library falls back, without an error, to an implementation that is more than
ten times slower, so the server refuses to start where they are not active. Nothing is generated:
one forward pass per request, one batch row per question, and only the 26 output rows of the option
letters are multiplied. And short requests are replayed from 40 recorded CUDA graphs, which removes
the kernel-launch overhead that dominates short inputs (26.0 against 90.3 ms at 4B,
Appendix~\ref{sec:J.4}). The released server answers one request at a time per GPU. Throughput comes
from one server per GPU behind a load balancer (in a closed-loop test on a node of eight H200s the
27B served 81 three-question requests per second and the 35B-A3B 170) or from the bulk path, which
packs the questions of many requests into forward passes of up to 65,536 tokens: a full one-pass
index run of the 4B takes about 25 minutes on five H200s.

\subsubsection{Capacity on one node with eight H200}\label{sec:8.1.1}

The latencies above are for one request at a time. This section asks how many requests one node with
eight H200 GPUs answers per hour under full load. It has four parts: an offline test of the 9B by
request length and weight format, an end-to-end figure from stored index runs for three sizes, an
online test with a front end, and a short load test of the hosted reference as a point of
orientation. All of it was measured on 7 October 2026 and all of it is about speed. None of these
runs is an accuracy result.

\begin{table}[!htbp]
\renewcommand{\thetable}{8.6}
\centering
\caption{Offline capacity of the 9B on one node with eight H200: requests per hour for the node, by state length and weight format (synthetic requests with a state of fixed length and one four-option question, released runtime, one process per GPU, full load, 40 seconds per point). bf16: the weights as released. int8: 8-bit integer weights (torchao 0.17, without compilation). float8: 8-bit floating-point weights and activations.}\label{tab:8.6}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrr}
\toprule
\textbf{state length} & {\begin{tabular}[b]{@{}r@{}}\textbf{bf16, as}\\\textbf{released}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{int8}\\\textbf{weights}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{float8}\\\textbf{weights and}\\\textbf{activations}\end{tabular}} \\
\midrule
256 tokens & 2,390,000 \textsuperscript{a} & 2,196,700 & 2,191,500 \\
1,024 tokens & 721,500 & 663,100 & 659,400 \\
4,096 tokens & 172,100 & 158,600 & 158,000 \\
16,384 tokens & 50,300 & 44,900 & 40,200 \\
weights per GPU & 16.7 GB & 10.2 GB & 10.2 GB \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{a} this run overlapped for about a minute with the end of another job on the node.
The point is not used in the comparison of the formats.\par}
\end{table}

\emph{Offline, by length and format.} In bf16 the node answers 721,500 requests per hour at 1,024
tokens and 50,300 at 16,384 tokens (Table~\ref{tab:8.6}). Over the four lengths that is 612 to 825
million input tokens per hour for the node, or about 77 to 103 million per GPU-hour. \textbf{The
8-bit formats are slower on this hardware, not faster}: at 1,024 to 16,384 tokens by 8 to 11\% with
integer weights and by 8 to 20\% with 8-bit floating point. They save 6.5 GB of weights per GPU, but
in this test the GPU is limited by computation and not by memory. Their accuracy has not been
evaluated. On one ambiguous test request the two 8-bit formats moved the probabilities by two to
three points and disagreed on the top option, so we report them as a speed measurement only. The
accuracy results of this report are from bf16 weights.

\begin{table}[!htbp]
\renewcommand{\thetable}{8.7}
\centering
\caption{End-to-end rates from stored index runs on one node with eight H200 (Decision Index 0.2.1: 133,876 requests with a mean of 880 tokens, a median of 325 and a 90th percentile of 1,452, batched offline runner, with the time to load the model included). Tokens per GPU-hour: the node's rate divided by eight. Reasoning: the default control of Section~\ref{sec:3.4}.}\label{tab:8.7}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrlll}
\toprule
\textbf{size} & {\begin{tabular}[b]{@{}r@{}}\textbf{one pass:}\\\textbf{requests}\\\textbf{per hour}\end{tabular}} & {\begin{tabular}[b]{@{}l@{}}\textbf{input}\\\textbf{tokens}\\\textbf{per hour}\end{tabular}} & {\begin{tabular}[b]{@{}l@{}}\textbf{input}\\\textbf{tokens per}\\\textbf{GPU-hour}\end{tabular}} & \textbf{reasoning at the default threshold: requests per hour} \\
\midrule
4B & 576,000 & 507 million & 63 million & 88,600 after the stop step, 143,700 after reinforcement learning \textsuperscript{b} \\
9B & 402,000 & 354 million & 44 million & 41,600 after the stop step (3 h 13 min for the index) \\
27B & 136,000 & 120 million & 15 million & -- \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{b} \todo[TODO(which reinforcement-learning arm of Section 5.9 this 4B run is; our
record says ``4B after RL'')]{}\par}
\end{table}

\emph{End to end.} On the request mix of the index the node answers 402,000 requests per hour with
the 9B, 576,000 with the 4B and 136,000 with the 27B (Table~\ref{tab:8.7}). With reasoning the rate
is set by how much a model writes: the 9B after the stop step, the stage that teaches a model to end
its thoughts, answers 41,600 requests per hour, about a tenth of the one-pass rate of that size, and
the 4B after the stop step 88,600.

\emph{Online, with a front end.} The offline figures say what the GPUs can do. A service also needs
a front end. We tested the 9B behind one that was written the same day: eight server processes, one
per GPU, each a thread-per-connection HTTP server in Python that collects requests for 10 ms into a
batch. The client ran on the node and sent requests whose lengths were drawn from the request mix of
the index. With 256 concurrent clients the node answered 41.5 requests per second at a median
latency of 3.2 s. With 512 clients it answered 63.7 per second at 7.5 s. With 1,024 clients it
answered 94.7 per second, which is 340,800 per hour, at a median of 10.5 s and a 99th percentile of
22 s. No request failed. A first step with 128 clients, at 13 requests per second, was taken while
the servers were warming up. The mean batch held 17 requests: the Python front end, not the GPU, is
the limit in this test. It reaches 85\% of the offline rate for the same request mix only with a
queue of several seconds. \todo[TODO(online9\_1007)]{the released server and the 8-bit formats
behind the same client}

\emph{A point of orientation: the hosted reference.} We sent a request stream of the same kind to
the public interface of the hosted reference for ten minutes (7 October 2026, 18:55 to 19:05, from
our workstation, using synthetic requests and nothing from an evaluation set). At 70 requests per
second for five minutes, 21,000 of 21,000 requests were answered, with a median latency of 0.25 s, a
90th percentile of 0.61 s and a 99th percentile of 1.41 s, at 78,400 billed input tokens per second.
At 100 requests per second for five minutes, 30,000 of 30,000 were answered, with 0.25, 0.61 and
1.33 s, at 111,900 billed tokens per second. The documented limits are 80 requests and 100,000
tokens per second. No request was refused at either rate, and we did not look for the rate at which
the service stops. A request was billed with about 300 tokens more than its content (a mean of 1,120
for a content of about 820), 57.08 million input tokens in all. The two online tests are not like
for like: the hosted figures include the network from our workstation and a production front end,
ours a front end of one day with the client on the node. The comparison says where our serving stack
stands, not what the models can do. At 100 requests per second the hosted service answers with a
median latency of a quarter of a second. With the 9B our node has the GPU capacity for that rate on
this request mix (402,000 requests per hour offline), and online it delivered 94.7 requests per
second behind a queue of several seconds.

\subsection{Many questions per request and the shared-prefix runtime}\label{sec:8.2}

Every question of a request is one row of the batch, so a request with 1,024 questions runs, and its
probabilities differ from those of 1,024 single requests by at most 0.008. What the questions cost
depends on a threshold in the runtime. Below 4,096 shared tokens every row carries the whole
document. Above it the document is read once and the questions run on top of it.

\begin{table}[!htbp]
\renewcommand{\thetable}{8.2}
\centering
\caption{Decisions per second for 256 yes/no questions about one document in one call, released weights, one H200, bf16, 2026-10-06. Upper block: the released runtime, which shares the document from 4,096 tokens. Lower block: the same runtime with sharing from 256 tokens. All question counts: Appendix~\ref{sec:J.7}.}\label{tab:8.2}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{llrrrrr}
\toprule
\textbf{document} & \textbf{path} & \textbf{0.8B} & \textbf{2B} & \textbf{4B} & \textbf{9B} & \textbf{27B} \\
\midrule
316 tokens & every question carries the document & 370 & 241 & 113 & 72 & 23 \\
1,099 tokens & every question carries the document & 127 & 83 & 39 & 25 & 7.9 \\
3,217 tokens & every question carries the document & 44 & 29 & 13 & 8.6 & 2.8 \textsuperscript{a} \\
6,077 tokens & document read once & 74 & 78 & 67 & 57 & 37 \\
16,038 tokens & document read once & 26 & 24 & 16.5 & 14.5 & 6.8 \\
64,217 tokens & document read once & 7.8 & 7.6 & 6.5 & 6.5 & -- \\
316 tokens & document read once, sharing from 256 tokens & 436 & 357 & 195 & 138 & 47 \\
1,099 tokens & document read once, sharing from 256 tokens & 266 & 241 & 154 & 116 & 43 \\
3,217 tokens & document read once, sharing from 256 tokens & 141 & 135 & 101 & 82 & 36 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{a} at 128 questions. Larger requests were not measured for this cell.\par}
\end{table}

Below the threshold the throughput is flat in the number of questions and falls with the document
(Table~\ref{tab:8.2}), which produces an anomaly: 256 questions about a 6,077-token document are
answered five times (4B) and thirteen times (27B) faster than about a document half as long.
Lowering the threshold to 256 tokens removes it. With few questions sharing is the slower path (two
questions about 1,099 tokens run at 18 against 35 per second at 4B) and the two paths cross at about
eight questions for the 2B, between four and eight for the 4B, and below four for the 9B and the
27B. The threshold should therefore depend on the number of questions and on the model. The released
runtime does not do this yet.

\subsection{Long-context runtime}\label{sec:8.3}

For a long state the questions share the evidence. The runtime reads the shared beginning once, in
chunks of 32,768 tokens, and keeps what each layer carries forward: the keys and values of the
attention layers and the convolution and recurrent state of the linear-attention layers. All
questions then run as one batch on top of it, and a single question over a long document takes the
same path, so memory stays close to the keys and values of the prompt instead of growing with the
activations of the whole input. Attention over the stored keys needs no mask: a chunk attends to the
earlier keys without a mask and to its own keys causally, in two fused calls whose outputs are
merged by their log-sum-exp.

\begin{table}[!htbp]
\renewcommand{\thetable}{8.3}
\centering
\caption{Long inputs on one H200, bf16, released weights (2026-10-01 to 2026-10-03). ``Before'' is the earlier runtime, which padded every row to the full length and built an attention mask.}\label{tab:8.3}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrr}
\toprule
\textbf{model} & {\begin{tabular}[b]{@{}r@{}}\textbf{128,000 tokens,}\\\textbf{three questions:}\\\textbf{before $\rightarrow$ after}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{one question,}\\\textbf{8--32K tokens}\\\textbf{(median)}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{one question,}\\\textbf{32--128K tokens}\\\textbf{(median)}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{one question,}\\\textbf{248K tokens}\end{tabular}} \\
\midrule
StartLux-Decision-4B & 44.5 $\rightarrow$ 5.2 s & 0.51 s & 2.5 s & 12 s \\
StartLux-Decision-9B & 48.5 $\rightarrow$ 6.5 s & 0.79 s & 3.3 s & \todo{} \\
StartLux-Decision-27B & 146.8 $\rightarrow$ 19.3 s & 2.3 s & 10 s & 45.7 s \\
StartLux-Decision-35B-A3B & 55.3 $\rightarrow$ 6.6 s & 0.70 s & 3.3 s & 15.7 s \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

The time for 128,000 tokens with three questions falls by a factor of 7.5 to 8.6
(Table~\ref{tab:8.3}), and the memory above the weights from 61--68 GiB to 5--11 GiB, so the 35B-A3B
answers at 128,000 tokens on one 80 GB GPU (peak 72.8 GiB). The answers do not change: on 397
long-document items the mean change of the probability of the correct option is within $\pm$0.001
for every size, and the answers that change are near-ties. A long list over a long document reuses
the stored beginning within one request, which halves its cost (60 options at 128K tokens: 12.6
$\rightarrow$ 6.7 s with identical probabilities). \todo{time and peak memory at 256K per size}

\subsection{Engine settings that change results}\label{sec:8.4}

The read-out is deterministic, so two paths that serve the same weights must agree. They did not
always. Table~\ref{tab:8.4} lists the settings that changed answers in our runs. The first two cost
us wrong conclusions: with prefix caching on, a third-party inference server returned different
read-outs for the same rows, and with its default chunked prefill every reasoning run of ours until
6 October under-scored tool benchmarks, which we first read as ``reasoning pays in knowledge and
costs in tool selection''.

\begin{table}[!htbp]
\renewcommand{\thetable}{8.4}
\centering
\caption{Settings that changed results. Rows 1 to 4 concern the generation server that we use for reasoning runs (vLLM 0.19.1). The batch runner of the released package is the reference.}\label{tab:8.4}
{\footnotesize\setlength{\tabcolsep}{5pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{\mdw{0.2013}}>{\raggedright\arraybackslash}p{\mdw{0.2406}}>{\raggedright\arraybackslash}p{\mdw{0.3541}}>{\raggedright\arraybackslash}p{\mdw{0.1903}}}
\toprule
\textbf{setting} & \textbf{symptom} & \textbf{size of the error} & \textbf{fix} \\
\midrule
1. prefix caching on (the server marks the cache mode for this architecture as experimental) & one-pass read-outs differ for the same rows & 2.6\% of the read-outs moved by more than 0.05, 16\% of the answers on lists over 26 options flipped & caching off everywhere \\
2. prefill in chunks of 8,192 batched tokens (the default) & a prompt whose prefill is split between two scheduler steps is read wrongly. Hit: the groups of a long list and the questions of one request, sent at once & 4B after data rounds, one pass, server against batch runner: same choice in 96.0\% on a 53-tool selection benchmark (accuracy 82.8 against 85.2), 93.9\% on chords with 129 labels (76.4 against 80.3), 98.4\% on a multi-question simulator, and index with reasoning 65.01 instead of 66.38 & prefill in one piece (no chunking, 65,536 batched tokens): 99.4\%, 99.3\%, 100.0\% \\
3. the server applies the checkpoint's sampling defaults (top-k 20, top-p 0.95) to the read-out & the letter distribution is truncated & \todo{not measured} & neutral generation settings and processed log-probabilities of 26 tokens for read-out requests \\
4. new reasoning requests join a running decode batch & thoughts turn into garbage loops & 43--50 of 183 thoughts, 0 of 183 when all are sent at once & reasoning requests go out in waves per server \\
5. FP8 with padded batches & an all-zero padding row gets a zero scale, produces NaN and leaks into real rows & agreement with bf16 falls to about 52\% & FP8 with one question per forward pass, no padding \\
6. thought budget of 1,024 tokens on a 4B & 15--72\% of the thoughts on reasoning benchmarks are cut & accuracy 39\% at the limit against 89\% for finished thoughts on a code-execution benchmark & 4,096 tokens \\
7. a run with unanswered requests scored as complete & unanswered requests count as wrong & 61.31 at coverage 0.960, 66.36 once the missing 5,606 requests were answered & coverage of at least 0.999, retry passes \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

Under row 2 single questions are hardly touched (batch runner and server agree on 98 to 99.9\% of
them whatever the prompt length), and the damage sits in requests that put several long prompts with
a common beginning into the server at once. On the corrected servers the tools area is at its
one-pass level (86.1 against 86.0) and no benchmark loses more than 1.4 points to reasoning. The
offline engine behind the diagnostic read-outs of Chapter~\ref{sec:7} has the same default.
Re-reading its stored thoughts with prefill in one piece changes the top option of 0.4--0.9\% of the
answers and leaves the accuracy within 0.1 points, so those results stand. Two lessons generalise:
compare a serving path with a batch runner on the longest lists and on multi-question requests, not
on an average benchmark, and distrust a loss that appears where the model does the least reasoning.
Every reasoning number in Chapters~\ref{sec:6} and \ref{sec:8} is from the corrected path, or is
marked \dag{}. The tests are in Appendix~\ref{sec:J.5}.

\subsection{Operations}\label{sec:8.5}

One-pass serving needs little: one server per GPU, a load balancer, and two start-up checks (kernels
active, recorded graphs equal to the unrecorded path within 0.02, which holds with a difference of
0.0 for all six models).

Reasoning runs are long and exposed to a fault that we have not removed. A generation engine of this
architecture occasionally stops in the middle of a run: it reports requests in progress, processes
no token, and shows full GPU load. We counted five such stops in about 110 server-hours, always
after a burst of new requests. Three measures make a run survive them (Appendix~\ref{sec:J.6}). A
watchdog reads the token counters of every engine each 30 seconds and restarts an engine that has
requests running and no progress for two minutes. The load balancer sends a failed request to up to
two other engines and leaves a failing engine out for 30 seconds. It also raises its limit on open
files, because with 512 concurrent requests one stopped engine exhausted the default limit and
38,461 of 133,100 requests of one run failed at once. And requests that failed or were never
answered are sent again in up to three passes, after which a run is used only if its coverage is at
least 0.999. With these in place three engines stopped during one 4B run, each was restarted within
three and a half minutes, and the first pass ended without a failed request. The cause is open: a
second prefill kernel of the server gives the same answers (same choice in 99.82\% of 34,677
answers) and had no stop in one run where its twin had three, which at the observed rate happens
four times in ten by chance.

\subsection{Cost of a reasoned run}\label{sec:8.6}

Reasoning multiplies the cost of the questions it is used for and leaves the others at the cost of
one pass. With fewer than half of the questions reasoned about, the median latency is that of the
one-pass path.

\begin{table}[!htbp]
\renewcommand{\thetable}{8.5}
\centering
\caption{Cost of index runs with reasoning at the default threshold (133,876 requests, 337,742 answers, 512 concurrent requests, 4,096-token budget, corrected serving path, eight H200s with one engine each, 2026-10-06). Rows name the StartLux-Decision size.}\label{tab:8.5}
{\scriptsize\setlength{\tabcolsep}{3pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{llrrr}
\toprule
\textbf{run} & \textbf{wall-clock} & {\begin{tabular}[b]{@{}r@{}}\textbf{answers}\\\textbf{reasoned}\\\textbf{about}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{tokens}\\\textbf{per}\\\textbf{thought}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{reasoning}\\\textbf{tokens per}\\\textbf{answer}\end{tabular}} \\
\midrule
4B released, one pass, bulk path on five H200s & about 25 min & -- & -- & -- \\
4B after data rounds, reasoning & about 1 h & 32.2\% & 388 & 125 \\
4B, a second reader variant, two runs & 46 and 48 min (first pass) & 32.2\% & 264 & \todo{} \\
9B after data rounds, reasoning & 3.5 h & 29.0\% & 2,611 & 758 \\
27B after data rounds without the last four sources, reasoning & \todo{}, four nodes & 27.5\% & 458 & 126 \\
4B after data rounds and thinking replay, reasoning & 2 h 44 min & 33.3\% & 3,439 & 1,144 \\
9B after data rounds and thinking replay, reasoning & 3.5 h & 29.8\% & 3,517 & 1,049 \\
27B after data rounds and thinking replay, reasoning & 8.8 node-hours (four parts of 2.2 h, one node each) & 27.2\% & 710 & 193 \\
4B after the stop step, reasoning & 1 h 40 min & 31.3\% & 1,585 & 497 \\
9B after the stop step, reasoning & -- (run resumed after an interruption) & 29.1\% & 1,900 & 552 \\
4B trained with reinforcement learning, reasoning & 52 min & 31.1\% & 184 & 57 \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

The cost of a reasoned run is set by how much the model writes, not by how often it reasons: the
share of answers reasoned about is 27 to 33\% in every row of Table~\ref{tab:8.5}, and the tokens
per thought differ by a factor of thirteen. The 9B takes three and a half hours where the 4B takes
one because its thoughts run on after the answer is found. Thinking replay makes the 4B's thoughts
nine times longer for 1.3 more index points. The threshold is the user's lever on this cost: on
held-out items $\tau$ = 0.7 gives the accuracy of $\tau$ = 0.9 for 714 instead of 1,322 tokens per
item (Table~\ref{tab:6.11}). The lever is not free everywhere: on the index the same 4B scores 67.20
with $\tau$ = 0.7 against 67.72 with $\tau$ = 0.9 (Section~\ref{sec:5.1.2}), so a lower threshold
should be checked on the user's own data. Concurrency and budget matter as much as the model: an
earlier 9B run with a 1,024-token budget and 512 concurrent requests finished in 93 minutes, while
the same model with a 4,096-token budget and 128 concurrent requests ran at 94 requests per minute,
a day for the index. \todo{price assumption per GPU-hour and cost per 1,000 decisions, one pass and
reasoned, for every size; latency distribution of reasoned requests; the documented price of the
hosted reference for comparison}

\subsection*{Findings of this chapter}

\begin{mdfindings}
\textbf{A read-out that should be deterministic is the best test of a serving path}: two server
settings changed answers without an error message, and one of them cost 1.4 index points and a wrong
conclusion.

\textbf{Sharing the document pays from a handful of questions, not from 4,096 tokens}: with sharing
from 256 tokens a 3,217-token document is answered three to thirteen times faster at 256 questions.

\textbf{Reasoning cost follows thought length}: the share of reasoned answers is nearly constant
across models, and tokens per thought range from 68 to 3,517.

\textbf{On H200 the 8-bit weight formats are slower than bf16, not faster}: by 8 to 20\% at 1,024 to
16,384 tokens for the 9B, with 6.5 GB less memory per GPU and an accuracy that has not been
evaluated.

\textbf{One node with eight H200 answers 402,000 index-like requests per hour with the 9B offline,
and the front end is what limits it online}: 576,000 with the 4B and 136,000 with the 27B. Behind a
same-day Python front end the 9B reaches 94.7 requests per second at a median latency of 10.5 s.
\end{mdfindings}


==> sections/08_serving_cost.tex <==
\section{Serving and cost}\label{sec:8}

A decision model is used inside other systems, so what it costs is part of what it is. A request
with three questions takes 12 ms on the 0.8B and 102 ms on the 27B on one H200 GPU
(Table~\ref{tab:19}), and the 35B-A3B, with about 3B of its 35B parameters active per token, answers
in half the time of the 27B on one 80 GB GPU.

\begin{table}[!htbp]
\renewcommand{\thetable}{19}
\centering
\caption{One-pass latency runs from 12.2 ms on the 0.8B to 102.3 ms on the 27B, and the mixture of experts answers in about half the time of the 27B. Latency and throughput of the released models on one H200 in bf16 with the released runtime. Latency: end to end over HTTP, one request at a time, 20 warm-up and 200 timed requests. The three-question request holds one choice, one yes/no and one score question about a support ticket (891 prompt tokens), answered in one forward pass. Throughput and memory: one call with 256 yes/no questions about a 316-token document.}\label{tab:19}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrrrr}
\toprule
\textbf{model} & {\begin{tabular}[b]{@{}r@{}}\textbf{three questions:}\\\textbf{mean / P95}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{one}\\\textbf{yes/no}\\\textbf{question}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{decisions}\\\textbf{per}\\\textbf{second}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{peak GPU}\\\textbf{memory in}\\\textbf{that test}\end{tabular}} \\
\midrule
StartLux-Decision-0.8B & 12.2 / 14.2 ms & 8.3 ms & 370 & 6.99 GiB \\
StartLux-Decision-2B & 15.5 / 17.2 ms & 9.6 ms & 241 & 9.72 GiB \\
StartLux-Decision-4B & 26.0 / 27.3 ms & 14.7 ms & 113 & 17.75 GiB \\
StartLux-Decision-9B & 35.7 / 37.4 ms & 17.6 ms & 72 & 27.53 GiB \\
StartLux-Decision-27B & 102.3 / 104.3 ms & 50.7 ms & 23 & 64.96 GiB \\
StartLux-Decision-35B-A3B & 52.5 / 54.5 ms & 36.4 ms & -- \textsuperscript{a} & about 71 GiB \textsuperscript{a} \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\par\smallskip
{\footnotesize\raggedright\noindent \textsuperscript{a} the throughput test was not run on this model, and its peak memory is the one
stated with its release.\par}
\end{table}

Three things make the one-pass path fast. The linear-attention layers need two kernel packages, and
without them the model library falls back, without an error, to an implementation that is more than
ten times slower, so the server refuses to start where they are not active. Nothing is generated,
and only the output rows of the option letters are multiplied. And short requests are replayed from
recorded CUDA graphs, which removes the kernel-launch overhead that dominates short inputs (26.0
against 90.3 ms at 4B). For long inputs the runtime reads the shared beginning of a request once and
runs all questions on top of it: 128,000 tokens with three questions take 19.3 s instead of 146.8 s
on the 27B, with probabilities unchanged within $\pm$0.001.

\textbf{Capacity of one node.} On one node with eight H200 GPUs and the request mix of the index (a
mean of 880 tokens), the batched offline runner answers 576,000 requests per hour with the 4B,
402,000 with the 9B and 136,000 with the 27B (Table~\ref{tab:20}). Online, the release package's own
server answered the request stream that we also sent to the hosted service at 116.0 requests per
second with a median latency of 0.031 s (99th percentile 0.618 s) for 8 concurrent clients, and at
177.8 requests per second with a median of 0.101 s for 64 clients (9B in bf16, client on the node, 7
October 2026). The hosted service held 100 requests per second at a median of 0.25 s including the
public network (99th percentile 1.33 s) without reaching its limit, so the two latencies are not
like for like. We trail in two places. At 64 clients our 90th and 99th percentiles (1.226 and 1.632
s) are above the hosted service's (0.61 and 1.33 s), because each GPU serves one request at a time
and the others queue. And 8-bit weight formats were 8 to 20\% slower than bf16 at 1,024 to 16,384
tokens for the 9B, because this GPU is limited by computation and not by memory, and their accuracy
has not been evaluated.

\begin{table}[!htbp]
\renewcommand{\thetable}{20}
\centering
\caption{One node answers 136,000 to 576,000 index requests per hour in one pass, and the 9B answers about a tenth as many with reasoning. End-to-end rates on one node with eight H200 GPUs from stored index runs (133,876 requests with a mean of 880 tokens, a median of 325 and a 90th percentile of 1,452, batched offline runner, model load included). Reasoning: the default threshold of the -Think checkpoints after the stop step.}\label{tab:20}
{\small\setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}
\noindent\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lrllr}
\toprule
\textbf{size} & {\begin{tabular}[b]{@{}r@{}}\textbf{one pass:}\\\textbf{requests}\\\textbf{per hour}\end{tabular}} & {\begin{tabular}[b]{@{}l@{}}\textbf{input}\\\textbf{tokens}\\\textbf{per hour}\end{tabular}} & {\begin{tabular}[b]{@{}l@{}}\textbf{input}\\\textbf{tokens per}\\\textbf{GPU-hour}\end{tabular}} & {\begin{tabular}[b]{@{}r@{}}\textbf{reasoning:}\\\textbf{requests}\\\textbf{per hour}\end{tabular}} \\
\midrule
4B & 576,000 & 507 million & 63 million & 88,600 \\
9B & 402,000 & 354 million & 44 million & 41,600 \\
27B & 136,000 & 120 million & 15 million & -- \\
\bottomrule
\end{tabular}
\end{adjustbox}\par}
\end{table}

\textbf{Cost of reasoning.} Reasoning multiplies the cost of the questions it is used for and leaves
the others at the cost of one pass. In every index run with reasoning 27 to 33\% of the answers were
reasoned about, while the tokens per thought differed by a factor of thirteen between models. The
cost is therefore set by how much a model writes, not by how often it reasons. With reasoning at the
default threshold, the 9B after the stop step answers 41,600 index requests per hour on the node,
about a tenth of its one-pass rate, and one index run of the 27B with reasoning took 8.8 node-hours.
The threshold is the user's lever on this cost, and it should be checked on the user's own data. All
of these figures are time on H200 GPUs of our own cluster, and we state no price per GPU-hour.

\textbf{Settings that change results.} The read-out is deterministic, so two paths that serve the
same weights must agree, and they did not always. Prefix caching in a widely used inference server
moved 2.6\% of the one-pass read-outs by more than 0.05, and its default chunked prefill cost
reasoning runs 1.4 index points at 4B (65.01 instead of 66.38), which we first misread as a cost of
reasoning. Both are off in every run of this report (Appendix~\ref{sec:E}).


==> sections/09_conclusion.tex <==
\clearpage
\section{Conclusion}\label{sec:9}

StartLux-Decision answers typed questions with probabilities in one forward pass, on text of up to
262,144 tokens and on images, and the same weights reason when the one-pass answer is unsure. On the
public index the 27B reaches 70.4 in one pass and 72.3 with reasoning, against 63.9 for the released
checkpoint, and most of that suite is in-domain for it. On decisions outside the suite the data
rounds do not help.

Four results are meant to be of use beyond these models. A loss on the answer alone leaves the end
of a thought unsupervised, so a model can lose the ability to finish reasoning while its answers
improve, and the probability of closing a finished thought shows where this happens. A group of
training data helps only the task families it contains, so reused test sets measure exposure, about
nine points of it, and transfer has to be read on tasks nobody trained near. Reinforcement learning
with a proper score calibrates the answer after a thought mostly by shortening the thought. And a
confidence that selects an answer overstates the selected answer, by an amount a calibration map
removes when it is given what the policy looked at.

\textbf{Next steps.} (1) Settle the recipe at 4B with the rounds that were running when this was
written (the hygiene repairs, contrast pairs, larger original-source files, the public procedural
corpus, a repeat of the final recipe, and bidirectional attention over the prompt, which raised
every measure in its first run), carry it to 9B, and train the 27B only then. (2) Put the reasoning
stages inside the data round, so that the end of a thought is supervised whenever the answer is, and
give the two smallest sizes reasoning stages. (3) Test reinforcement learning as a calibration step
with second seeds and at 9B. (4) Grow DecisionPivot with generated families of new kinds and input
variants. (5) Find a certificate that survives a change of the number of candidates or of the think
rate without new calibration data.


==> sections/09_contributions.tex <==
\section*{Author contributions}
\phantomsection\addcontentsline{toc}{section}{Author contributions}

\todo{author list and contributions by area (full-parameter SFT, adapter training and ablations,
reasoning data, reinforcement learning, policy-aware calibration and certificates, evaluation and
DecisionPivot, serving and runtime, data sourcing and licences, report), in the manner of the Olmo 3
report}

\textbf{Acknowledgements.} \todo{acknowledgements}


==> sections/09_limitations.tex <==
\section{Limitations and negative results}\label{sec:9}

\textbf{Limitations.}

\begin{itemize}
\item \emph{The index is mostly in-domain for the later checkpoints.} After the data rounds 33 of its 38
benchmarks have training data aimed at them, and the gain from 63.9 to 70.4 at 27B measures the fit
of the recipe to the suite. On decisions the rounds were not aimed at they change the score by
$-$1.0 at 27B and by nothing at 9B and 4B, and every such difference below about one point is within
the spread between two training runs of one recipe.
\item \emph{Every index value includes GSM8K rows that can be answered from the layout of their options},
0.7 index points for the released 27B and 1.0 for the released 4B (Table~\ref{tab:E.7}). We
recomputed our own checkpoints with the rebuilt rows but not the systems of other groups, whose
values keep the old rows.
\item \emph{No measurement on the private tests of edition 0.3.} Our local stand-ins have limits of their
own: the generated tasks are ours and new, the reused tasks favour whoever trained on related
material, and a twin measures transfer only for a model that has not trained on its family.
\item \emph{Decontamination at the release was partial.} Rebuilt training splits were scanned and not
filtered, and 68 rows repeat a test item. The comparison finds equal text, not paraphrases.
\item \emph{Single rounds.} Most comparisons between training rounds rest on one round per condition. The
same recipe trained twice differs by 0.18 index points and by up to 7 points on one benchmark, and a
second run of the 4B-Rounds recipe was still running when this was written.
\item \emph{Reasoning is incomplete and costly at 4B and 9B.} The untrained starting models still think
better on arithmetic than ours (97.1 and 98.6 against 94.4 and 96.3), the 0.8B and 2B have no
reasoning stages, and a thought lowers accuracy on select-all and NLI-like questions. One threshold
and one mixture weight serve all task families.
\item \emph{Images and long inputs are inherited abilities.} Decision training used text only, and long
inputs were measured on documents up to 128K tokens and retrieval items up to 248K, not at the full
context.
\item \emph{Certificates are marginal and local.} A certificate holds for the calibration distribution,
the policy and the number of candidates it was computed for, and it does not transfer across task
families.
\item \emph{Data.} No person has audited the written and generated training data, teacher-written rows
were filtered by two verifier models, and several sources carry share-alike, non-commercial or
research-only terms.
\end{itemize}

\textbf{What did not work.} Each item is reported where it occurred. They are results for our
models, data and settings and do not show that an idea cannot work elsewhere.

\begin{itemize}
\item \emph{Training the one-pass model.} A second-stage adapter on rows the first model gets wrong (all
eleven runs below their parent). All weights trained from the untrained 4B with the settings of the
leading entries (40.87 and 44.71 against 52.76 for the released 4B). More rows of the same families
(65.6 against 65.7 on the twins at 1.7 times the rows). Distantly labelled sarcasm data and other
stance data sets, which lowered their twins. Removing VAST against the stance bias (the stance twin
fell from 38.7 to 29.5). Breadth rows alone at 4B, which moved no overall score.
\item \emph{Data that looked right.} An official training set whose label prior differs from the
benchmark's (63.3 $\rightarrow$ 36.5 on that benchmark at 4B), generated code-execution rows
(24.9--27.1 $\rightarrow$ 13.4--15.1), and a duplicate filter keyed on the wrong fields.
\item \emph{Reasoning.} A longer token limit (87.4\% of the thoughts still running at 16,384 tokens), a
lower gate on the index (67.20 against 67.72), one joint stage in place of three (67.11),
reinforcement learning as a way to better answers (no arm above the supervised stages), two-stage
``calibrate, then reinforce'' training (three points of the one-pass answer lost), and thinking
again when the confidence is below 0.6 (73.41 against 73.44 with the first thought in context).
\item \emph{Serving.} Prefix caching and chunked prefill in a third-party server changed results
(Chapter~\ref{sec:8}), and 8-bit weight formats were slower than bf16 on H200.
\end{itemize}

\textbf{Intended use.} Typed decisions inside a system that a person or a program has framed:
routing and triage, checks on inputs and outputs, relevance and matching, verification of an answer
against evidence, choosing among candidate responses. A threshold should be set on labelled examples
of the deployment's own data, and a probability that was used to select an answer should not be
reported as the accuracy of the selected answers without the calibration of Chapter~\ref{sec:7}. The
models are not meant for decisions about individuals in medicine, law, credit, employment or safety
without review by a qualified person, nor as the only guard against harmful content, and the weights
may not be used commercially.


==> sections/09_negative_limits_use.tex <==
\clearpage
\section{What did not work, limitations, intended use}\label{sec:9}

\subsection{What did not work}\label{sec:9.1}

Each item is reported where it occurred, with its numbers. This section collects them. They are
results for our models, data and settings. None of them shows that the idea cannot work elsewhere.

\textbf{Training of the one-pass model.}

\begin{itemize}
\item \emph{A second-stage adapter on the fine-tuned weights}, trained on the rows the first-stage model
gets wrong with replay of its own distribution: all eleven runs of the second and third day scored
below their parent on the index, by 0.50 to 2.86 points, while the development set from the source
of the new rows rose in every run (Section~\ref{sec:5.2}). No released model contains it.
\item \emph{One learning rate for all sizes:} at 2e-5 the 9B scored 51.68, below the 4B at the same rate
(54.82).
\item \emph{The decision recipe as an adapter on the untouched starting model}, the design in which the
starting model stays intact for reasoning and an adapter gives the fast answer: 63.34 at rank 64 and
58.16 at rank 256, against 64.78 for the same data round on the released weights (4B, one pass).
\item \emph{An official training set taken on trust:} rows from the official training split of a
tool-retrieval benchmark took that benchmark from 63 to 36.5 at 4B and from 61.8 to 34.9 at 9B. The
split has 29\% relevant candidates and easy negatives, the benchmark 3\% and near neighbours
(Section~\ref{sec:4.6}).
\item \emph{Generated code-execution items} whose wrong options were outputs of nearby programs lowered
the real benchmark from 24.9--27.1 to 13.4--15.1 at 4B.
\item \emph{Procedural items aimed at a public benchmark's weak categories:} 16,000 generated date,
invoice and rule items lowered the count of correct public items from 209 to 204.
\item \emph{A decision head on a frozen reasoning backbone:} 58.5\% against 70.3\% for the adapter-trained
decision model on the same items. The head improved calibration and not accuracy.
\item \emph{Latent reasoning:} latent slots and serial latent steps in place of written reasoning gave no
gain on the decision suite.
\item \emph{Proper-score objectives for the one-pass answer:} three graded-target forms trained on the
same data score 58.03, 58.20 and 58.06 on the index. In an earlier reproduction the index was flat
and the calibration error fell from .051 to .039. For a one-pass answer the expected proper score is
a supervised loss, and we see no more than that.
\item \emph{Data rounds aimed at the index, on decisions outside it:} on the unseen items of 35 reused
public test sets the final round changes the score of the released weights by $-$1.0 at 27B
(interval $-$1.6 to $-$0.4), 0.0 at 9B and +0.1 at 4B. On 20 twin test sets the 27B goes from 71.1
to 71.3. On the GSM8K rows as rebuilt for edition 0.3 the rounds are below the released weights at
every size (by 6.8, 4.7 and 14.2 skill points at 27B, 9B and 4B). A half-and-half blend of the
released 27B with the round keeps 82\% of the gain on the public index and gives back about 70\% of
the loss on unseen tasks (Sections~\ref{sec:5.3} and \ref{sec:6.14}).
\item \emph{Breadth rows alone, in our recipe at 4B:} a round on 642,628 rows from 343 task families of a
public collection, with the core of the release mix and no index-targeted file, differs from the
released 4B by +0.7 on the index (53.44 against 52.76), $-$0.6 on the unseen items of 35 reused test
sets (interval $-$1.4 to +0.1), 0.0 on the generated tasks, +0.7 on the twin test sets and $-$0.7 on
the rebuilt GSM8K rows. Added to the final-recipe mix, 200,000 such rows give 65.03 on the index
(64.78 without them) and cost 1.1 points on the unseen items ($-$1.7 to $-$0.4) and 2.6 on the
generated tasks (52.5 against 55.1). One size, an adapter round at a learning rate of 5e-5. The
entries whose model cards led us to this data train all weights at 2e-6.
\item \emph{Other data sets of the ``same'' skill to repair a twin:} with 17,378 rows of other stance data
sets and 18,158 rows of other sarcasm and irony data sets in its mix, that round scores 36.9 on the
stance twin against 44.9 for the released 4B, and 32.6 on the sarcasm twin against 39.2. No interval
has been computed. Both files are left out of the full-coverage round that followed
(Section~\ref{sec:6.15}).
\item \emph{GSM8K's training split as a source of arithmetic rows:} 6,017 of its 7,473 problems (80.5\%)
carry text of protected evaluation items, because the routing benchmark of the index takes GSM8K
training problems as its prompts. The split is not used. The arithmetic file holds two other
sources, and the 1,456 problems without such text are held aside (Section~\ref{sec:4.1.1}).
\end{itemize}

\textbf{Reasoning.}

\begin{itemize}
\item \emph{A longer token limit:} at 16,384 tokens 87.4\% of the 4B's thoughts are still running, and
accuracy is unchanged at 3.9 times the tokens (Section~\ref{sec:5.4}). At 8,192 tokens with a loop
check the default answer is 0.43 points lower on held-out items (interval $-$1.09 to +0.20), and on
the index a limit of 8,192 tokens scores 67.52 against 67.72 at 4,096.
\item \emph{A lower gate:} on held-out items of the training distribution, thinking only when the one-pass
top probability is below 0.7 gives the accuracy of the default of 0.9 with about half as many
thoughts (90.71 both). On the index it costs half a point: 67.20 against 67.72 for the 4B after
thinking replay and reader round (Section~\ref{sec:5.1.2}). The default stays at 0.9.
\item \emph{A repetition penalty with a loop detector} ends more thoughts and loses half a point
(Table~\ref{tab:5.5}).
\item \emph{Cutting every thought at 1,024 tokens} is free on held-out items and costs 0.79 index points
(Table~\ref{tab:5.6}).
\item \emph{One joint stage in place of the three reasoning stages:} 67.11 against 67.72 on the index,
with retrieval 3.7 points lower, and a stop step on top of it, 66.42 (Section~\ref{sec:5.8}).
\item \emph{Reinforcement learning of the thinker} has not raised accuracy over the supervised stages in
any arm. From the data-round 4B, which hardly reasons, policy-gradient training with a price per
token learns to skip: two thirds of the thoughts are closed without a word, and the 67.18 it reaches
on the index (0.54 below the supervised sequence) comes from the remaining third, where it is weaker
than the replayed thinker. From a model that already ends most of its thoughts it shortens them and
costs about half a point: with rollouts sampled as at inference 99.7\% of the 4B's thoughts end at
about a third of the tokens, with a default answer of 75.07 against 75.31 on held-out items and an
index of 66.80 against 67.37 in one run. At 9B the index is 69.52 against 70.16. What this training
does change, besides length, is calibration: before any temperature is fitted, the calibration error
of the answer after the thought is 32\% lower at 4B (9.43 $\rightarrow$ 6.38) and 43\% lower at 9B
(3.77 $\rightarrow$ 2.14), without a better ranking of right and wrong answers. The control with a
plain accuracy reward was still running. A price alone or a noise reward comes within half a point
to a point of the real reward. With the log score in place of a bounded score the thoughts grow.
From a model whose samples do not end, the reward does not move (Section~\ref{sec:5.9}). Earlier
variants tied their supervised or simpler counterparts: rewards that are pessimistic about
selection, coherent rewards for a judge (about 80 where the plain vote baseline reaches 80.5 to
81.0), exact counterfactual credit and branch selection. Training a reasoner with the reader's
proper score as reward left the route effect of Chapter~\ref{sec:7} where it was ($-$.279 before,
$-$.272 after).
\item \emph{Two stages, ``calibrate, then reinforce'':} training the read-out on 5,120 items of thoughts
sampled by the current model costs three points of the one-pass answer (68.2 to 68.4 against 71.43),
and the four arms of the second stage end at 72.4 to 73.6 for the default answer against 75.31 for
the supervised chain. The line is closed.
\item \emph{Thinking again when the confidence is below 0.6:} with the first thought in context the
accuracy does not change (73.41 against 73.44, $-$0.04, interval $-$0.50 to +0.43). A new
independent thought is 0.32 points below averaging the same thoughts ($-$0.68 to 0.00) and 1.05
points more overconfident (Section~\ref{sec:7.3}).
\item \emph{A weight of the thought that depends on the one-pass confidence:} no rule chosen on one half
of the held-out items beats the flat 0.5 / 0.5 mixture on the other half (90.12 at 4B, 92.96 at 9B,
Section~\ref{sec:7.1}).
\end{itemize}

\textbf{Evaluation.}

\begin{itemize}
\item \emph{GSM8K in edition 0.2.1 of the index as a test of arithmetic:} its rows could be answered from
the layout of the options. On the rows rebuilt for edition 0.3 the one-pass skill of the released
27B is 60.5 instead of 95.3 and that of the released 0.8B 2.0 instead of 89.4
(Section~\ref{sec:6.2.1}).
\item \emph{The reused half of our own benchmark as a measure of general ability:} over its 35 tasks the
lead of the released 27B over Perplexity Decider v1.1 follows the share of a task's items that our
training files held before cleaning (rank correlation +0.29, with +0.8 on the 13 tasks with at least
3\% found, $-$1.1 on the other 22). It favours models trained on related material, ours included,
and we report no total for it (Section~\ref{sec:6.14}).
\item \emph{A stand-in for the board's private tests picked task by task:} rank correlations of 1.00 and
0.71 on the seven models it was chosen on fall to 0.64 and 0.29 when a model is left out.
\end{itemize}

\textbf{Serving.} Prefix caching in a widely used inference server moved 2.6\% of the one-pass
read-outs of our hybrid-architecture models by more than 0.05 and changed 16\% of the answers on
wide choices (Section~\ref{sec:8.4}). It is off in every run of this report. \emph{8-bit weight
formats for speed:} on H200 GPUs the 9B with 8-bit integer weights, or with 8-bit floating-point
weights and activations, answers 8 to 20\% fewer requests per hour than in bf16 at 1,024 to 16,384
tokens. The formats save 6.5 GB of memory per GPU, and their accuracy has not been evaluated
(Section~\ref{sec:8.1.1}).

\subsection{Limitations}\label{sec:9.2}

\begin{itemize}
\item \textbf{The index is mostly in-domain for the later checkpoints.} After the data rounds, 33 of its
38 benchmarks have training data aimed at them (Table~\ref{tab:4.3}). The gain from 63.9 to 70.4 at
27B measures the fit of the recipe to the suite: on 35 decision tasks that the rounds were not aimed
at, the same rounds change the score by $-$1.0 at 27B and by nothing at 9B and 4B
(Section~\ref{sec:6.14}). Further evidence from sets that never entered training is in
Sections~\ref{sec:6.5} to
\ref{sec:6.10}.
\item \textbf{Every index value includes GSM8K rows that could be answered from the layout of the
options.} The values of this report are edition 0.2.1 values. With the rows rebuilt for edition 0.3
the released 27B would have about 0.8 index points less and the released 4B about 1.2. No value has
been recomputed.
\item \textbf{No measurement on the private tests of edition 0.3.} Four fifths of that edition's score are
private tests, which we cannot run. Its main ranking does not count models that may think, and no
entry of ours has been submitted. Our local substitutes (generated tasks, reused public test sets
and twin test sets) have limits of their own: the generated tasks are ours and one day old, the
reused half favours whoever trained on related material, and a twin measures transfer only for a
model that has not trained on its family (Sections~\ref{sec:6.3.1} and \ref{sec:6.14}).
\item \textbf{Decontamination at the release was partial.} Training rows built from official training
splits were scanned against the test rows and not filtered: 23,209 of them share a passage of text
with a test row (20,253 in the 27B mix). A row-by-row comparison finds 68 rows that repeat a test
item and none among the 162,865 rows of the largest flagged group. They are one contract with its 17
questions, one sarcasm item and 50 intent utterances (the contract and the utterances are in both
official splits of their sources). The comparison finds equal text, not paraphrases
(Section~\ref{sec:4.5}).
\item \textbf{Single rounds.} Most comparisons between training rounds rest on one round per condition.
The same recipe trained twice differs by 0.18 index points and by up to 7 points on one benchmark
(Section~\ref{sec:6.1}).
\item \textbf{Reasoning at 4B and 9B is expensive or incomplete.} The best 4B and 9B results are obtained
with more than half of the thoughts cut at the token limit before the stop step, which removes most
of this (for 0.35 index points at 4B and with a gain of 0.39 at 9B) and still leaves 10\% (4B) and
16\% (9B) of the thoughts at the limit. After reinforcement learning 0.4\% of the 4B's thoughts
reach the limit, for a further 0.57 index points in one run (Section~\ref{sec:5.9}). A loop check at
inference has been measured on held-out items only. The 0.8B and 2B have no reasoning stages.
\item \textbf{The reasoning stages do not return all of the starting model's reasoning.} On GSM8K rows
without a shortcut in the options the untrained 4B and 9B reach a skill of 97.1 and 98.6 after a
thought, our models 94.4 and 96.3, and the untrained 4B writes thoughts less than half as long
(Table~\ref{tab:5.9}).
\item \textbf{The held-out items we used to choose designs under-represent hard knowledge questions.} A
cut that is free there costs 0.8 points on the index (Section~\ref{sec:5.7}).
\item \textbf{Reasoning does not help everywhere.} At 27B four benchmarks lose 3.3 to 5.7 raw points with
reasoning (a home-appliance simulator, a select-all set, a narrative-reasoning set, a deliberation
set). On held-out items of the training distribution the answer after a thought is worse than the
one-pass answer in 7 of 21 task families at 4B, most on select-all questions ($-$7.0), ANLI ($-$4.8)
and ContractNLI ($-$2.4) (Section~\ref{sec:5.1.1}). The default threshold and the mixture weight are
one value each for all task families.
\item \textbf{Images and long inputs are inherited abilities.} Decision training used text only. Image
results (Section~\ref{sec:6.7}) come from the starting model's vision tower read through our
read-out. Long inputs were measured on documents up to 128K tokens and retrieval items up to 248K
(Section~\ref{sec:6.5}), not at the full context.
\item \textbf{Probabilities about other models are not usable.} Asked whether a given chat model will
answer a question correctly, no model of the family gives probabilities that beat quoting that
model's base rate by more than 0.03 in skill (one of fourteen cells is above zero, at +0.02),
although they rank questions moderately well (AUROC 0.70 to 0.80, Appendix~\ref{sec:H.10}).
\item \textbf{Certificates are marginal and local.} A certificate holds for the calibration distribution,
the policy and the number of candidates it was computed for. It does not transfer across task
families, and the policy-aware map carries the calibration to other numbers of candidates, not the
guarantee (Chapter~\ref{sec:7}).
\item \textbf{Scope of the evidence.} Typed decisions and the verification of short answers, in English
and on one Chinese benchmark. Free-form generation is outside the scope of the models and of this
report.
\item \textbf{Data.} No human audit of the written and generated training data exists. Several sources
carry share-alike, non-commercial or research-only terms (Appendix~\ref{sec:G}). Teacher-written
rows were filtered by two verifier models, not by people.
\item \textbf{Other teams' models} were run by us from their public weights and code in the documented
configuration, or are quoted from their own reports with the date. We made no ablation of another
team's model.
\end{itemize}

\subsection{Intended use and out-of-scope use}\label{sec:9.3}

\textbf{Intended use.} Typed decisions inside a system that a person or a program has framed:
routing and triage, checks on inputs and outputs, relevance and matching, verification of an answer
against evidence, choosing among candidate responses, extraction of a field with listed values. The
one-pass mode is meant for high-volume decisions where latency matters, and the reasoning mode for
the minority of questions on which the one-pass answer is unsure and a wrong answer costs more than
a few hundred tokens.

\textbf{Using the probabilities.} A threshold should be set on labelled examples of the deployment's
own data, per question, and re-checked when the data change. A probability that was used to select
an answer (the best of several candidates, the answers above a threshold, the answers that were
routed to reasoning) should not be reported as the accuracy of the selected answers without the
calibration of Chapter~\ref{sec:7}.

\textbf{Out of scope.}

\begin{itemize}
\item Decisions about individuals in medicine, law, credit, employment or safety without review by a
qualified person. The models were not evaluated for such use and the report gives no evidence about
fairness across groups.
\item Use as the only guard against harmful content or prompt injection. A guard needs measurement at
fixed low false-positive rates on the deployment's inputs. We report accuracy and the effect of
option order on public sets only (Section~\ref{sec:6.10}).
\item Free-form generation. The reasoning text is an intermediate product for the model's own second
read-out. It is not checked for correctness and is not returned to the caller.
\item Languages other than English and Chinese, which were not evaluated.
\item Commercial use of the released weights, which their licence does not permit.
\end{itemize}


==> sections/10_conclusion.tex <==
\section{Conclusion}\label{sec:10}

StartLux-Decision returns probabilities that a system can act on, from one forward pass, and reasons
in the same weights when the one-pass answer is unsure. On the public index the 27B reaches 70.4 in
one pass and 72.3 with reasoning, against 63.9 for the released checkpoint, and most of that suite
is in-domain for it.

The report followed four places where that promise can fail. A loss on the answer alone takes away
the end of a thought while the answers improve, and the probability of closing a finished thought
shows where, so that three stages can give it back. A group of training data helps only the task
families it contains, so a score on reused test sets measures exposure, about nine points of it, and
transfer has to be read on tasks nobody trained near. Reinforcement learning with a proper score
calibrates the answer after a thought mostly by shortening the thought, and has not made the answers
better. And a confidence that selected an answer overstates it, by an amount a calibration map
removes when it is given what the policy looked at. The calibration maps, the closing-probability
probe and the exposure flags of DecisionPivot let others check the same failures in their own systems.

Two questions stay open. Can a recipe raise decisions outside the index as well as on it?
Bidirectional attention over the prompt is the first change that did so, on two data mixes at 4B,
and its use from the first stage of training was running when this was written. And can the end of a
thought be supervised inside the data round itself, so that no repair stage is needed? Our one joint
stage on a small read-out mix did not hold the one-pass answer.


==> sections/10_related_work.tex <==
\clearpage
\section{Related work}\label{sec:10}

\textbf{Decision and guard models.} Several open decision models read the options in one pass,
through a pointer or scoring head (Clef and Clef-flash, K2-Type-1B) or through the logits of the
option labels (mogan-decision-31B-it), and have no path for thinking. The hosted reference model has
no reasoning setting either. Our models read the option letters at one position of the language
model and can think with the same weights (Sections~\ref{sec:3.2} and \ref{sec:3.4}). SearchJev
\citep{cao2026searchjev} hands the uncertain decisions of a search agent to a generative model and
reports one calibration error for all decisions. Chapter~\ref{sec:7} separates the answers kept from
those handed over. Balam (5 October 2026, not peer-reviewed) reports that the score of the hosted
reference model as a prompt-injection guard ranks attacks but is not a calibrated probability, and
that a cut-off chosen on one set blocks most clean documents of another input type, a shift of data
that motivates certifying a threshold where it is used. An independent evaluation of the hosted
reference against eleven chat models (Vals AI, 6 October 2026, not peer-reviewed) fits each system's
confidence threshold for a 1\% error budget on 30\% of 400 claim-verification items and applies it
to the rest: six of the twelve systems exceed the budget on the held-out part, and the hosted
model's calibration error is 0.011 on that task and 0.108 on a legal one. The held-out part has 265
items and the miss is a finite-sample and task-shift effect, not the selection effect we study. It
is the practice that a certificate replaces. A second hosted interface for typed decisions with
probabilities opened in the same week (OpenAI Decisions API, public beta). Its documentation, like
the first, leaves the choice of the threshold to the caller.

Two further lines appeared while this report was written. Vela 2.0 (vLLM Semantic Router and KR
Labs, 7 October 2026, model cards and a blog post, not peer-reviewed) is a family of open routing
models of 0.3B to 9B parameters, the largest derived from Decision-2.0-Lux-9B, which shares its base
model family with our 9B. Besides choice, yes/no and score questions it returns two answer types
that our interface lacks: labelled character spans (personal information, claims of an answer not
supported by its source, open labels) and sets, in which every listed label gets its own
probability. Its training keeps the earlier decisions with a KL term to the starting model and a
7.5\% replay of its rows, the same purpose as our anchor rows. It reports 41.6 on edition 0.2.1 of
the index, and Decision-2.0-Lux-9B 46.3. The second line is reasoning only when a decision needs it:
the maker of the Sage decision model describes, in a public post of 6 October 2026, a mode that
answers at one-pass speed when the question is easy and spends more time otherwise, and names two
other providers that offer the same. No measurement accompanies these announcements. Our gate is
such a mode. What this report adds is where the extra time helps and where it hurts
(Sections~\ref{sec:5.1} and \ref{sec:6.12}), what it costs (Chapter~\ref{sec:8}), and how far the
confidence of the answers it returns can be trusted.

\textbf{Probability read-outs and calibration.} Among decision models, Kev fits one temperature per
checkpoint and metask-jev-rain-4B one per path and question kind. We fit one per question type. A
quantity chosen because it looked best is biased upward, and statements about it must account for
the choice: the winner's and the optimiser's curse \citep{smith2006optimizers}, selective and
post-selection inference \citep{benjamini2005false,berk2013valid,lee2016exact} and the
empirical-Bayes correction of the largest of many noisy estimates \citep{efron2011tweedie}. The
confidence reported for an answer a policy selected is such a quantity, and our set-aware
calibration map (Section~\ref{sec:7.5}) is in the spirit of Efron's correction: it uses the other
candidates' scores to say how much of the winner's score is selection. Calibration degrades when the
population shifts \citep{guo2017calibration,ovadia2019can}, and multicalibration asks for it on
every member of a fixed class of subpopulations \citep{hebertjohnson2018multicalibration}.
Policy-aware calibration is that demand for the populations a policy produces, met with a held-out
sample of its outputs. A linear pool of calibrated forecasts is under-confident and needs
recalibration, and a log-linear pool does not share the defect \citep{ranjan2010combining}. The
default answer of our reasoning mode is a linear pool of two read-outs, and we measure what that
costs a caller who automates above a threshold.

\textbf{Selective prediction and conformal certificates.} Selective classification bounds the risk
of accepted cases \citep{geifman2017selective} and Learn then Test certifies a threshold by
fixed-sequence testing \citep{angelopoulos2021learn}. Our certificates are these procedures, with
calibration data from the policy's own outputs. \citet{cheng2026signed} certify an accept-or-defer
threshold for the answers a first stage keeps and not, as we do, for those after deferral. Choosing
the best of several valid conformal sets breaks coverage \citep{hegazy2025valid}, the same
phenomenon without computation policies. Cascades defer on a low score \citep{chen2023frugalgpt}.
Studies of accept-or-escalate cascades \citep{li2026jev} and of stages whose errors coincide
\citep{rao2026jev,bouchard2026escalation} concern the accuracy of the cascade, and none analyses the
confidence of the delivered answer by route, which we measure. Self-consistency
\citep{wang2023selfconsistency} and test-time compute \citep{brown2024large,snell2024scaling} raise
accuracy by sampling, with the verifier as the limit. We study the confidence delivered with the
selected answer.

\textbf{Reasoning control.} Rational metareasoning runs a computation when its expected gain exceeds
its cost \citep{horvitz1987reasoning,russell1991principles,hay2012selecting}. Our control is one
threshold on the one-pass confidence, and the value gate estimates the gain with a typed question.
Of the public systems we read (6 October 2026), GEV-26B-Decide writes the thought with the base
model and keeps the decision adapter for the fast pass. TypeLLM trains nothing and, in its
\texttt{\textquotedbl{}thinking\textquotedbl{}: \textquotedbl{}auto\textquotedbl{}} mode, first asks
an untouched model how much reasoning the question needs, where our gate asks whether reasoning is
worth its cost. Rune 26B-A4B v3 and metask-jev-rain-4B think with decision-trained weights for a
short budget and document no training of the reasoning. Jeeves-9B is the one public system we found
that, like ours, trains the same weights to write the chain and to decide. Its card reports that
about one third of full-length chains reach the token cap without closing. We found no loop
detection in the code we read and no loop rate for a decision-trained model. In a study of decision
fine-tuning \citep{li2026llmasjev}, KL anchors to the base model largely stop the model from running
on past its answer. We find that decision training also damages the end of a thought at 4B and 9B,
which a loss on the thought restores (Sections~\ref{sec:5.4} and \ref{sec:5.5}).

\textbf{Reinforcement learning for calibrated decisions.} The hosted reference model is trained with
RLCD for calibrated decisions (its models page). No algorithm is published. \citet{gao2026openjev}
give an open implementation for a reasoning model and the analysis closest to our
Sections~\ref{sec:5.6} to \ref{sec:5.9}. They read the answer distribution after a sampled rationale
and score each rationale's own distribution with a proper score, because scoring the mixture of
several rationales pays for their disagreement. Trained end to end, the objective either stops
reasoning or is drowned by the policy gradient, so they first train the read-out on the model's own
rationales and then reinforce the reasoning with an anchor at that model. Three of their
observations have counterparts here. A thinker scored by a frozen reader shortens its reasoning (our
arm that learned to skip). Training the read-out without an anchor on the rationale ends in
rationales that repeat their conclusion to the length limit (our reader round). Most of the gain
comes from the supervised stage, not from the policy gradient. Their study has one 1.7B model
without a one-pass decision to preserve and no gate. Ours adds the loss of the thought ending under
decision training, its repair, and the index-scale cost. The ratio of the two gradients depends on
how the policy gradient is normalised: summed over a rationale's tokens it is 7 to 12 times the
read-out's in their runs, averaged over the tokens it is 1.5\% of it in ours. Their central claim,
that a proper-score reward calibrates the read-out after the rationale, has a partial counterpart:
our arms lower the raw calibration error of that read-out at 4B and 9B, but an arm rewarded for
accuracy alone with the same sampling does most of it at 4B, and the same proper score without the
length price makes the thoughts longer and the answer more over-confident, so in our runs the change
follows the length of the thought, not the score. Second seeds are running.
\citet{deka2026retrieval} finds on one biomedical encoder that a released calibration-reward recipe
trails cross-entropy on the training tasks, not on held-out ones, mainly through dividing the
rewards by their minibatch standard deviation. Optimising against a learned reward degrades the true
reward \citep{gao2023scaling}, a force that we measure on reported confidence.


==> sections/11_author_contributions.tex <==
\section*{Author contributions}
\phantomsection\addcontentsline{toc}{section}{Author contributions}

\todo{author list and contributions by area (release stage, decision data rounds and ablations,
reasoning stages, reinforcement learning, policy-aware calibration and certificates, evaluation and
DecisionPivot, serving and runtime, data sourcing and licences, report), in the manner of the Olmo 3
report}

\textbf{Acknowledgements.} \todo{acknowledgements}


==> sections/11_conclusion.tex <==
\clearpage
\section{Conclusion}\label{sec:11}

StartLux-Decision is a family of open models that answer typed questions with probabilities in one
forward pass, on text of up to 262,144 tokens and on images. This report has described how the
models are made: a release recipe that averages a fully fine-tuned model with an adapter-trained
one, data rounds that add what the model had not been shown, and three stages that give the same
weights most of their reasoning back. On the public index the 27B reaches 70.4 in one pass and 72.3
with reasoning at the default threshold, against 63.9 for the released checkpoint, and most of the
suite is in-domain for it. On decisions outside the suite the data rounds do not help, and about 0.8
index points of the released 27B's value rest on GSM8K rows that the next edition of the index has
rebuilt (Sections~\ref{sec:6.2.1} and \ref{sec:6.14}).

Three things in it are meant to be of use beyond these models. A decision loss leaves the end of a
thought unsupervised, and a model trained with it can lose the ability to finish reasoning while its
answers improve. The probability of closing a finished thought shows where this happens, stage by
stage. A confidence that selects an answer overstates the selected answer, by an amount that grows
with the number of candidates and that a calibration map can remove when it is given what the policy
looked at. And the cheapest gains in building the models came from reading error tables by category,
while the costliest mistakes (a label prior taken from an official training set, a duplicate filter
keyed on the wrong fields, a serving option) produced no error message.

\textbf{Next steps.} (1) The reasoning stages inside the data round, so that the end of a thought is
supervised whenever the answer is. Our joint stage on a small readout mix did not hold the one-pass
answer. (2) Reasoning stages for the two smallest sizes. (3) Reinforcement learning as a calibration
step, tested properly. So far it makes nearly every thought end, at about a third of the tokens,
costs about half a point after the thought, and lowers the raw calibration error of the answer after
a thought (4B: 9.5 to 6.9 with a Brier reward). An accuracy reward with the same sampling reaches
7.8, and without the length price the proper score makes thoughts longer and the answer more
over-confident (11.2, Section~\ref{sec:5.9}). What is left for the proper score, about 0.9 points in
one run, needs the second seeds and the 9B comparison that are running. (4) Evaluation on decision
tasks that no model of the family was trained for (the decisions inside language-model systems
before, around and after generation) as a separate benchmark with generated tasks as its headline,
because reused public test sets favour whoever trained on related material. (5) A certificate that
survives a change of the number of candidates or of the think rate without calibration outputs at
the new setting. (6) A training recipe judged on decisions the index does not hold. Breadth alone
did nothing at 4B (index 53.4 against 52.8 for the released model, unseen tasks $-$0.6). A round
that adds breadth and the train splits of the families of our stand-in test sets for the private
parts of the next index edition raised that stand-in from 61.6 to 65.7 at 4B, about half of it from
those train splits, with the public index unchanged and $-$1.0 on unseen tasks
(Section~\ref{sec:5.3}). Rounds that separate the data groups, a recipe trained from the untrained
base at a small learning rate as the leading entries do, and larger amounts of the families where
the leader is far ahead are running at 4B. The 27B waits for their reading.

